From User Perceptions to Technical Improvement: Enabling People Who Stutter to Better Use Speech Recognition

Consumer speech recognition systems do not work as well for many people with speech diferences, such as stuttering, relative to the rest of the general population. However, what is not clear is the degree to which these systems do not work, how they can be improved, or how much people want to use them. In this paper, we frst address these questions using results from a 61-person survey from people who stutter and fnd participants want to use speech recognition but are frequently cut of, misunderstood, or speech predictions do not represent intent. In a second study, where 91 people who stutter recorded voice assistant commands and dictation, we quantify how dysfuencies impede performance in a consumer-grade speech recognition system. Through three technical investigations, we demonstrate how many common errors can be prevented, resulting in a system that cuts utterances of 79.1% less often and improves word error rate from 25.4% to 9.9%.

==> CHI2023 Stuttering/sections/1-introduction.tex <==
\section{Introduction}
Performance of speech recognition systems has improved substantially in recent years, leading to widespread adoption of speech input across computing platforms. Speech is especially important for devices with limited or no screen real estate, such as smart speakers (e.g., Amazon Echo, Google Nest Audio)
and hearables (e.g., Pixel Buds, Apple AirPods), where it is used 
%Speech recognition technology is ubiquitous and its importance has increased with screen-free devices like smart speakers and hearables (e.g., Pixel Buds, Apple AirPods). 
for everyday tasks like playing music, searching for facts, and controlling smart devices in the home~\cite{AmmariCHI21}.
% and for reading dialog on streaming video.
%Automated captions, while error prone, have improved the accessibility of speech in video and are common on modern streaming services~\cite{glasser2017deaf}. 
% This importance is only expected to increase with the development of new always-on consumer AR/VR devices~\cite{?} where speech could replace existing touch controls. 
%While performance of speech recognition systems has improved significantly in recent years,
%thanks to advances in machine learning,
Yet, speech interaction presents accessibility barriers for many people with communication disabilities such as stuttering, dysarthria, or aphasia~\cite{projecteuphonia,ballati2018assessing,fok2018towards,roper2019speech}.
%limiting who can use what consumer technology and is ultimately an access barrier and an equity issue.
% In a world where speech is a primary mode of interaction, it is imperative that these systems work for everyone.
In this work, we investigate user experiences and speech recognition system performance with one large population in this demographic of communication disability: people who stutter (PWS).

Stuttering, also called stammering~\cite{ward2011cluttering}, impacts approximately 1\% of the world's population, although estimated incidence ranges from 2\% to 5\% for sub-populations such as children and males~\cite{craig2002epidemiology}.  
% Stuttering and cluttering are types of fluency disorders, defined by an interruption in the flow or fluidity of connected speech. 
Stuttering is a breakdown in speech fluency that can affect the rate and flow of speech and can include dysfluency types such as sound repetitions (``p-p-pop''), syllable repetitions (``be-be-become''), word or phrase repetitions (``mom, mom, mom''), sound prolongations (``mmmmmom''), and audible or silent blocks (pauses or breaks in speech) \cite{sander1963frequency, SSI}. 
% (inability to initiate target sound)
Frequent interjections (``um'', ``eh'') are also common. 
The rate, duration, and distribution of these dysfluencies varies substantially between people and across contexts~\cite{tichenor2021variability}. 
% , which commonly assumes fluent speech~\cite{clark2020speech}.
% \note{move} Stuttering may be developmental, neurogenic, or psychogenic \cite{roth1989clinical, seery2005differential}.  


% Speech recognition systems are not tuned to understand these dysfluencies, which means it is an access barrier for modern voice-driven technology, which commonly assumes fluent speech~\cite{clark2020speech}.
% Blocks may be perceived as pauses in speech and often occur in the middle of a word. 

% While the speech characteristics of people who stutter vary, there tends to be an increased rate of sound, syllable, and word repetitions, sound prolongations, and/or blocks compared to people who do not stutter. 
% Stuttering is more common and may also be referred to as stammering~\cite{ward2011cluttering}.  
% Speech recognition systems are not tuned to understand these dysfluencies, which means it is an access barrier for modern voice-driven technology, which commonly assumes fluent speech~\cite{clark2020speech}.
% These dysfluencies prevent PWS from 
% This can result in a large psychological toll and is an access barrier for modern voice-driven technology, which commonly assumes fluent speech~\cite{clark2020speech}.

% \note{move} For people with more severe stuttering characteristics, people may interrupt them or not take the extended time to listen \cite{meyers1985interruptions}. 

% For people high rates of dysfluencies these devices simply do not work~\cite{}. 
% With the proliferation of speech-first and screen-free devices like smart speakers and hearables (e.g., Pixel Buds, Apple AirPods) this limits who can use what technology and is a matter of equity. 
% Enabling speech recognition for everyone is fundamentally an access issue, and if consumer devices cannot understand all speech characteristics then it limits who can use what technology. Smart speakers and other screen-free devices like hearables (e.g., Pixel Buds, Apple AirPods) -- which are primarily voice-driven -- have continued to increase in popularity in recent years~\cite{?}. Future devices like AR glasses, which while nascent, are likely to increase usage of speech-driven devices even more. 
% As these and new wearables become com
% It is critical that we understanding these limitations and develop speech technology that works for everyone. 

% The disfluencies caused by stuttering also result in lower automatic speech recognition performance compared to speech without such disfluencies [cites], causing potential issues when people who stutter attempt to use speech input. 

Research on speech technology for PWS has largely focused on technical improvements to automatic speech recognition (ASR) models~\cite{shonibare2022enhancing,Mendelev2020,gondala2021error,mitra2021,HeemanInterSpeech16}, dysfluency detection~\cite{lea2021sep,kourkounakis2020detecting,Mahesha2016,DasNSRE2020}, and dataset development~\cite{FluencyBank,UCLASS,lea2021sep,KSoF}. 
This body of work has largely lacked a human-centered approach to understanding the experiences that PWS have with speech recognition systems~\cite{clark2020speech}, which could in turn inform how to prioritize and advance technical improvements. A recent exception from Bleakley et al.~\cite{bleakley2022exploring} conducted an interview and diary study on the use of voice assistants with 11 PWS. That study provides an initial understanding of user experiences with a voice assistant, identifying issues with the device timing out and that social pressure can influence use. There are still open questions, however, in how PWS more broadly experience speech technologies (i.e., not just voice assistants), the prevalence of accessibility challenges encountered, how these experiences relate to stuttering severity and specific dysfluencies, and how speech recognition systems perform---and can be improved---in the context of these reported challenges.

%What is missing from this body of work, however, is a human-centered and systems-level understanding of the experiences that PWS have when using speech technologies.

In this paper, we report on two studies designed to address these questions of user experience and system performance for both voice assistants (VAs) and dictation: a survey on the use of speech technology with 61 PWS, and an investigation of VA and dictation system performance on speech data collected from a larger set of 91 PWS (53 of whom overlapped with the survey). 
Both studies characterize what attributes, including prevalence of dysfluency types, tend to impact experience and cause recognition errors. Furthermore each study highlights ways in which speech systems could be improved to support the nuanced speech patterns of PWS.
% (e.g., word and phrase repetitions). 
Overall, the findings show that speech technologies work reasonably well for some PWS with mild speech dysfluency patterns, as reflected in both the survey and performance data of those. However, people with more moderate or severe patterns encountered high truncation (e.g., > 20\%) and word error rates (13.6\% to 49.2\%)---which is also reflected by many survey participants. Motivated by these results, we describe and evaluate three technical solutions (two new and one previously published~\cite{mitra2021}) that apply production-oriented improvements to a consumer-grade ASR system. These solutions reduce truncation rates by 79.1\% and improve word error rates in transcribed speech from 25.4\% to 9.9\% for a set of participants with moderate to severe dysfluent speech.
%Many PWS report interest in using speech systems, especially if they worked better, but are frequently cut off while speaking or have their speech incorrectly transcribed. 
%The solutions reduce truncation rates by 79.1\% and improve word error rates for PWS from 25.4\% to 9.9\% using production-oriented  improvements to a consumer-grade ASR system. 

Overall, this paper contributes an understanding of the subjective experiences that PWS have with VAs and dictation across a range of stuttering severities, confirms and reflects those experiences through performance evaluation with a commercial ASR system, and demonstrates the utility of three technical improvements that can be applied with relatively small adaptations to existing systems.
While continued effort is needed to improve these technologies for people with speech disabilities, as frequently noted in popular press (\eg ~\cite{Slate,USAToday,WSJ}), our solutions start to narrow the performance gap for many PWS and potentially improve performance for people with other speech disabilities as well. 


% Furthermore, we 
% Participants across both studies spanned a range of stuttering severity levels, as graded by a speech-language pathologist. 
%The most common concerns from the survey were that VAs cut off speech early and that both VAs and dictation systems incorrectly recognize speech, so we quantify these errors using audio clips from a larger 91-person study in which PWS recorded themselves saying VA- and DS-like phrases. 
% Baseline results with one consumer speech recognition system indicate performance is worse than the general population so we investigate three approaches that greatly improve performance: Endpointer Tuning, ASR Tuning and Dysfluency Refinement. When combined, word error rates are ``good enough'' for a VA to be considered useful, as suggested by \cite{tobin2022personalized}, for 80.5\% of participants.
% \cite{green2021automatic,tobin2022personalized}
% these solutions enable  results for 86.8\% of participants, as defined in Section~\ref{sec:asr_results} using cutoff- and word error rates. 
% While results indicate that performance is far worse than the general population, 
% speech technologies that
% We take these subjective and quantitative learnings and highlight open questions and more targeted avenues of research. 
% These questions go beyond specific technical improvements and can help prioritize future work towards improving the accessibility of speech recognition systems.

% Key findings include: 
% \begin{itemize}
%     \item \note{revise with something that's better representative of our findings} Some people who stutter use speech recognition technology regularly (48\% daily; 66\% monthly), but at lower rates than the general population (57\% daily, 75\% monthly \cite{npr_smart_audio}), and much less so for people with higher (``severe'') dysfluency rates (\note{X}\% daily; \note{X}\% monthly). Of PWS surveyed, 55.7\% would be interested in using these systems more frequently if accuracy was higher. 
%     \item Voice Assistants frequently cut off speech due to blocks or pauses (59.0\% of survey data; 23.5\% of audio clips). By tuning an ASR model on data from PWS, these errors can be reduced to 2.5\% with only a small increase in latency. 
%     \item PWS do not think VAs or DSs understand their speech well enough (55.7\% from survey data), which is corroborated by a average Word Error Rate (WER) of 19.9\%, far above estimates for the general population (?\% \cite{missingcitationgoeeshere}).  Using ASR Tuning and Dysfluency Refinement Voice Assistant performance improves to 9.7\%.
%     \item Using a rich set of dyfluency annotations in our auido clips, we identify important trends in how each dysfluency type impacts WER and cutoff errors (e.g., partial word repetitions and WER have $r=0.78$ Pearson Correlation).
% \end{itemize}


% ASR performance varies depending on types and characterization of dyfluencies, but not strictly clinical severity. Partial word repetitions have the highest correlation with WER ($r=0.8$) whereas blocks and prolongations are more minimal ($r=0.1$ and $r=0.29$). This means someone who only blocks may still be able to use a system effectively, in a way that is less affected by severity.     
% Others generally think they are not useful (9.8\%), require too much physical effort (21.3\%),  or are not interested for social or emotional reasons (36.1\%).

% \todo{consider replacing this with a shorter set of bullets or paragraphs that highlights our three primary contributions with a subset of the numbers below: (1) User perception and interests, (2) Speech collection, assessment, and characterization, (3) Modeling improvements.}
% By combining both survey and audio data we were able to identify the following:
% \begin{itemize}
%     \item Many people who stutter use speech recognition technology regularly (48\% daily; 66\% monthly), but at lower rates than the general population (57\% daily, 75\% monthly \cite{npr_smart_audio}), and less so for people with severe stutters. If these systems were more accurate 55.7\% of PWS surveyed would be interested in using them more frequently. Others generally think they are not useful (9.8\%), require too much physical effort (21.3\%),  or are not interested for social or emotional reasons (36.1\%).
%     \item Voice assistants frequently cut off speech due to blocks or pauses (59.0\% of survey data; 23.5\% of audio clips). We show that by tuning an ASR’s endpointer model on data from PWS, these errors can be reduced by 97.5\% with only a small increase in latency. 
%     \item Generally, PWS do not think VAs or DSs understand their speech well enough (55.7\%) and this is corroborated by an average measured Word Error Rate of 19.9\%, which is far above estimates for the general population (?\% \cite{missingcitationgoeeshere}). 
%     We show that error rates for PWS have improved over time, but not enough for these systems to be considered useful for people with higher rates of dysfluencies. 
%     Our solutions, when combined, can improve VA performance to 9.7\% error (61.1\% improvement).
%     % We describe two approaches applicable, to most consumer ASR systems, that when combined improve performance by .
%     \item ASR performance varies depending on types and characterization of dyfluencies, but not strictly clinical severity. Partial word repetitions have the highest correlation with error rates ($r=0.8$) whereas blocks and prolongations are more minimal ($r=0.1$ and $r=0.29$). This means someone who only blocks may still be able to use a system effectively, in a way that is less affected by severity.     
%     \item Respondents were open to spending time training their own speech models or using VAs with limited commands if that would mean they would work well. There was additional interested in improved wake word detection, punctuation models, and  \todo{X}. 
%     % \note{Something related to future work (personalization) or how is no (or limited) work on invocation models, punctation models, or other support}

%     % \item Most(?) PWS are frequently cut off by speech recognition systems, as evidenced by survey results and from audio recordings. Some people already have work-arounds, like using Hold to Speak. We show optimizing the endpointer on data from PWS prevents people from being cut off 97.5\% of the time while still maintaining responsiveness. 
%     % % to the speech of people who stutter new features analagoud to Siri Pause Time and similar features will mostly fix this issue. Ideally, we could do this without requiring individuals to turn on the feature.  

%     % \item Intent recognition rates for VAs are substantially higher for PWS. By tuning a VA decoder model on PWS ... [Proper nouns are big issue? (how can we verify? maybe look at WER for percent of clips with proper nouns vs without?)]
    
%     % \item There is large interest in using Dictation Systems to text while driving and general interest in using speech for dictating notes or other transcription tasks. However ... and there are emotional effects of seeing large numbers of word repetitions. While performance for many individuals is much worse than general public, we describe heuristics that start to bridge the gap. 
    
%     % \item Future Tech: Most people are generally interested. Many would be willing to train a personalized model or be very interested in a limited VA that only offered a subset of commands. 
% \end{itemize}


% \note{consider rewriting now that we have Zifang's awesome new results} 
% While these technologies have a long way to go for people with speech disabilities, as frequently noted in the popular press (\eg ~\cite{Slate,USAToday,WSJ}), one silver lining is that we show demonstrable improvements in consumer technology over time -- a 32.5\% Word Error Rate (WER) reduction since 2017 with one system -- and a reduction in people being cut off too early when using new accessibility features like Siri Pause Time and Alexa Adaptive Listening. 
% While continued effort is needed to improve these technologies for people with speech disabilities, as frequently noted in popular press (\eg ~\cite{Slate,USAToday,WSJ}), this work adds a more nuanced understanding of some of the community's needs and concerns.
% , and for people who stutter for some of these individuals, as well as solutions that work well for some. 
% Our technical solutions do not require vast quantities of data and could be readily incorporated into production speech systems.
% one silver lining is that we show demonstrable improvements in consumer technology over time -- a 32.5\% Word Error Rate (WER) reduction since 2017 with one system -- and a reduction in people being cut off too early when using new accessibility features like Siri Pause Time and Alexa Adaptive Listening. 
% If ideas described throughout this paper are implemented then we can start to close the performance gap for many people who stutter and potentially improve performance for people with other speech disabilities as well. 
% Our technical solutions do not require vast quantities of data, could be readily incorporated into production speech systems, and start to narrow the performance gap for many people who stutter and potentially improve performance for people with other speech disabilities as well. 


% We think that the framing of these systems at the systems-level can also help prioritize future work towards improving the accessibility of speech recognition systems.

% These questions go beyond specific technical improvements and can 

% Furthermore, the methodologies used may be 


% As such, we gathered feedback from 62 individuals
% in the stuttering community 
% covering how they use speech technology, error modes, and their interests in current or future speech technologies. 
% to better understand their experience and interest levels in current and future technology. We 
% We then describe the findings from a 62 person survey from people who stutter covering how they use speech technology, error modes, and their interests in future speech technologies. 
% Lastly, we assess speech recognition performance on audio recordings from a 91 person user study with many of the same participants, and investigate baseline improvements to each part of the the voice assistant and dictation pipelines. 


% and were able to relate subjective experiences to actual ASR word error rates, command recognition performance, and ultimately the ability to do daily tasks like send a text message while driving a car.
% Speech technologies, such as Voice Assistants and Dictation Systems, are more than just a set of ASR models

% , and we seek to understand holistically where they fail and how they can be improved. 

% how people who stutter feel about existing speech-based interactions and what are their experiences and interest levels. 
% We investigate how subjective experiences relate to actual ASR word error rates, command recognition performance, and ultimately the ability to do daily tasks like send a text message while driving a car.


% , which we attempt to divulge in this paper, is that there is more nuance. We describe when they do work, attempts within industry to improve performance, and promising paths forward to make them more accessible. 
% While they are far from perfect, one silver lining, which we attempt to divulge in this paper, is that there is more nuance. We describe when they do work, attempts within industry to improve performance, and promising paths forward to make them more accessible. 
% If you are to take articles on stuttering from the popular press (\eg ~\cite{Slate,WSJ,?}) at face value it would appear that speech systems completely fail for people who stutter or have other speech disabilities. 
% While they are far from perfect, one silver lining, which we attempt to divulge in this paper, is that there is more nuance. We describe when they do work, attempts within industry to improve performance, and promising paths forward to make them more accessible. 

% \todo{explicitly mention different parts of speech system in intro? or wait til Section 2}

==> CHI2023 Stuttering/sections/2-relatedwork-old.tex <==
\section{Background \& Related Work}
\todo{swap sections; add some more details to ASR; move ASR related work to ASR background}

% \subsection{Background on Stuttering \todo{move or incorporate elsewhere}} 


% Individuals may develop reactions to speaking in various situations leading to avoidance of target words, sounds, or speaking situations and observable escape behaviors such as foot stomping or eye blinking. 






% Stuttering and cluttering are types of fluency disorders, defined by an interruption in the flow or fluidity of connected speech.  Stuttering is more common and may also be referred to as stammering~\cite{ward2011cluttering}.  Stuttering is a breakdown in speech fluency that can affect the rate and flow of speech and can include specific dysfluency types, such as sound (``p-p-pop'') and syllable repetitions (``be-be-become''), word repetitions (``mom, mom, mom``), sound prolongations (``mmmmmom''), and silent or audible blocks (inability to initiate target sound) \cite{sander1963frequency, SSI}. Frequent interjections (``um'', ``eh'') are also common.  

% PWS typically cannot control when their stuttering will occur and cannot control how people or technology perceive and respond to their dysfluencies. 
% The setting or environment, current mood/stress level, communication partners, or other variables can impact stuttering.  Some people stutter frequently when in a group but not when on their own \cite{tichenor2021variability}. Some people stutter more when in front of a smart device because of ``pressure to perform.'' 
% Individuals may develop reactions to speaking in various situations leading to avoidance of target words, sounds, or speaking situations and observable escape behaviors such as foot stomping or eye blinking.  
% Over time, a PWS may also experience negative psychological outcomes such as social anxiety, low self-esteem, and negative feelings about communication~\cite{boyle2015identifying}. This can be a cycle as increased anxiety may then lead to an increase in producing stutter events.  
% Stuttering may be developmental, neurogenic, or psychogenic \cite{roth1989clinical, seery2005differential}.  

% PWS vary in terms of how many and what types of dysfluencies they produce. 
% The frequency of dysfluencies, duration of dysfluencies, physical concomitants (i.e., stomping a foot, moving hands), and the impacts that stuttering has on participation in communication across settings varies significantly across individuals \cite{tichenor2021variability}. These overt cues are used in clinical settings to assess severity and changes over time~\cite{SSI,yaruss2006overall}. 
% In this work we used severity to recruit participants, but ultimately find a more nuanced understanding of the rates and characteristics of each dysfluency type and their impact on speech recognition technology.  


% Multiple factors are considered when clinically assessing stuttering severity including . 
% We are working to improve ASR so that PWS can be successful and more confident with use of speech recognition.   

% [\textbf{TODO}\textbf{: change citations and put in bibliography]}

% @article{boyle2015identifying,
%   title={Identifying correlates of self-stigma in adults who stutter: Further establishing the construct validity of the Self-Stigma of Stuttering Scale (4S)},
%   author={Boyle, Michael P},
%   journal={Journal of Fluency Disorders},
%   volume={43},
%   pages={17--27},
%   year={2015},
%   publisher={Elsevier}
  
%   @book{ward2017stuttering,
%   title={Stuttering and cluttering: frameworks for understanding and treatment},
%   author={Ward, David},
%   year={2017},
%   publisher={Psychology Press}
% }
  
%   @article{yaruss2006overall,
%   title={Overall Assessment of the Speaker's Experience of Stuttering (OASES): Documenting multiple outcomes in stuttering treatment},
%   author={Yaruss, J Scott and Quesal, Robert W},
%   journal={Journal of fluency disorders},
%   volume={31},
%   number={2},
%   pages={90--115},
%   year={2006},
%   publisher={Elsevier}
% }
% Riper~\cite{VanRiper1982}, SSI-4~\cite{SSI}, Andrew \& Harris~\cite{andrews1964syndrome}, Time-interval measurement~\cite{valente2015event,ingham1993time}.




% ------------------------------------------------------------------------------------

\subsection{Related Work} %HCI \& Technical Literature}
A wide range of people with disabilities use voice interaction which enables people with motor disabilities to control computing devices with speech commands (e.g.,~\cite{zhong2014justspeak, corbett2016can}). It is also an inherently accessible input modality for many blind and low vision users (e.g., ~\cite{pradhan2018accessibility, abdolrahmani2018siri}). However, this work often assumes that speech input itself is accessible.

% Focusing on studies with users who have atypical speech, 
Researchers have captured speech input challenges encountered by people with dysarthria~\cite{ballati2018assessing,projecteuphonia}, deaf or hard of hearing people~\cite{fok2018towards}, and people with aphasia~\cite{roper2019speech}. 
For stuttering specifically, there has been relatively little human-centered work~\cite{clark2020speech}. A recent exception comes from Bleakley et al.~\cite{bleakley2022exploring}, who report on interviews and a three-week diary study of smart speaker use at home with 11 PWS. 
%Usage followed patterns typical of the general population (e.g., music and information queries were most common). 
While participants had ``some success’’ in using the device, challenges included the device timing out, social pressure when using the device around other people, and difficulty with specific sounds (especially that could interfere with the wake word, i.e., ``OK Google’’). Participants reported repeating and reformulating utterances to overcome these issues. While this study provides an initial understanding of how PWS use voice assistants, it does not report the stuttering severity of the participants and does not provide an objective assessment indicating how well the smart speakers recognized their speech. In contrast, our study examines speech input technology more broadly (e.g., including dictation), and includes both quantitative subjective data from a larger sample of (n=61) PWS and system performance on stuttered speech samples collected from (n=91) PWS. 

% Beyond Bleakley et al.'s study on speech input accessibility and stuttering~\cite{bleakley2022exploring}, 
A few other human-centered projects have looked at supporting speech therapy for PWS and at managing stuttering in everyday life. Demarin et al.~\cite{demarin2015impact} and Madeira et al.~\cite{madeira2013building} both present apps to record stuttering experiences with the goal of increasing awareness and informing therapy decisions; small user evaluations included 2 and 5 PWS, respectively.
Focused on managing speaking situations, Fluent~\cite{ghai2021fluent} supports people in writing scripts that they will be more likely to read aloud fluently. The tool uses active learning to identify words that the user is likely to encounter issues with, and suggests alternative words that may be easier to speak; no user study has been reported. Finally, McNaney et al.~\cite{mcnaney2018stammerapp} employed a multi-stakeholder co-design process to design StammerApp, a mobile app that allows users to set goals, practice, and reflect on their experiences in especially challenging situations. While the project did not focus on speech input, it provides a qualitative understanding of a total of 39 participants’ experiences with stammering, including specific challenges (e.g., talking on the phone), and a general desire to be able to ``stammer openly and feel more confident and relaxed with their own voice''. Ultimately, our goal is for PWS to have this freedom and confidence when interacting not only with other people, but with speech input technology as well.


Technical work on improving speech assistants for PWS has focused on Automatic Speech Recognition (ASR) models~\cite{shonibare2022enhancing,Mendelev2020,gondala2021error,mitra2021,Tripathi2018,Tripathi2020,HeemanInterSpeech16}, stuttering detection~\cite{LeaStutterDetection2021}, dysfluency detection or classification~\cite{lea2021sep,kourkounakis2020detecting,Mahesha2016,DasNSRE2020,riad2020identification}, clinical assessment~\cite{BayerlTSD2020}, and dataset development~\cite{FluencyBank,UCLASS,lea2021sep,KSoF}.
% Much of this work has centered on dysfluency detection either as a standalone task or as part of an ASR system. 
% Three ASR-oriented approaches are as follows. 
Shonibare \etal \cite{shonibare2022enhancing} and Mendelev \etal  \cite{Mendelev2020} investigate training end-to-end RNN-T ASR models on speech from PWS. 
Shonibare \etal\ introduces a detect-then-pass approach that incorporates a dysfluency detector where audio frames with dysfluencies are ignored entirely by the RNN-T decoder. 
Examples in the paper demonstrate how this can be used to ignore some partial-word repetitions and blocks.
% The temporal context is very short (100 ms) so it is unlikely to generalize to whole word or phrase repetitions or to inaudible blocks mid-word. 
Mitra \etal \cite{mitra2021} describes a fine-tuning approach for Voice Assistant tasks that can be applied on top of existing ASR models, which does not require as much data as end-to-end solutions.
% which may be production-oriented 
% It is challenging to get large amounts of stuttered speech data and moreover dysfluency detection labels, so investigated 
% optimizing a small set of ASR decoder parameters on stuttered speech, such that the system is biases towards more common phrases and shorter phrases without repetitions.
%  for Voice Assistant task
Their system optimizes a small set of ASR decoder parameters on stuttered speech, such that the system is biased towards more common phrases and shorter phrases that remove sound and partial-word repetitions. 
% and Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly}
Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly} focused on stuttered speech from youths and incorporates the structure of repetitions and other dyfluencies into an augmented language model that is better at including dysfluencies in a transcription. 
% \note{[mention Mendelev which just trained an RNN-T model with a tiny amount of stuttered speech and tries replacing partial-word annotations with another symbol. ] [Neither paper uses absolute WER! only relative. ]} 
Efforts from Project Euphonia~\cite{projecteuphonia}, the largest atypical speech project to date, have included data from PWS but it has not been a core focus in publications.
% \todo{mention limitations and connections to our work}

\note{need to figure out whether to keep this content or not}Speech has also been explored as a form of input for augmentative and alternative communication (AAC) systems, which are traditionally controlled through touch, gaze or switch input. 
The VIVOCA project, for example, recognizes spoken input from users with atypical speech by training a personalized limited vocabulary speech recognition model that can activate pre-defined synthesized speech output~\cite{hawley2012voice}. Speech recognition has also been employed for speech therapy goals---including using both off-the-shelf systems such as smart speakers (e.g., \cite{smith2021smart}), and custom-designed games to increase enjoyment of speech therapy exercises, such as Apraxia World~\cite{hair2018apraxia}.


% There has been significant interest 
% [Project Euphonia has stuttering data as well but I can't remember seeing anything stuttering-specific that they've worked on.]



%%scratch (could remove)
% \subsection{Voice Assistant Usage}


% ------------------------------------------------------------------------------------------------------------------
\subsection{Background on Speech Recognition Systems}
% \todo{Refactor and trim this section.}

Our goal is not only to understand perceptions of speech technology for PWS, but to achieve a deeper understanding where existing pipelines break and technical avenues for improvement. 
% In this paper, we focus on two applications: . 
In this section we describe common pipelines for Voice Assistants and Dictation Systems and in Section~\ref{sec:asr_results} evaluate constituent models.
% \note{Should we mention why VA and DS versus any other tasks?}
% While these two systems are similar, their use cases and limitations 

% We chose VAs because they are ubiquitous in smart phones and speakers and can be an important access tool, especially for people with motor disabilities. 

\note{An attempt to describe ASR before we talk about VAs and DSs.} 

Voice assistants and dictation systems rely on automatic speech recognition (ASR) technology. On a high level, ASR uses machine learning algorithms to convert spoken language to text. Traditionally people use a Hybrid Approach to build an ASR~\cite{KelseyFoster}. It usually consists of a lexicon model that provides pronunciation knowledge, an acoustic model that models acoustic patterns, and a language model that gives information about word sequence likelihood, and finally a decoder that utilizes all above information to produce a transcription~\cite{gondala2021error}. With the emerging of deep neural networks recent years, components such as acoustic model in the hybird ASR adopts deep neural networks to improve ASR performance~\cite{AlexGraves} while an end-to-end deep learning approach of building ASR system sprung. An end-to-end ASR directly maps a sequence of input acoustic features into a sequence of words~\cite{AlexGraves}, instead of having separately trained acoustic, pronunciation and language model components, 

Though end-to-end systems reduce efforts needed from domain experts (for example for lexicon expert phoneticians need to handcraft a phoneme set for each language) and tends to outperform hybird models~\cite{AwniHannun}, hybird ASRs are still dominantly used in commercial VAs and DSs ~\cite{KelseyFoster}.
% though many companies are transitioning to an end-to-end approach. 

% TO be cited:
% Deep Speech: Scaling up end-to-end speech recognition. Awni Hannun
% Towards End-to-End Speech Recognition with Recurrent Neural Networks, Alex Graves
% Need to cite this properly: https://www.assemblyai.com/blog/what-is-asr/, Kelsey Foster

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6 \paperwidth]{figures/VA_Illustration.png}
    \caption{Simplified Workflow and Components of a Voice Assistant. Figure adapted from \cite{ranantha2020intent} 
    % \todo{to be updated}\todo{replace user head. I think this was taken from some random website based on a reverse image search}  
    }
    \label{fig:VA Illustration}
\end{figure}
% \note{colin: (1) Can "Behind the Scene" be renamed to "Voice Assistant Models, and (2) "When do I endpoint" be changed from a thought bubble to something else? It is a model... and thus there should be a blue box, but it's iterative so I don't know the best way to display with this graphic.}
\textbf{Voice Assistants} (e.g., Amazon Alexa, Apple Siri, and Google Assistant) listen for spoken questions or commands. For example, ``What is the weather?'' or ``Set a timer for five minutes.'' 
% They usually have a spoken response but some can also show visual information. 
A typical user flow is as follows and as shown in Figure~\ref{fig:VA Illustration} . 
A user may start by using an \textit{wake word}, such as saying ``Alexa'', ``Hey Siri'', or ``OK Google,'' to initiate a query. This may also be called \textit{Invocation}. 
% On most smart devices there is an always-running invocation model that attempts to recognize one of these phrases. 
They then start to vocalize their command. 
% \note{we usually call this payload... I see it mentioned below in text only so not sure we want to introduce term: trigger=wake-word + command=payload]}
% , such as ``What is the weather?'' 
As the user speaks, an \textit{ASR} model takes this speech and transcribes the words being said.
% , typically verbatim. 
Meanwhile the system tries to automatically detect when the user has finished their phrase using an \textit{endpointer} model. This can also be referred to as an end-of-speech detection model. 
% , which uses cues like how much time has elapsed since the last vocalization to know when to perform recognition.
Finally, a \textit{Natural Language Understanding (NLU)} model takes the predicted phrase and metadata output from the ASR and identifies the user's intent and how to respond. 
Based on the user's query, the VA may respond with information, perform a command, ask the user a follow-up question, or notify the user that the query could not be understood. 
% Note that a streaming version of the ASR model may be run while the user is still speaking, and the prediction may be displayed on-screen so the user gets feedback on what the system thinks the person is saying.

% No less than three models are run on this speech. An \textit{endpointer} model computes the likelihood that a person is finished speaking so the system knows when to respond. An \textit{Automatic Speech Recognition (ASR)} model takes the speech and attempts to identify the words being said. Finally, a \textit{Natural Language Understanding (NLU)} model takes the predicted phrase and metadata output from the ASR and identifies the users intent and how to respond. Based on the query, the VA may respond with information, perform a command, ask the user a followup question, or notify the user that the query could not be understood. Note that a streaming version of the ASR model may be run while the user is still speaking, and the prediction may be displayed on-screen so the user gets feedback on what the system thinks the person is saying. 

There are alternative ways of interacting with a Voice Assistant. Instead of using a speech-based invocation mechanism on a phone or tablet, you may hold down a button on the side of the device (``Hold to Speak'' on iOS) or squeeze the side of the phone (some Android devices). 
VAs can also be invoked using accessibility features such as Accessibility Menu on Android or Assistive Touch on iOS.
Instead of speaking, a user can type in a command using a keyboard using features such as ``Type with Alexa'' or ``Type to Siri''. This bypasses the ASR component and may directly process the input text through NLU. 



% This model may take multiple cues such as how much silence has elapsed since the last word, what was the last word that was said, and how many words have been said  to identify when someone is finished speaking. 
% Typically this is computed at a high sample rate (e.g., 100 hz)
Endpointers are optimized to balance the trade-off between cutting someone off too early and having a long delay after their speech, and rely on cues such as how much silence has elapsed since the last word. These are largely optimized using data from people who do not stutter and tuned to respond to the user as quickly as possible. It is very common for the endpointer model to cut PWS off before they are done speaking especially during blocks, where there may be a long pause or gasp, or even partial word repetitions, where the vocalization may be indecipherable. 

% https://www.forbes.com/sites/stevenaquino/2021/10/05/exclusive-amazon-adds-new-speech-setting-to-alexa-app-to-help-stutterers-finish-commands-queries/?sh=3380f1542b34
% This Alexa news may serve as a support for being cutoff.

ASR models are less certain on dysfluent speech with sound, syllable, or partial word repetitions and wrongfully detect words that are whole word repetitions and interjections, even if the user does not intend to say them.
%\note{pg: I think here we need a better explanation: Acoustics attempt to be faithful to the sound, so what you said is right, but also suffer when the sounds are not complete words. Language models on the other hand try to use predictability, which makes repetitions unlikely so they tend to substitute with more likely/similarly sounding words...}
For a VA, it may be inconsequential if someone stutters on unimportant words, but is fluent for important ones. The NLU may implicitly identify which words are important or use additional context to route a transcription with dysfluencies to the correct task. 
% For non-consequential words NLU models may 
% Word or phrase repetitions may not be problematic because of the fuzzy match, and errors on less important 
% Because of this fuzzy match, repetitions may not be very problematic. , however substitutions. 
%\note{pg:Above paragraph is confusing as to the point is trying to make, and doesn't make it accurately}

% \textbf{Dictation Systems}
\textbf{Dictation Systems} provide an alternative to using a keyboard to enter text and take a user's speech and convert to text for any use, such as composing messages, notes, or emails. 
% \note{pg: this sentence is unnecessary} 
%A common use case it to create a text with your voice while in a car. 
% To contrast with Voice Assistants, 
Dictation typically does not rely on a wake word; the user may initiate manually with a button click. 
Similarly, there is often no endpointer, as the user may push a button once they finish talking and users are often dictating multiple sentences at a time. 
While VAs and DS may rely on the same ASR system, a VAs model may be biased towards a smaller set of assistant commands, whereas the DS may be biased towards free speech from arbitrary topics. 
Dictation may have additional models for \textit{punctuation} and \textit{revisions}. The former attempts to add grammatical structure to spoken words, like adding commas and periods, and may do so using a combinations of linguistic and prosodic cues (i.e., pausing between sentences).
% (i.e., via a language model) or cues from prosody in the speech . 
A revision model may identify words or phrases for which the ASR has low confidence, highlight them for the user on-screen, and offer suggestions for replacement. 
In contrast, VAs may rely on speech communication to confirm requests in cases of uncertainty, either due to low recognition confidence (did user say ``set'' or ``said'') or conceptual ambiguity (e.g., is the alarm request for a.m. or p.m.?).
% Invocation of this system varies based on usage: in a text message or notes app you may click on a microphone button to initiate or in a car you may initiate a text with a VA query which then prompts the user for the body of the text. 
% In the car scenario there may be an endpointing model, but in many other situations the users presses a button once they are done composing a message. 
% A real-time/streaming version of an ASR model is often used, especially for long-form text entry like in notes or email, so the user sees what is being written as they speak. 

% Often the ASR transcription is used verbatim, but an additional \textit{revision} models may be used to overlay potential errors within the text. For example, words that have low ASR confidence may be underlined, and if you click on-screen, there are options to swap out the word with other options. These revisions systems may also include grammar checkers. 

% \textbf{Implications of Dysfluencies.}
% \todo{consider integrating this subsection into the previous section and maybe Section 4 (ASR)}
% \hfill\\
% Endpointer “model-feature-list": "num-trailing-sil,end-of-sentence,num-of-words,pause-counts,silence-posterior",
% https://compass.scv.apple.com/confluence/display/SiriPerception/Endpoint+Feature
% \textit{Endpointer}: 
% \note{mention implications on invocation and punctuations models?}

% For an overview


% \note{move} The definitive ASR evaluation metric is Word Error Rate (WER). In some papers on stuttering, there are separate metrics for intended speech and articulated speech and correspondingly metrics iWER and aWER. 
% Intended speech has all dysfluencies removed and articulated speech retains all spoken words included repetitions.  
% For PWS, partial-word repetitions and blocks tend to cause word substitutions and increase both iWER and aWER. 
% Word and phrase repetitions increase iWER but not aWER.
% Errors in the acoustic model may be caused by blocks, sound repetitions, or partial words. 
% Errors in the language model may be caused by repetitions. 
% And if the number of candidates in the Beam Search decoder is too small it may not have enough memory to smooth over partial word repetitions. 

% For Voice Assistants, an \textit{NLU} model routes a transcription to the correct VA command. 
% For example ``What what is the weather?'' and ``What is the weather?'' would map to the same ``weather'' action. 
% This can mask transcription errors in the ASR by doing selective word finding.
% In this work we look at the use of intents~\cite{GoogleConversationalAI} where an intent may be a slotted command like ``Search for the weather in [city] on [date]'' where ``[city]'' and ``[date]'' are filled in by the user. 
% We compute results for intent recognition using the ML-based NLU system described in~\cite{chen2019active}.
% These are used as an upper bound on final accuracy or ``usefulness'' of a VA system. 


% A commercial Natural Language Understanding \textit{(NLU)} model may route ASR predictions to Voice Assistant commands using \textit{domains}, \textit{intents}, and \textit{actions}~\cite{chen2019active}. A domain may be a category of commands such as ``weather'' or ``timers.'' 
% The action would be responding to the user with the weather on that day and in that city. 
% There may be multiple different phrases that can lead to the same intent and action. 
% Typically, there is a machine learning model that attempt to identify the domain and parameter inputs. This model may also use outside information, like contacts on your phone or your GPS location to determine the most likely response. 
% In traditional NLU models, the system must simply identify critical words
% , but there is more flexibility than in Dictation. 
% For example, there is often a fuzzy search which improves performance on proper nouns., \eg ``New New York City'' translates to ``New York City.'' 
% In addition, repetitions or inaccurate prediction of unimportant words may be skipped by the model and result in the same intent, such as ``what is the weather'' and ``what in is what is the weather.``
% \todo{turn google link into citation. do they have a paper describing?} \url{https://developers.google.com/assistant/conversational/overview}.
% Word or phrase repetitions may not be problematic because of the fuzzy match, and errors on less important 
% Because of this fuzzy match, repetitions may not be very problematic. , however substitutions. 

% \todo{revision model?}
% \todo{Should we mention other models like speaker recognition or Personalized HS?}

% \subsubsection{Impact of Stuttering Events on Speech Systems}



% [issues: repetitions and LM; partial word reps and beam search; sound reps and prolongations with AM; blocks and endpointing, etc.]





% ---------------------------------------------------------------
% \subsection{Related Work}

% \subsection{Technical Literature \note{integrate with Speech Tech section?}}

% \todo{THIS SECTION IS COPIED FROM MATERIAL IN OUR PREVIOUS PAPERS; COLIN WILL CLEAN UP/CONDENSE/ETC}

% Technical work on improving speech assistants for PWS has focused on ASR models~\cite{shonibare2022enhancing,Mendelev2020,gondala2021error,mitra21,Tripathi2018,Tripathi2020,HeemanInterSpeech16}, stuttering detection~\cite{LeaStutterDetection2021}, dysfluency detection or classification~\cite{lea2021sep,kourkounakis2020detecting,Mahesha2016,DasNSRE2020,riad2020identification}, clinical assessment~\cite{BayerlTSD2020}, and dataset development~\cite{FluencyBank,UCLASS,lea2021sep,KSoF}.

% Much of this work has centered on dysfluency detection either as a standalone task or as part of an ASR system. 
% Shonibare \etal \cite{shonibare2022enhancing} and Mendelev \etal  \cite{Mendelev2020} incorporate dysfluency detectors as part of training end-to-end RNN-T ASR models. Shonibare \etal introduces a detect-then-pass approach where audio frames with detected dysfluencies are ignored entirely by the RNN-T decoder. 
% Examples in the paper demonstrate how this can be used to ignore some partial-word repetitions and blocks.
% % The temporal context is very short (100 ms) so it is unlikely to generalize to whole word or phrase repetitions or to inaudible blocks mid-word. 
% Mitra \etal \cite{mitra2021} takes a production-oriented approach that can be applied on top of a pre-trained ASR model. 
% % It is challenging to get large amounts of stuttered speech data and moreover dysfluency detection labels, so investigated 
% % optimizing a small set of ASR decoder parameters on stuttered speech, such that the system is biases towards more common phrases and shorter phrases without repetitions.
% They show that for Voice Assistant task you can optimize a small set of ASR decoder parameters on stuttered speech, such that the system is biased towards more common phrases and shorter phrases that remove sound and partial-word repetitions. 
% % and Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly}
% Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly} focused on stuttered speech from kids that incorporates the structure of repetitions and other dyfluencies into an augmented language model that is better at including dysfluencies in a transcription. 
% % \note{[mention Mendelev which just trained an RNN-T model with a tiny amount of stuttered speech and tries replacing partial-word annotations with another symbol. ] [Neither paper uses absolute WER! only relative. ]} 
% Efforts from Project Euphonia~\cite{projecteuphonia}, the largest atypical speech project to date, have included data from people who stutter but it has not been a core focus in publications. 
% % There has been significant interest 
% % [Project Euphonia has stuttering data as well but I can't remember seeing anything stuttering-specific that they've worked on.]

% \todo{sort these}
% * "Systematic review ... detecting developmental stuttering." \cite{barrett2022systematic}. 
% * Machine learning for stuttering identification: Review \cite{sheikh2021machine}
% * Stuttering detection: Introducing ECAPA-TDNN and Wav2Vec2. 0 embeddings to stuttering detection. arXiv'22
% * “Identification of primary and collateral tracks in stuttered speech,” \cite{riad2020identification}
% * Automatic recognition of children’s read speech for stuttering application,” vol. WOCCI, 2017. \cite{AlharbiWOCCI17}
% * Intelligent processing of stuttered speech \cite{Czyzewski2003}
% * A lightly supervised approach \cite{alharbi2018lightly, AlharbiWOCCI17} 

% Stuttering Challenge (2022): \cite{schuller2022acm} uses the KSoF dataset. 

% KSoF: The Kassel State of Fluency Dataset--A Therapy Centered Dataset of Stuttering
% * " the ability to detect stuttering events and modifications in speech could help PWSs and speech pathologists to track the level of fluency"
% * " 5500 clips of PWSs. The clips were labeled with six stuttering-related event types: blocks, prolongations, sound repetitions, word repetitions, interjections, and – specific to therapy – speech modifications."



% Prolongations, or extended sounds, have been detected using short-window autocorrelations [16] and low-level acoustic models [10]. Word/phrase repetitions, if they are well articulated, are easily detected using LM- based approaches [19], with the caveat that single-syllable words such as in the phrase “I-I-I am” will often be smoothed into “I am” due to the underlying acoustic model and phrases like “I am [am]” may be pruned because the LM has never seen the word “am” repeated before. This is fine for speech recognition but bad for stuttering event analysis. Arjun et al. [16] addressed this repetition problem by segment- ing pairs of subsequent words and analyzing correlations in their spectral features. Interjections, including “um”, “uh”, “you know” and other filler words, are perhaps the easiest type to recognize with a language model if well articulated. Blocks, or gasps/pauses typically within or between words, are difficult to detect because the gasp for breath or pause is often inaudible. Sound repetitions are also challenging because syllables may vary in duration, count, style, and articulation (e.g.,“[moh-muh-mm]-ommy”).
% Efforts in HCI have sought out an understanding of speech recognition needs for users with speech impairments, which is critical for framing problems like ours [1, 2, 22].





==> CHI2023 Stuttering/sections/2-relatedwork.tex <==
\section{Background \& Related Work}

% ------------------------------------------------------------------------------------------------------------------
\subsection{Speech Recognition Systems}
\label{sec:rw-speechrecsystems}

% In this paper, we focus on two applications: . 
In this section, we describe common pipelines for Voice Assistants and Dictation Systems, to build an understanding of how people use them and how the underlying models work. 
% Our goal is not only to understand perceptions of speech technology for PWS, but to achieve a deeper understanding where existing pipelines break and technical avenues for improvement. 
In Section~\ref{sec:survey_results} we describe how PWS use and perceive these systems and in Section~\ref{sec:asr_results} we demonstrate how dysfluencies impact performance of constituent models.
% \note{Should we mention why VA and DS versus any other tasks?}
% While these two systems are similar, their use cases and limitations 
% We chose VAs because they are ubiquitous in smart phones and speakers and can be an important access tool, especially for people with motor disabilities. 

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8 \paperwidth]{figures/Updated_VA_Workflow2.png}
    \caption{Simplified workflow and components of a voice assistant. Figure adapted from \cite{ranantha2020intent}. 
    In this work we seek to understand performance on speech from people who stutter.
    % , with emphasis on the endpointer and ASR models. 
    In Section~\ref{sec:asr_results}  we report on baseline performance of the endpointer and ASR models for dysfluency speech, and investigate three interventions to better support PWS at different points in the workflow: (1) endpointer tuning; (2) ASR decoder tuning; and (3) refinement of dysfluencies in the transcribed ASR output.
    }
    % \note{Copied Leah's caption text from a screenshot she shared: A voice assistant workflow with separate endpointer and ASR components; 
    % in contrast a typical dictation workflow only includes the ASR component shown here, and the user often signals the beginning and end of dictation through an explicit action like a button press or other command. 
    % In section 4 we report on baseline performance of the endpointer and ASR models for dysfluency speech, and investigate three interventions to better support PWS at different points in the workflow: (1) endpointer tuning; (2) ASR decoder tuning; and (3) refinement of dysfluencies in the transcribed ASR output.}
    % } 
    \label{fig:VA Illustration}
    \Description{A pipeline with each element of a voice assistant. A user speaks into a device to invoke the VA, an endpointer model monitors that speech and decides when to clip the audio into an utterance. 
    %\note{The description seems faithful to the figure but not so accurate to the model. Can we say something like: an endpointer model monitors that speech and decides when to clip the utterance.} 
    The ASR model is run on that utterance and outputs a text string, the NLU model takes the transcribed string and outputs the user intent, and a decision making model determines how the intent translates to a system response which is displayed to the user. }
\end{figure*}
% \note{colin: (1) Can "Behind the Scene" be renamed to "Voice Assistant Models, and (2) "When do I endpoint" be changed from a thought bubble to something else? It is a model... and thus there should be a blue box, but it's iterative so I don't know the best way to display with this graphic.}


\subsubsection{Overview of Speech Recognition Systems}

\paragraph{Voice Assistants (e.g., Amazon Alexa, Apple Siri, and Google Assistant)} These systems listen for spoken questions or commands. For example, ``What is the weather?'' or ``Set a timer for five minutes.'' 
% They usually have a spoken response but some can also show visual information. 
A typical user flow is as follows, where a simplified view is shown in Figure~\ref{fig:VA Illustration}. 
A user may initiate a query by saying a \textit{wake word}, such as ``Alexa'', ``Hey Siri'', or ``OK Google.'' This may also be called \textit{invocation}. 
% On most smart devices there is an always-running invocation model that attempts to recognize one of these phrases. 
They then start vocalizing their command. 
% \note{we usually call this payload... I see it mentioned below in text only so not sure we want to introduce term: trigger=wake-word + command=payload]}
% , such as ``What is the weather?'' 
As the user speaks, an \textit{ASR} model starts to transcribe their words and simultaneously an \textit{endpointer} model---also called end-of-speech detector---detects whether the user has finished speaking.\footnote{For simplicity, Figure \ref{fig:VA Illustration} shows the endpointer and ASR in sequence. In practice, endpointers range from being independent of an ASR \cite{Maas2018DNNEndpointer} to fully integrated \cite{li2020RNNTEndpointer}.}
% , typically verbatim. 
% Simultaneously the system  using an . This can also be referred to as an . 
% , which uses cues like how much time has elapsed since the last vocalization to know when to perform recognition.
A \textit{Natural Language Understanding (NLU)} model then takes the transcribed phrase and any metadata from the ASR and identifies the user's intent, which is then sent to the \textit{Decision Making} component to perform the appropriate action. 
Based on the user's query, the VA may respond with information, perform a command, ask the user a follow-up question (i.e., ``is the alarm request for AM or PM''), or notify the user that the query could not be understood. 
% In contrast, VAs rely on speech communication to confirm requests in cases of uncertainty, either due to low recognition confidence (did user say ``set'' or ``said'') or conceptual ambiguity (e.g., is the alarm request for am or pm?).

% Note that a streaming version of the ASR model may be run while the user is still speaking, and the prediction may be displayed on-screen so the user gets feedback on what the system thinks the person is saying.

% No less than three models are run on this speech. An \textit{endpointer} model computes the likelihood that a person is finished speaking so the system knows when to respond. An \textit{Automatic Speech Recognition (ASR)} model takes the speech and attempts to identify the words being said. Finally, a \textit{Natural Language Understanding (NLU)} model takes the predicted phrase and metadata output from the ASR and identifies the users intent and how to respond. Based on the query, the VA may respond with information, perform a command, ask the user a followup question, or notify the user that the query could not be understood. Note that a streaming version of the ASR model may be run while the user is still speaking, and the prediction may be displayed on-screen so the user gets feedback on what the system thinks the person is saying. 

There are alternative ways of interacting with a VA. Instead of using a speech-based invocation mechanism on a phone or tablet, a user may hold down a button on the side of the device (``Hold to Speak'' on iOS) or squeeze the side of the phone (some Android devices). 
VAs can also be invoked using accessibility features such as Accessibility Menu on Android or Assistive Touch on iOS.
Instead of speaking, a user can type a command with a keyboard using ``Type with Alexa'' or ``Type to Siri.'' This bypasses the ASR component and may directly process the input text through NLU. 

\paragraph{Dictation Systems} These systems provide an alternative to using a keyboard by converting a user's speech to text for tasks such as composing text messages, notes, or emails. 
A common use case is to verbalize a text while in a car. 
% To contrast with Voice Assistants, 
Typically, a user starts dictation by manually clicking a button on a device, instead of via a wake word, and they finish by manually clicking a button again, instead of relying on an endpointer.   
% Dictation typically does not rely on a wake word; the user may initiate manually with a button click. 
% Similarly, there is often no endpointer, as the user may push a button once they finish talking and users are often dictating multiple sentences at a time. 
An ASR model may transcribe their speech in real-time and visualize the text if the device has a screen. 
A \textit{punctuation} model may add grammatical structure to spoken words, like adding commas and periods.
% , and may do so using a combinations of linguistic and prosodic cues (i.e., pausing between sentences) \note{cite}.
% (i.e., via a language model) or cues from prosody in the speech . 
Finally, if the ASR model yields low confidence in a predicted word, this word may be highlighted on screen along with suggestions for replacement. 
A user can then manually revise their statement or click on low confidence words for suggestions. 

% A revision model may identify words or phrases for which the ASR has low confidence, 
% Invocation of this system varies based on usage: in a text message or notes app you may click on a microphone button to initiate or in a car you may initiate a text with a VA query which then prompts the user for the body of the text. 
% In the car scenario there may be an endpointing model, but in many other situations the users presses a button once they are done composing a message. 
% A real-time/streaming version of an ASR model is often used, especially for long-form text entry like in notes or email, so the user sees what is being written as they speak. 

% Often the ASR transcription is used verbatim, but an additional \textit{revision} models may be used to overlay potential errors within the text. For example, words that have low ASR confidence may be underlined, and if you click on-screen, there are options to swap out the word with other options. These revisions systems may also include grammar checkers. 

\subsubsection{Model Descriptions \& Implications of Dysfluencies}

To refine speech technologies for PWS, we focus on endpointer and ASR models independently. Endpointer models are optimized to balance the trade-off between cutting someone off too early and having a long delay after their speech, and implicitly or explicitly rely on cues such as how much silence has elapsed since the last word (e.g., \cite{Maas2018DNNEndpointer,li2020RNNTEndpointer}). These models are largely optimized on data from people who do not stutter, and are tuned to respond to the user with as low latency as possible. 
For PWS, as described by Bleakley \etal~\cite{bleakley2022exploring} and in Sections \ref{sec:survey_results} and \ref{sec:asr_results}, endpointer models commonly cut off before the user is done speaking, especially during blocks where there may be a long pause or gasp, or even partial word repetitions where the vocalization may be indecipherable.

At a high level, ASR models (e.g., \cite{yi2021hybridASR, hinton2012HybridASR,chan2015ListenAttendSpell,graves2012RNNT}) commonly consist of an acoustic component that encodes low-level phoneme or phone-like patterns, a language component that acts as a prior over word sequences, in some cases a pronunciation component that describes the phonetic pronunciation of words (e.g., for hybrid ASRs \cite{hinton2012HybridASR, Sak2013HybridModelComponents, le2020hybridASR}),
% MehryarMohri2008ASR <- this isn't a hybrid ASR
and a decoder that may map these together and generate candidate transcriptions. 
For PWS, we hypothesize that sound, syllable, or partial word repetitions fed into the acoustic component may have lower confidence phone- or phone-like outputs, as these models may not be trained with large amounts of dysfluent speech.
Similarly, the language component may not be trained with word or phrase repetitions, meaning these repetitions may have lower likelihood and be misrecognized. 
Furthermore, interjections mid-word or partial word repetitions may cause errors when paired with a pronunciation dictionary and decoder, as there may be spurious phone-like units interspersed with known words. 
% (e.g., hybrid \& end-to-end models
% ~\cite{gondala2021error} \todo{check citation}. 
% uses machine learning algorithms to convert spoken language to text. 
% Traditionally people use a Hybrid Approach to build an ASR~\cite{KelseyFoster}. 
% ASR models get less certain on dysfluent speech with sound, syllable, or partial word repetitions and they output words where there are whole word repetitions and interjections, so are misrecognized words and repetitions even if the user did not intend to say them.
%\note{pg: I think here we need a better explanation: Acoustics attempt to be faithful to the sound, so what you said is right, but also suffer when the sounds are not complete words. Language models on the other hand try to use predictability, which makes repetitions unlikely so they tend to substitute with more likely/similarly sounding words...}

It is worth noting that while VAs and Dictation often rely on the same underlying ASR system, a VA's model may be tuned to work better for a smaller set of assistant commands~\cite{gondala2021error}, whereas Dictation may be biased towards free speech from arbitrary topics. 
In addition, for VAs, an NLU model (e.g., Chen \etal~\cite{chen2019active}, which is used in this paper) may take an erroneous transcription and map it to the correct action using context and error cues. 
This means that individual ASR errors may play a more important role in Dictation than for VA tasks.
% to  implicitly identify which words are important or use additional context to route a transcription with dysfluencies to the correct task. 
% For a VA, it may be inconsequential if someone stutters on unimportant words, but is fluent for important ones. The NLU may implicitly identify which words are important or use additional context to route a transcription with dysfluencies to the correct task. 
% For non-consequential words NLU models may 
% Word or phrase repetitions may not be problematic because of the fuzzy match, and errors on less important 
% Because of this fuzzy match, repetitions may not be very problematic. , however substitutions. 



% a lexicon model that maps pronunciation knowledge
% With the emerging of deep neural networks recent years, components such as acoustic model in the hybrid ASR adopts deep neural networks to improve ASR performance~\cite{AlexGraves} while an end-to-end deep learning approach of building ASR system sprung. 
% An end-to-end ASR directly maps a sequence of input acoustic features into a sequence of words~\cite{AlexGraves}, instead of having separately trained acoustic, pronunciation and language model components, 
% Though end-to-end systems reduce efforts needed from domain experts (for example for lexicon expert phoneticians need to handcraft a phoneme set for each language) and tends to outperform hybrid models~\cite{AwniHannun}, hybrid ASRs are still dominantly used in commercial VAs and DSs ~\cite{KelseyFoster}.
% though many companies are transitioning to an end-to-end approach. 



% TO be cited:
% Deep Speech: Scaling up end-to-end speech recognition. Awni Hannun
% Towards End-to-End Speech Recognition with Recurrent Neural Networks, Alex Graves
% Need to cite this properly: https://www.assemblyai.com/blog/what-is-asr/, Kelsey Foster




% https://www.forbes.com/sites/stevenaquino/2021/10/05/exclusive-amazon-adds-new-speech-setting-to-alexa-app-to-help-stutterers-finish-commands-queries/?sh=3380f1542b34
% This Alexa news may serve as a support for being cutoff.


% \textbf{Implications of Dysfluencies.}
% \todo{consider integrating this subsection into the previous section and maybe Section 4 (ASR)}
% \hfill\\
% Endpointer “model-feature-list": "num-trailing-sil,end-of-sentence,num-of-words,pause-counts,silence-posterior",
% https://compass.scv.apple.com/confluence/display/SiriPerception/Endpoint+Feature
% \textit{Endpointer}: 
% \note{mention implications on invocation and punctuations models?}

\subsubsection{Dysfluent Speech Recognition}

Technical work on improving speech assistants for PWS has focused on ASR models~\cite{shonibare2022enhancing,Mendelev2020,gondala2021error,mitra2021,Tripathi2018,Tripathi2020,HeemanInterSpeech16}, stuttering detection~\cite{LeaStutterDetection2021}, dysfluency detection or classification~\cite{lea2021sep,kourkounakis2020detecting,Mahesha2016,DasNSRE2020,riad2020identification}, clinical assessment~\cite{BayerlTSD2020}, and dataset development~\cite{FluencyBank,UCLASS,lea2021sep,KSoF}.
% Much of this work has centered on dysfluency detection either as a standalone task or as part of an ASR system. 
% Three ASR-oriented approaches are as follows. 
Shonibare \etal ~\cite{shonibare2022enhancing} and Mendelev \etal  ~\cite{Mendelev2020} investigate training end-to-end RNN-T ASR models on speech from PWS. 
Shonibare \etal\ introduces a detect-then-pass approach that incorporates a dysfluency detector where audio frames with dysfluencies are ignored entirely by the RNN-T decoder. 
Examples in the paper demonstrate how this approach can be used to ignore some partial-word repetitions and blocks.
% The temporal context is very short (100 ms) so it is unlikely to generalize to whole word or phrase repetitions or to inaudible blocks mid-word. 
Alharbi \etal~ \cite{AlharbiWOCCI17,alharbi2018lightly} focused on stuttered speech from kids that incorporates the structure of repetitions and other dyfluencies into an augmented language model that is better at including dysfluencies in a transcription. 
In our work, we focus on solutions, like Mitra \etal's \cite{mitra2021}, which can be applied on top of existing recognition systems and do not require as much data as end-to-end solutions. 
Their VA-oriented approach was to optimize a small set of ASR decoder parameters on stuttered speech, such that the system is biased towards common VA phrases, and was effective in removing dysfluencies such as repetitions in speech.
% sound and partial-word repetitions. 
One limitation of that work is that it was only applied to speech from 18 PWS, so in this paper we validate results on our much larger 91 person study. 
% approach for Voice Assistant tasks that can be applied on top of existing ASR models, and
% and apply it to our 91 person dataset
% which may be production-oriented 
% It is challenging to get large amounts of stuttered speech data and moreover dysfluency detection labels, so investigated 
% optimizing a small set of ASR decoder parameters on stuttered speech, such that the system is biases towards more common phrases and shorter phrases without repetitions.
%  for Voice Assistant task
% and Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly}
% \note{[mention Mendelev which just trained an RNN-T model with a tiny amount of stuttered speech and tries replacing partial-word annotations with another symbol. ] [Neither paper uses absolute WER! only relative. ]} 
% Efforts from Project Euphonia~\cite{projecteuphonia}, the largest atypical speech project to date, have included data from PWS but it has not been a core focus in publications.
% \todo{mention limitations and connections to our work}


% \note{move} The definitive ASR evaluation metric is Word Error Rate (WER). In some papers on stuttering, there are separate metrics for intended speech and articulated speech and correspondingly metrics iWER and aWER. 
% Intended speech has all dysfluencies removed and articulated speech retains all spoken words included repetitions.  
% For PWS, partial-word repetitions and blocks tend to cause word substitutions and increase both iWER and aWER. 
% Word and phrase repetitions increase iWER but not aWER.
% Errors in the acoustic model may be caused by blocks, sound repetitions, or partial words. 
% Errors in the language model may be caused by repetitions. 
% And if the number of candidates in the Beam Search decoder is too small it may not have enough memory to smooth over partial word repetitions. 

% For Voice Assistants, an \textit{NLU} model routes a transcription to the correct VA command. 
% For example ``What what is the weather?'' and ``What is the weather?'' would map to the same ``weather'' action. 
% This can mask transcription errors in the ASR by doing selective word finding.
% In this work we look at the use of intents~\cite{GoogleConversationalAI} where an intent may be a slotted command like ``Search for the weather in [city] on [date]'' where ``[city]'' and ``[date]'' are filled in by the user. 
% We compute results for intent recognition using the ML-based NLU system described in~\cite{chen2019active}.
% These are used as an upper bound on final accuracy or ``usefulness'' of a VA system. 

% A commercial Natural Language Understanding \textit{(NLU)} model may route ASR predictions to Voice Assistant commands using \textit{domains}, \textit{intents}, and \textit{actions}~\cite{chen2019active}. A domain may be a category of commands such as ``weather'' or ``timers.'' 
% The action would be responding to the user with the weather on that day and in that city. 
% There may be multiple different phrases that can lead to the same intent and action. 
% Typically, there is a machine learning model that attempt to identify the domain and parameter inputs. This model may also use outside information, like contacts on your phone or your GPS location to determine the most likely response. 
% In traditional NLU models, the system must simply identify critical words
% , but there is more flexibility than in Dictation. 
% For example, there is often a fuzzy search which improves performance on proper nouns., \eg ``New New York City'' translates to ``New York City.'' 
% In addition, repetitions or inaccurate prediction of unimportant words may be skipped by the model and result in the same intent, such as ``what is the weather'' and ``what in is what is the weather.``
% \todo{turn google link into citation. do they have a paper describing?} \url{https://developers.google.com/assistant/conversational/overview}.
% Word or phrase repetitions may not be problematic because of the fuzzy match, and errors on less important 
% Because of this fuzzy match, repetitions may not be very problematic. , however substitutions. 


% [issues: repetitions and LM; partial word reps and beam search; sound reps and prolongations with AM; blocks and endpointing, etc.]


% ---------------------------------------------------------------
% \subsection{Related Work}

% \subsection{Technical Literature \note{integrate with Speech Tech section?}}

% \todo{THIS SECTION IS COPIED FROM MATERIAL IN OUR PREVIOUS PAPERS; COLIN WILL CLEAN UP/CONDENSE/ETC}

% Technical work on improving speech assistants for PWS has focused on ASR models~\cite{shonibare2022enhancing,Mendelev2020,gondala2021error,mitra21,Tripathi2018,Tripathi2020,HeemanInterSpeech16}, stuttering detection~\cite{LeaStutterDetection2021}, dysfluency detection or classification~\cite{lea2021sep,kourkounakis2020detecting,Mahesha2016,DasNSRE2020,riad2020identification}, clinical assessment~\cite{BayerlTSD2020}, and dataset development~\cite{FluencyBank,UCLASS,lea2021sep,KSoF}.

% Much of this work has centered on dysfluency detection either as a standalone task or as part of an ASR system. 
% Shonibare \etal \cite{shonibare2022enhancing} and Mendelev \etal  \cite{Mendelev2020} incorporate dysfluency detectors as part of training end-to-end RNN-T ASR models. Shonibare \etal introduces a detect-then-pass approach where audio frames with detected dysfluencies are ignored entirely by the RNN-T decoder. 
% Examples in the paper demonstrate how this can be used to ignore some partial-word repetitions and blocks.
% % The temporal context is very short (100 ms) so it is unlikely to generalize to whole word or phrase repetitions or to inaudible blocks mid-word. 
% Mitra \etal \cite{mitra2021} takes a production-oriented approach that can be applied on top of a pre-trained ASR model. 
% % It is challenging to get large amounts of stuttered speech data and moreover dysfluency detection labels, so investigated 
% % optimizing a small set of ASR decoder parameters on stuttered speech, such that the system is biases towards more common phrases and shorter phrases without repetitions.
% They show that for Voice Assistant task you can optimize a small set of ASR decoder parameters on stuttered speech, such that the system is biased towards more common phrases and shorter phrases that remove sound and partial-word repetitions. 
% % and Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly}
% Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly} focused on stuttered speech from kids that incorporates the structure of repetitions and other dyfluencies into an augmented language model that is better at including dysfluencies in a transcription. 
% % \note{[mention Mendelev which just trained an RNN-T model with a tiny amount of stuttered speech and tries replacing partial-word annotations with another symbol. ] [Neither paper uses absolute WER! only relative. ]} 
% Efforts from Project Euphonia~\cite{projecteuphonia}, the largest atypical speech project to date, have included data from people who stutter but it has not been a core focus in publications. 
% % There has been significant interest 
% % [Project Euphonia has stuttering data as well but I can't remember seeing anything stuttering-specific that they've worked on.]

% \todo{sort these}
% * "Systematic review ... detecting developmental stuttering." \cite{barrett2022systematic}. 
% * Machine learning for stuttering identification: Review \cite{sheikh2021machine}
% * Stuttering detection: Introducing ECAPA-TDNN and Wav2Vec2. 0 embeddings to stuttering detection. arXiv'22
% * “Identification of primary and collateral tracks in stuttered speech,” \cite{riad2020identification}
% * Automatic recognition of children’s read speech for stuttering application,” vol. WOCCI, 2017. \cite{AlharbiWOCCI17}
% * Intelligent processing of stuttered speech \cite{Czyzewski2003}
% * A lightly supervised approach \cite{alharbi2018lightly, AlharbiWOCCI17} 

% Stuttering Challenge (2022): \cite{schuller2022acm} uses the KSoF dataset. 

% KSoF: The Kassel State of Fluency Dataset--A Therapy Centered Dataset of Stuttering
% * " the ability to detect stuttering events and modifications in speech could help PWSs and speech pathologists to track the level of fluency"
% * " 5500 clips of PWSs. The clips were labeled with six stuttering-related event types: blocks, prolongations, sound repetitions, word repetitions, interjections, and – specific to therapy – speech modifications."



% Prolongations, or extended sounds, have been detected using short-window autocorrelations [16] and low-level acoustic models [10]. Word/phrase repetitions, if they are well articulated, are easily detected using LM- based approaches [19], with the caveat that single-syllable words such as in the phrase “I-I-I am” will often be smoothed into “I am” due to the underlying acoustic model and phrases like “I am [am]” may be pruned because the LM has never seen the word “am” repeated before. This is fine for speech recognition but bad for stuttering event analysis. Arjun et al. [16] addressed this repetition problem by segment- ing pairs of subsequent words and analyzing correlations in their spectral features. Interjections, including “um”, “uh”, “you know” and other filler words, are perhaps the easiest type to recognize with a language model if well articulated. Blocks, or gasps/pauses typically within or between words, are difficult to detect because the gasp for breath or pause is often inaudible. Sound repetitions are also challenging because syllables may vary in duration, count, style, and articulation (e.g.,“[moh-muh-mm]-ommy”).
% Efforts in HCI have sought out an understanding of speech recognition needs for users with speech impairments, which is critical for framing problems like ours [1, 2, 22].




% \subsection{Background on Stuttering \todo{move or incorporate elsewhere}} 
% Individuals may develop reactions to speaking in various situations leading to avoidance of target words, sounds, or speaking situations and observable escape behaviors such as foot stomping or eye blinking. 

% Stuttering and cluttering are types of fluency disorders, defined by an interruption in the flow or fluidity of connected speech.  Stuttering is more common and may also be referred to as stammering~\cite{ward2011cluttering}.  Stuttering is a breakdown in speech fluency that can affect the rate and flow of speech and can include specific dysfluency types, such as sound (``p-p-pop'') and syllable repetitions (``be-be-become''), word repetitions (``mom, mom, mom``), sound prolongations (``mmmmmom''), and silent or audible blocks (inability to initiate target sound) \cite{sander1963frequency, SSI}. Frequent interjections (``um'', ``eh'') are also common.  

% PWS typically cannot control when their stuttering will occur and cannot control how people or technology perceive and respond to their dysfluencies. 
% The setting or environment, current mood/stress level, communication partners, or other variables can impact stuttering.  Some people stutter frequently when in a group but not when on their own \cite{tichenor2021variability}. Some people stutter more when in front of a smart device because of ``pressure to perform.'' 
% Individuals may develop reactions to speaking in various situations leading to avoidance of target words, sounds, or speaking situations and observable escape behaviors such as foot stomping or eye blinking.  
% Over time, a PWS may also experience negative psychological outcomes such as social anxiety, low self-esteem, and negative feelings about communication~\cite{boyle2015identifying}. This can be a cycle as increased anxiety may then lead to an increase in producing stutter events.  
% Stuttering may be developmental, neurogenic, or psychogenic \cite{roth1989clinical, seery2005differential}.  

% PWS vary in terms of how many and what types of dysfluencies they produce. 
% The frequency of dysfluencies, duration of dysfluencies, physical concomitants (i.e., stomping a foot, moving hands), and the impacts that stuttering has on participation in communication across settings varies significantly across individuals \cite{tichenor2021variability}. These overt cues are used in clinical settings to assess severity and changes over time~\cite{SSI,yaruss2006overall}. 
% In this work we used severity to recruit participants, but ultimately find a more nuanced understanding of the rates and characteristics of each dysfluency type and their impact on speech recognition technology.  


% Multiple factors are considered when clinically assessing stuttering severity including . 
% We are working to improve ASR so that PWS can be successful and more confident with use of speech recognition.   

% [\textbf{TODO}\textbf{: change citations and put in bibliography]}

% @article{boyle2015identifying,
%   title={Identifying correlates of self-stigma in adults who stutter: Further establishing the construct validity of the Self-Stigma of Stuttering Scale (4S)},
%   author={Boyle, Michael P},
%   journal={Journal of Fluency Disorders},
%   volume={43},
%   pages={17--27},
%   year={2015},
%   publisher={Elsevier}
  
%   @book{ward2017stuttering,
%   title={Stuttering and cluttering: frameworks for understanding and treatment},
%   author={Ward, David},
%   year={2017},
%   publisher={Psychology Press}
% }
  
%   @article{yaruss2006overall,
%   title={Overall Assessment of the Speaker's Experience of Stuttering (OASES): Documenting multiple outcomes in stuttering treatment},
%   author={Yaruss, J Scott and Quesal, Robert W},
%   journal={Journal of fluency disorders},
%   volume={31},
%   number={2},
%   pages={90--115},
%   year={2006},
%   publisher={Elsevier}
% }
% Riper~\cite{VanRiper1982}, SSI-4~\cite{SSI}, Andrew \& Harris~\cite{andrews1964syndrome}, Time-interval measurement~\cite{valente2015event,ingham1993time}.




% ------------------------------------------------------------------------------------

\subsection{Accessibility of Speech Recognition Systems} %HCI \& Technical Literature}
Voice interaction is used by a wide range of people with disabilities---such as the speech input that enables many people with motor disabilities to control computing devices (e.g.,~\cite{zhong2014justspeak, corbett2016can}), and as an inherently accessible input modality for many blind and low vision users (e.g., ~\cite{pradhan2018accessibility, abdolrahmani2018siri}). However, this work often assumes that speech input itself is accessible.

% Focusing on studies with users who have atypical speech, 
Researchers have captured speech input challenges encountered by people with dysarthria~\cite{ballati2018assessing,projecteuphonia}, deaf or hard of hearing people~\cite{fok2018towards}, and people with aphasia~\cite{roper2019speech}. 
For stuttering specifically, there has been relatively little human-centered work~\cite{clark2020speech}. A recent exception comes from Bleakley et al.~\cite{bleakley2022exploring}, who report on interviews and a three-week diary study of smart speaker use at home with 11 PWS. 
%Usage followed patterns typical of the general population (e.g., music and information queries were most common). 
While participants had ``some success’’ in using the device, challenges included the device timing out, social pressure when using the device around other people, and difficulty with specific sounds (especially those that could interfere with the wake word, i.e., ``OK Google’’). Participants reported repeating and reformulating utterances to overcome these issues. While this study provides an initial understanding of how PWS use VAs, stuttering severity of the participants is not reported, and an objective assessment indicating how well the smart speakers recognized their speech is not provided. In contrast, our study examines speech input technology more broadly (e.g., including dictation), and includes both quantitative subjective data from a larger sample of n=61 PWS and system performance on stuttered speech samples collected from n=91 PWS. 

% Beyond Bleakley et al.'s study on speech input accessibility and stuttering~\cite{bleakley2022exploring}, 
A few other human-centered projects have looked at supporting speech therapy for PWS and at managing stuttering in everyday life. Demarin et al.~\cite{demarin2015impact} and Madeira et al.~\cite{madeira2013building} both present apps to record stuttering experiences with the goal of increasing awareness and informing therapy decisions; small user evaluations included 2 and 5 PWS, respectively.
Focused on managing speaking situations, Fluent~\cite{ghai2021fluent} supports people in writing scripts that they will be more likely to read aloud fluently. The tool uses active learning to identify words that the user is likely to encounter issues with, and suggests alternative words that may be easier to speak; no user study has been reported. Finally, McNaney et al.~\cite{mcnaney2018stammerapp} employed a multi-stakeholder co-design process to design StammerApp, a mobile app that allows users to set goals, practice, and reflect on their experiences in especially challenging situations. While the project did not focus on speech input, it provides a qualitative understanding of a total of 39 participants’ experiences with stammering, including specific challenges (e.g., talking on the phone), and a general desire to be able to ``stammer openly and feel more confident and relaxed with their own voice.'' Ultimately, our goal is for PWS to have this freedom and confidence when interacting not only with other people, but with speech input technology as well.




% \note{need to figure out whether to keep this content or not \note{LF: Yeah I guess we can cut. What do you think now, Colin?}}Speech has also been explored as a form of input for augmentative and alternative communication (AAC) systems, which are traditionally controlled through touch, gaze or switch input. 
% The VIVOCA project, for example, recognizes spoken input from users with atypical speech by training a personalized limited vocabulary speech recognition model that can activate pre-defined synthesized speech output~\cite{hawley2012voice}. Speech recognition has also been employed for speech therapy goals---including using both off-the-shelf systems such as smart speakers (e.g., \cite{smith2021smart}), and custom-designed games to increase enjoyment of speech therapy exercises, such as Apraxia World~\cite{hair2018apraxia}.


% There has been significant interest 
% [Project Euphonia has stuttering data as well but I can't remember seeing anything stuttering-specific that they've worked on.]




==> CHI2023 Stuttering/sections/3a-survey-method.tex <==
\section{Speech technology survey for PWS}\label{sec:survey_results}
% \section{Findings}

Our first goal is to understand the experience of speech technology for PWS, including how well existing systems are perceived to work, what challenges arise, and areas for improvements. 
We accomplished this by deploying a comprehensive online survey to 61 PWS in the United States during a three-month period in mid-2022.
% with varying frequency and severity of dysfluencies, as determined by
%and who were screened by 
% a speech language pathologist (SLP). 


   
% screen out individuals who did not have a 
% An SLP using the Andrew \& Harris (A\&H) Scale~\cite{AndrewsHarris1964} into mild, moderate, and severe stuttering groups. 



% and \note{92}  contributed audio recordings. 
% \note{technically 100 people for audio, but we don't have annotations for 8}.
% \todo{how do we want to discuss Phase 1 and Phase 2? should they be merged entirely? there are some protocol changes like the connected speech sample}
% Of these individuals, [X] were rated as mild (0-5\% of words have dysfluencies), [X] mild (6-20\% dysfluencies), and [X] severe ($\geq$20\% dysfluencies) using the A&H scale. 

% to understand the perception of PWS and through a user study where
% We analyzed interest, usefulness, and performance of speech recognition systems for PWS in two ways. 
% We did this by deploying a comprehensive survey to understand the perception of PWS and through a user study where participants recorded hundreds of audio clips that could be used for Voice Assistant and Dictation tasks. 
% We performed baseline ASR, endpointing, and intent recognition experiments and report results in Section~\ref{sec:asr_results}. 
% as well as production-oriented experiments that could be used to improve performance for PWS. 
% Most participants overlapped between the two data modalities so we also looked at correlations between system performance and survey results. 

% \subsection{Survey Results}\label{sec:survey_results}

\subsection{Survey Methods}


\subsubsection{Survey Design and Protocol}\label{survey_design}


Screened participants filled out the survey online using a commercial survey website. The survey took 30 to 60 minutes to complete and included the following four primary sections with up to 77 questions depending on conditional logic. 
% For an expanded listing of survey questions see the Supplementary Material.\todo{can we release?}
\begin{description}
    \item[Background:] Demographics (age group, gender, race/ethnicity); self-description of speech characteristics; intelligibility of speech to family/acquaintances/strangers; ownership and usage of smart devices.

    \item[Voice Assistants (VAs):] Usage, usefulness, and accuracy of VAs; why and when do PWS use VAs; when do VAs break and areas for improvements; awareness and effectiveness of features including endpointing, hold-to-speak, invocation models, and other common features. 

    \item[Dictation Systems (DSs):] Usage, usefulness, and accuracy of DSs; why and when do PWS use DSs; when do DSs break and areas for improvements; awareness and effectiveness of relevant features, whether people revise or restate transcriptions upon error. 

    \item[Future Technology:] Interest in future forms of VAs/DSs, especially if speech were perfectly transcribed.
\end{description}

Many of these questions had multiple choice responses and open-ended text input to further explain responses. For questions related to the endpointer and other technical material, layperson descriptions like ``How often does a VA cut off your speech'' were used. See the Appendix for the list of survey questions discussed here. 

\subsubsection{Participants}\label{participants}
Participants were recruited through social media, referrals from speech-language pathology clinics, and word of mouth. 
To participate, individuals had to self-identify as having a stutter, after which they signed an Informed Consent Form and were screened by a speech-language pathologist (SLP) who listened to their connected speech patterns. 
Stuttering characteristics such as frequency, duration, and distribution of dysfluency types 
%, along with physical concomitants (i.e., stomping a foot, moving hands) 
can vary greatly across individuals \cite{tichenor2021variability}, thus we aimed to recruit a broad range of participants with different stuttering severities. 
% , so speech patterns were evaluated to ensure a reasonable spread of clinical severities. 
% The frequency of dysfluencies, duration of dysfluencies, physical concomitants (i.e., stomping a foot, moving hands), and the impacts that stuttering has on participation in communication across settings varies significantly across individuals \cite{tichenor2021variability}, an we 
% These overt cues are used in clinical settings to assess severity and changes over time~\cite{SSI,yaruss2006overall}. 
% and by observing overt stuttering characteristics.
While there are many clinical severity assessments (e.g., \cite{SSI,yaruss2006overall}), 
% some of which include non-auditory cues like physical concomitants (i.e., stomping a foot, moving hands)~\cite{SSI,yaruss2006overall}, 
we chose the Andrew \& Harris (A\&H) Scale~\cite{AndrewsHarris1964} which can be performed entirely using audio recordings. 
% Candidate participants who presented as people who stutter were included and graded by the SLP using the Andrew \& Harris (A\&H) Scale~\cite{AndrewsHarris1964} into mild, moderate, and severe stuttering groups. 
The SLP performed this assessment by examining dysfluency rates in audio recordings of a participant reading a passage, talking impromptu about a topic of their interest, and speaking with other individual(s).
The result was a grading of mild (0-5\% of words have dysfluencies), moderate (6-20\% of words), or severe ($>$20\% of words) stuttering.  

With the A\&H scale, 12 participants were rated as having a mild stutter, 31 as moderate, and 18 as severe. 
When asked about whether people understood their speech, almost all participants (93.4\%, n=57/61) reported that friends and close contacts `always' or 'usually' understand their speech, however this was lower for acquaintances (73.8\%, n=45) and strangers (67.2\%, n=41). 
Many individuals noted that their speech qualities change day-to-day (65.5\%, n=40) or throughout the day (55.7\%, n=34) and on top of typical dysfluencies such as blocks, prolongations, and repetitions, their voice may be strained (42.6\%, n=26) or breathy (16.4\%, n=10). 
Most individuals noted that speaking requires `some' physical effort (67.2\%, n=41) with fewer responses of `very high` (11.4\%, n=7) or `very low` (9.8\%, n=6).

In terms of demographics, there was an even gender split between men (50.8\%, n=31) and women (49.2\%, n=30), with no participants reporting another gender. Most participants were under 40 years old: aged 18-19 (n=2), 20-29 (n=28), 30-39 (n=21), 40-49 (n=3), 50-59 (n=4), 60-69 (n=2), and 70-79 (n=1). Individuals identified as white (n=38), black or African American (n=12), Hispanic (n=5), Asian (n=2), American Indian or Alaska Native (n=1), or preferred not to answer (n=3). In terms of technology use, all participants owned smartphones, with most having an iPhone (93.4\%, n=57) and four having an Android phone. 
Over half (59.0\%, n=36) had smart speakers in the home: 27 had an Amazon device, 5 had a Google device, and 4 had an Apple device. For other technology, 58 participants reported having a computer, 35 had a tablet, and 27 had a smartwatch or fitness tracker.


\subsubsection{Analysis}
For closed-ended questions, we report primarily on descriptive statistics including counts and proportions. We have included a few comparative statistical tests for high-level questions of how often participants use VAs vs. dictation, and whether there is an impact of stutter severity ratings on usage. In doing so, we selected tests that are appropriate for ordinal data: Mann Whitney U and Kruskal Wallis tests. For open-ended questions, we conducted two open coding passes on each question and report on the prominent themes identified in this analysis to help contextualize the quantitative results.



==> CHI2023 Stuttering/sections/3b-survey-findings-old.tex <==

\paragraph{Usage and utility}
Most participants were familiar with dictation (90.2\%, n=55) and many had used it before (73.8\%, n=45). For 45 who had, a total of 26 reported regular use of at least monthly: `at least daily' (17.8\%; n=8 of 45), `at least weekly' (21.3\%; n=13), and `at least monthly' (11.1\%; n=5). These numbers are lower than for VA use, where 40 of the 61 participants reported regular use. Most people with experience using dictation had used it on the phone (88.9\%, n=40 of 45), while 24.4\% (n=11) had used it on the watch and 20.0\% (n=9) had used it in the car. Other less frequent platforms included traditional computers, tablets, and smart speakers. Common tasks included writing text messages (95.5\%, n=42), taking notes (37.8\%, n=17), writing email (18.0\%, n=11), and dictation within a web browser (16.4\%, n=10).
 
%Figure \ref{fig:usage_frequency_by_category_dictation} shows dictation usage by rated A\&H severity.  Respondents who reported that they have not heard of dictation (n=14) or did not know how how often they used dictation (n=2) were not included in the analysis.  Respondents with severe stutters had the highest proportion of users who reported they 'Never' used voice assistants, though respondents with severe stutters also had the highest proportion of daily users.
% For the 10 participants who were familiar with dictation but had not tried it, their reasons were split between concern about how well their speech would be recognized and not seeing value in dictation in general.

Most participants found dictation to be at least somewhat useful: `extremely useful' (8.9\%; n=4), `very useful' (31.1\%; n=14), and `somewhat useful' (37.8\%; n=17). The most common reasons people found it useful were for sending messages while driving, and general efficiency and ease. 
For people who reported that dictation is `not very useful' (20.0\%, n=9) or `not at all useful' (2.2\%,  n=1), the most common reasons were that it is inaccurate for their speech or inefficient compared to typing, due to having to fix errors. 
% \todo{need to decide if keeping this quote or the later similar one from this person}
As [P2-77], who did not find dictation to be useful at all, said, \textit{``because as a person who stutters I use fillers like umm, so, use a lot of repetitions, and also have frequent blocks and when I use dictation it writes down all my disfluencies that when I read the text it makes no sense.''} 
For other participants, the utility of dictation depended on the words and length of the task, as reflected by [P1-60]: \textit{``When I am using words I can say well it works good, when I have to use words that I am unable to say clearly it does not work at all.''}



% \subsubsection{Participant Background}
% These can be caused by the setting or environment, current mood/stress level, communication partners, or other variables can impact stuttering.  
% PWS vary in terms of how many and what types of dysfluencies they produce. 

% These assessments were performed 
% to ensure adequate severity distribution. The target was at least 30 from each group
% 12, 31, 18 = 61 (80% mod/severe)
% \todo{find target or final severity distribution for survey}

% Demographics were as follows. 
% There was a roughly even gender split between men (50.8\%, n=31) and women (49.2\%, n=30), with no participants reporting another gender. Most participants were under 40 years old: aged 18-19 (n=2), 20-29 (n=28), 30-39 (n=21), 40-49 (n=3), 50-59 (n=4), 60-69 (n=2), and 70-79 (n=1). Individuals identified as white (n=38), black or African American (n=12), Hispanic (n=5), Asian (n=2), American Indian or Alaska Native (n=1), or preferred not to answer (n=3).

% While we used the A\&H scale for recruitment, we wanted to better understand potential correlations with other speech patterns. For A\&H, 12 were rated as having a mild stutter, 31 as moderate, and 18 as severe. 
% When asked about whether people understood their speech, almost all participants (93.4\%, n=57) reported that friends and close contacts `always' or 'usually' understand their speech, however this was lower for acquaintances (73.8\%, n=45) and strangers (67.2\%, n=41). 
% Many individuals noted that their speech qualities change day-to-day (65.5\%, n=40) or throughout the day (55.7\%, n=34) and on top of typical dysfluencies such blocks, prolongations, and repetitions, their voice may be strained (42.6\%, n=26) or breathy (16.4\%, n=10). 
% Most individuals noted that speaking requires `some' physical effort (67.2\%, n=41) with fewer responses of `very high` (11.4\%, n=7) or `very low` (9.8\%, n=6).



% Survey (61): Counter({1: 12, 2: 31, 3: 18}) 1=mild, 2=mod, 3=severe
% Phase 1: (50): Counter({1: 25, 2: 18, 3: 7})
% Phase 2 (41): Counter({1: 2, 2: 12, 3: 27})
% Intersection of (S, P1, P2) (99): Counter({1: 25, 2: 48, 3: 26})
% Intersection of (P1, P2) (99): Counter({1: 25, 2: 44, 3: 22})


%%Note: explanation for the figure above.  This is mildly interesting, but the main points related to severity and accuracy may already be well covered elsewhere so maybe unnecessary...
% the number of surveyed participants who use voice assistants regularly (at least monthly or more frequently)
% \note{given small sample sizes is the following statistically significant? if not, maybe we should omit?}
% Figure \ref{fig:usage_frequency_by_category} shows the number of surveyed participants who use voice assistants regularly (at least monthly or more frequently) by  gender, age, A\&H severity, physical effort of speaking, and self-reported voice assistant accuracy. 
% Among the surveyed participants, men used voice assistants regularly at a proportionally higher rate than women, people with mild stutters used voice assistants more regularly at a proportionally higher rate than people with moderate and severe stutters, and people who reported that voice assistants rarely understood their speech used voice assistants at a proportionally lower rate than those who reported that voice assistants sometimes or often understood their speech.  
% Most participants surveyed reported that they were between 20-29 years old or 30-39 years old and that speaking required 'some effort'. 

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.6 \paperwidth]{figures/stacked_bar_usage_frequency_proportion.png}
%     \caption{Voice assistant usage frequency by A \& H severity and self-reported voice assistant accuracy.   Respondents who said that they didn't know how often they used a voice assistant (n=2) were not included in this analysis.  Respondents with severe stutters had the highest proportion of people who reported never using voice assistants, but also had the highest proportion of daily users.  Usage frequency was generally highest for those who reported that voice assistants often understood their speech accurately and lowest for those who reported that voice assistants rarely understood their speech accurately. 
%     %\todo{Can we add more ticks?} added additional ticks
%     }
%     \label{fig:usage_frequency_by_category}
% \end{figure}
% %\begin{figure}[t!]
% %    \centering
% %    \includegraphics[width=0.4 \paperwidth]{figures/stacked_bar_dictation_usage_frequency_proportion.png}
% %    \caption{Dictation usage frequency by A\&H severity, by participants who reported they are familiar with dictation technology.  Respondents with severe stutters had the highest proportion of users who reported they 'Never' used voice assistants.
% %    }
%     \label{fig:usage_frequency_by_category_dictation}
% %\end{figure}


% In terms of technology use, all participants owned smartphones, with most having an iPhone (93.4\%, n=57) and four having an Android phone. 
% Over half (59.0\%, n=36) had smart speakers in the home: 27 had an Amazon device, 5 had a Google device, and 4 had an Apple device. For other technology, 58 participants reported having a computer, 35 had a tablet, and 27 had a smartwatch or fitness tracker.


% \note{how did we analyze the open-ended responses. If we do any statistical analysis we can describe that here.}

% to do: add participant breakdown by age, gender, race?


% \subsection{Participant Recruitment}
% Participants were recruited through social media, referrals from speech language pathology clinics, and word of mouth. Individuals self-identified as having a stutter. An SLP also screened the individuals by listening to their connected speech and by observing overt stuttering characteristics.\note{Colin mentioned there were 4 tasks the vendor's SLP used to screen and grade a participant)}
% The participants who presented as people who stutter were included and graded using A&H Scale into mild, moderate, and severe stuttering groups to ensure adequate severity distribution. In total \note{66} people filled out the survey and \note{92}  contributed audio recordings. 
% % \note{technically 100 people for audio, but we don't have annotations for 8}.
% % \todo{how do we want to discuss Phase 1 and Phase 2? should they be merged entirely? there are some protocol changes like the connected speech sample}
% Of these individuals, [X] were rated as mild (0-5\% of words have dysfluencies), [X] mild (6-20\% dysfluencies), and [X] severe ($\geq$20\% dysfluencies) using the A&H scale. 

% --------------------------------------------
% \subsection{Overview, severities, characteristics, etc. }

% \todo{These sections are copied from our Quip summary; modify as makes sense...}

% \todo{?How do we want to show numbers? Should we include a table (or set of tables?)}


% --------------------------------------------

\subsubsection{Voice Assistants} \label{subsec:VAs}
All participants were familiar with voice assistants and almost all (96.7\%; n=59) had used one. 
Most of this experience was on phones (83.6\%; n=51) and smart speakers (45.9\%; n=28), while smartwatches and car infotainment systems were also relatively common (both 24.5\%; n=15); 10 or fewer participants had used voice assistants on tablets or traditional computers.
% Here, we report on usage patterns compared to the general population as well as \todo{whatever we report on}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4 \paperwidth]{figures/bar_va_usage_frequency_comparison.png}
    \caption{Voice assistant usage by the general population and by stuttering survey respondents.  Bars show 95\% confidence intervals of calculated proportion calculated using Clopper-Pearson "exact" method.  Raw data was not available to calculate confidence intervals for general population data \cite{npr_smart_audio}}
    \label{fig:utilization_comparison}
\end{figure}

\paragraph{Usage \& Utility}
% %relative to general population}
% %% Comparison to survey of general population (may be too long for how hard this is to interpret %%
Among voice-assistant users, reported usage frequencies were lower than estimates for the general population (Figure \ref{fig:utilization_comparison}).  Particularly, the proportion of daily users among PWS voice assistant users was significantly less than in the general population. 
From a survey- and interview-based study, National Public Media \cite{npr_smart_audio} estimated that, from among 62\% of voice-operated assistant users in America, 57\% use a voice-operated assistant at least daily, 23\% at least weekly, and 20\% at least monthly. From our stuttering survey respondents, among the 86.8\% (n=53) of voice assistant users (respondents who reported any frequency of voice assistant usage), 35.6\% use a voice assistant at least daily (n=19), 22.7\% at least weekly (n=12), and 17.0 (n= \% at least monthly (n=9).  

Respondents interested in voice technology may have been more likely to complete than the survey than those not interested in our technology, which may have biased some of our usage metrics - as reflected in the high proportion of voice-operated assistant users among our respondents compared to the general population.  Comparison of use frequency among voice assistant users only, as reported in Fig. \ref{fig:utilization_comparison}, is more valid than comparing overall usage percentages, as the base for both datasets are respondents who use voice technology only.  Respondents who used voice technology most often reported daily usage, among both the general population and PWS, suggesting that voice assistant users are more likely to use the technology frequently than sparingly irrespective of whether they stutter.


% Among our stuttering survey respondents, 65.6\% (n=40 of 61) reporting using a VA regularly (monthly or more frequently) and of those 47.5\% use daily (n=19, 31.1\% of all), 30.0\% use weekly (n=12, 19.7\% of all) and 20.0\% use monthly (n=9, 14.8\% of all). 
% Results suggest that the proportion of respondents who reported using a VA regularly may be related to stuttering severity (Figure \ref{fig:utilization_comparison_severity}), with users with mild stutters having usage rates similar to the general population. However, these results are not statistically significant due to the small number of participants in each severity group. 

\todo{proposed new points to make?:}
\begin{itemize}
    \item  report similar proportions of usage (i.e. majority are daily users, decreasing proportions as usage frequency decreases) compared to NPM study. Not enough samples to have statistical significance to determine whether usage is generally lower for PWS (added in a sentence describing this).
    \item Usage is correlated with self-reported understanding (for both VA and dictation systems
    \item  reported SR systems' understanding compared to understanding with family, acquaintances, strangers; larger proportion of understanding is seen with VAs (evidence of an area of improvement?) see Figure \ref{fig:understanding_comparison}

\end{itemize}

Figure \ref{fig:usage_frequency_by_category} shows usage breakdowns by  A\&H severity, and self-reported voice assistant accuracy.\footnote{Two respondents reported that voice assistants 'always' understood their speech.  For the presented analyses, this response was included in the 'Often' category.  No respondents reported that voice assistants 'never' understood their speech.} 

VA and DS usage appears to increase when users perceive themselves as being better understood by speech technology. 
We found this correlation to be statistically significant by Kendall Tau between VA usage and self-reported VA understanding (\textit{$r_{\tau}$}=0.45, \textit{p}<0.001) where VA usage is discretized into daily, weekly, monthly, more than monthly usage and never, and VA understanding is discretized into always/often, usually/sometimes, rarely/never. Similarly, DS usage and self-reported VA understanding had lower correlations(\textit{$r_{\tau}$}=0.17, \textit{p}=0.11). 

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4 \paperwidth]{figures/Understanding_proportions.png}
    \caption{Proportions of self-reported understanding by VAs, family, acquaintances, and strangers ($n$=59, $n$=57, $n$=57, $n$=56)\todo{double-check survey responses on why is N different}.}
    \label{fig:understanding_comparison}
\end{figure}


% \paragraph{Utility}
We distinguished usage with usefulness, as perhaps individuals do not use VAs frequently but when they do they find them highly valuable. 
A majority of participants (70.5\%) found VAs to be at least somewhat useful and many 27.3\% found it very or extremely useful: `extremely' (9.8\%; n=6), `very' (27.9\%; n=17), and `somewhat' (32.8\%; n=20). These roughly mirror usage patterns.

%% People who use voice assistants
Amongst regular users (n=40), n=16 described specific use cases that positively influenced their perception, including playing music/radio (n=8), retrieving information (n=5), controlling smart home devices like lights and temperature (n=3), and n=2 each for setting a timer, setting reminders, sending messages, settings alarms, and navigation.
Fourteen of these regular users highlighted the speed of voice assistants (n=6), that voice assistants can be used hands-free when driving (n=6), from across the room (n=1) or without a screen (n=1) and that they can be better than typing (n=6). 
% Participants who were more positive (extremely or very) commonly described the utility of common VA tasks such as listening to music or setting timers, while driving, and hands-free use. 

% described user experience factors that influenced their utility rating, including the speed of voice assistants (n=6), that voice assistants can be used hands-free (n=7) - as in when driving (n=6), from across the room (n=1) or without a screen (n=1) - and that voice assistants can be better than typing (n=6). 
% One regular user said that privacy concerns prevented them from using voice assistants more frequently. 
% Among regular voice assistant users, n=5 respondents reported that poor accuracy of voice assistants influenced their utility rating. 
% One respondent described feeling frustrated by being misunderstood when using a voice assistant.

In contrast, for participants who found VAs to be `not very' (16.4\%, n=10) or `not at all' (13.1\%, n=8) useful, reasons were split between participants who saw no inherent value in VAs (e.g., \textit{``I haven't felt a need for them in my life''} [P2-51]) and those who encountered accessibility challenges due to stuttering. 
For n=10 participants who did not use a VA regularly, they described challenges with poor recognition performance, that it takes longer to speak than type, or noted that they were simply not interested. 
% For example, [P2-64] wrote, \textit{``Voice assistants are not at all useful for me because I often have to repeat myself so many times for it to understand me that it’s quicker and easier for me to just use my hands and search or type what I want the assistant to do''}, while [P1-63] wrote, \textit{``It takes longer for me to speak/stutter [by] using voice assistants than it would for me to type what I need.''}
For example, [P2-64] wrote, \textit{``Voice assistants are not at all useful for me because I often have to repeat myself so many times for it to understand me that it’s quicker and easier for me to just use my hands [...]''}, and [P1-63] wrote, \textit{``It takes longer for me to speak/stutter [by] using voice assistants than it would for me to type what I need.''}
%%People who don't use voice assistants
% n=4 participants described user experience considerations that influenced how useful they found voice assistants.  
% One respondent said hands-free voice assistant usage while driving as a useful facet of voice assistants, one participant said voice assistants allow them to ask questions quickly, one participant said that voice assistants take longer than typing, and one participant said that speaking to voice assistants actually helps them pace their speech.  
% Of those respondents who do not use a voice assistant, n=10 said that their utility rating was influenced by poor accuracy of voice assistants.  
One respondent said that being misunderstood by voice assistants discouraged them from wanting to speak aloud. 
% Three respondents reported that they were not interested in voice recognition technology.

\paragraph{Overall challenges}
We asked about what factors prevented participants from using VAs more often. The most common were `voice assistants cut off my speech before I'm done talking' (59.0\%, n=36) and `voice assistants don't understand my speech well enough' (55.7\%, n=34). 
Other concerns, however, were not purely technical. 
Twenty-two participants (36.1\%) reported not wanting other people to hear them talking to the VA, reflecting a social consideration that past work has also identified~\cite{bleakley2022exploring}. 
As well, many participants (21.3\%, n=13) cited that it takes `too much physical effort for me to speak'. 
Only six participants (9.8\%) responded that `voice assistants don't seem useful'. 

\paragraph{Speech recognition accuracy and errors} \todo{add section similar to what's in dictation?}
\note{this is out of context... e.g. WER on what data? }
\todo{move to ASR section where we talk about similar things} 

The types of dysfluencies, frequency and severity may impact the performance of speech recognition systems (Section \ref{sec: clinical-component}), how comfortable users feel using them, and ultimately usage.

% \todo{Can we state somewhere that we only include correlations with $p<0.5$ instead of including everywhere? or is that insufficient?)
% There may be differences in satisfaction with voice assistants and usage practices between users with stuttered speech and the general population that are not reflected in use frequency metrics. 


% %Note: Redundant with Fig 3? 
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.4 \paperwidth]{figures/bar_va_usage_frequency_by_severity.png}
%     \caption{Voice assistant usage by stuttering survey respondents.  The proportion of u %by the general population (from \cite{npr_smart_audio}) and by stuttering survey respondents.  Bars show 95\% confidence intervals calculated using Clopper-Pearson "exact" method
%     }
%     \label{fig:utilization_comparison_severity}
% \end{figure}





% About half of people surveyed use a voice assistant on a daily or weekly basis. Two-thirds find it at least somewhat useful, especially when driving or when their hands are occupied but only about half says it works often or always. The rest either aren’t interested in this technology or recognition performance is too low to use. Interestingly, some people that are moderate-to-severe stutterers according to our data collection are regular users; stuttering can be very situational and some individuals report interest in Voice Assistants when they are alone and don’t stutter but not in public where stuttering is more likely. 

%\paragraph{Utility and Challenges}
%In general, most people surveyed are interested in speech technology, but are aware of its limitations. The perception of underlying features is in-line with expectations: people are regularly cut off, their words are miss-construed, and they are required to repeat themselves multiple times. 



\paragraph{Invocation}
Most VAs use a wake word to start the system like ``Alexa'' or ``OK Google''. Almost half of participants reported that these wake words `always' (11.5\%, n=7) or `often' (36.1\%, n=22) worked for them. 
Problematically, 17 participants (27.9\%) reported wake words only working `sometimes' and 8 participants reported `rarely' or `never' (13.1\%); the remaining participants had not used a wake word. 
While we did not ask participants to elaborate on their use of wake words, a handful of responses to other open-ended questions referred to challenges with wake words, including: \textit{``Problem with wake words is my biggest frustration. I would want to change it to something I can say easily''} [P2-1] and \textit{``It's [Hold/Squeeze to Speak is] useful on my phone to bypass the lag that occurs when [the VA] does not recognize me using the wake phrase''} [P1-28]. 
A potential solution is to allow users to change the wake word. Alexa has at least five options, Google Assistant has two, and Siri has one.

% TODO: Leah: I commented this out but maybe we should keep it somewhere? -- Very few people (5 of 55) know about Type to Siri and two of those people didn’t find it valuable. 

\paragraph{Endpointer and alternatives}
Being cut off by the VA was a common challenge reported in Bleakley et al.'s~\cite{bleakley2022exploring} interviews with 11 PWS. Our data demonstrates the pervasiveness of this problem: almost half of participants stated that VAs cut them off `always' (3.3\%, n=2) or `often' (37.7\%, n=23), while an additional 31 participants (50.1\%) reported being cut off `sometimes' or `rarely'. For the 57 participants who had at least some experience being cut off, when asked if they knew why they had been cut off, by far the most common explanation was that there was a pause or block in their speech and the system thought they had finished speaking (77.2\%, n=44 of 57). 
% For example, participants wrote: \textit{``[The VA cuts me off] Because I have a break in speaking due to stuttering''} [P2-49] and 
% \textit{``They cut me off because they don't realize I'm blocking''} [P2-29]. 
Being cut off could also have follow-on impacts, as [P2-42] described: \textit{``The [smart speaker] which I use most often does not like any hesitations in speech. It assumes the slightest pause means the person is done speaking. So I get cut off often. It creates a sense of having to rush which makes my speech worse.''}
We address endpointing errors in Section~\ref{sec: endpointer} and significantly reduce the problem for all study participants.
\note{moved from related work} Some people stutter frequently when in a group but not when on their own \cite{tichenor2021variability} or when in front of a smart device because of ``pressure to perform'' as we describe in Section~\ref{sec:survey_results}.


Android and iOS offer an alternative to automatic endpointing on smartphones, where you can push down a button (physical or virtual) while speaking and only release it when done, although this is not available on screen-free devices like smart speakers. Twenty-seven participants (44.3\%) reported using a device that supports this functionality. Of those 27, almost all found being able to press a button and speak to be useful: 51.9\% (n=14 of 27) `extremely useful', 18.5\% (n=5) `very useful', and 29.6\% (n=8) 'useful'. Reasons provided for this utility were most commonly that it eliminates being cut off, but some participants also explicitly referred to feeling less rushed or worried, such as: \textit{``I can fully get my phrase in without worrying about blocking''} [P1-62] and \textit{``I don't feel rushed to finish what I need to say''} [P1-45]. A few participants mentioned that pressing a button to talk also eliminated issues with wake words, such as [P1-73], \textit{``Because it knows when to start listening and when I'm done.''}

%(62.2\%, n=38) state that VAs sometimes, often, or always cut them off due to blocks or other dysfluencies. 

% \paragraph{Revisions} 
\paragraph{Failure mitigation} 
When VAs fail, one strategy used with mixed success by participants is to revise or restate the command. Many participants (36.1\%, n=22) reported `often' or `always' revising what they say due to inaccuracies in speech recognition. 
Of 33 people who reported on how often revision is effective, only 42.4\% (n=14 of 33) said `always' or `often', while an additional 45.5\% (n=15 of 33) said `sometimes'.  

%In order to get around endpointing issues some people use Hold to Speak. Half of the participants that use Siri at least weekly (14 of 27) have used Hold to Speak and generally have a positive impression. Users who do not find it useful say that their speech isn’t recognized even when holding down the button, likely due to word insertions errors associated with blocks or incorrect words sometimes due to partial-word repetitions. 

% [ASR/Intents]
% at least sometimes, (2) incorrect words due to partial word repetitions impacts a large percentage, and (3) in more open-ended voice queries (perhaps creating a reminder) people report word repetitions. Although, the latter is a larger problem for Dictation. 


% [?NLU?]

\paragraph{Improved Recognition} \note{move to challenges?} If speech recognition worked better for these individuals then they would be more likely to use Voice Assistants (at all or more frequently). When asked what would make them use VA’s more, responses were generally as expected: improve support for understanding or accommodating stuttered speech patterns (i.e., endpointing and general ASR). A few people are either not interested in VAs at all, expressed reluctance because of difficulty of speaking, or have other general technology-related concerns such as privacy. 

\paragraph{Non-technical}
% \subsubsection{Non-technical} 
% \note{Leah: I wonder if we can move this as an overarching theme to come in its own section after Dictation} 
There are social and psychological concerns for PWS that may not be as common in the general population.
% Errors from ASR systems may evoke an emotion in PWS that may be less prevalent in the general population. 
Multiple people note that being misunderstood can be stressful or induce negative emotion. For example: 
% one person it gives them the sense that they are inferior because Voice Assistants work for ``everyone else.'' 
    [P2-77] \textit{``I want it to be inclusive to all individuals who stutter, stammer clutter [...] we should be able to feel confident speaking in any devices and not feel inferior because [...] it was made for the population that doesn't have a speech impediment.''}, [P2-36] \textit{``It works for everyone but me. Even though I have virtually no interest in using them, it sucks that the option isn't even available to me.''}, and [P2-8] \textit{``The forcing of the technology on those that cannot navigate due to speech issues.''}
    % [P2-77] \textit{``I want it to be inclusive to all individuals who stutter, stammer clutter anyone with a speech impediment because we should be able to feel confident speaking in any devices and not feel inferior because our own voice assistant devices is not able to understand us because it was made for the population that doesn't have a speech impediment.''}
There is a related social component that extends beyond people’s general insecurities with using Voice Assistants in public. Many individuals who stutter don’t want other people to hear them stutter while talking into their device. From a practical standpoint, due to endpointing issues, there is pressure to say something without a pause or block, which in turn stresses people out, and makes them more likely to stutter.


\note{moved from related work} 
Over time, a PWS may also experience negative psychological outcomes such as social anxiety, low self-esteem, and negative feelings about communication~\cite{boyle2015identifying}. In Section \ref{sec:survey_results} we find that this extends to an emotional impact when VAs fail to recognize one's speech. 
This can be a cycle as increased anxiety may then lead to an increase in producing stutter events.  




% --------------------------------------------
\subsubsection{Dictation Systems}




\paragraph{Overall challenges} 
Of the 55 participants familiar with dictation, when asked what reasons prevent them from using dictation more often, the most common, cited by 31 participants (56.4\% of 55) was `dictation tools don't understand my speech well enough'. This response emphasizes the importance of speech recognition improvements for making dictation accessible to PWS. As with VAs, participants also commonly cited non-technical reasons for not using dictation more, most notably the physical effort it takes to speak (32.7\%, n=18) and not wanting other people to hear them dictate to the device (30.1\%, n=17). Additionally, 11 participants (20.0\%) reported that dictation does not seem useful, and 12 (26.7\%) felt that they use more refined language when they type than when they speak.

The survey asked participants if they don't use dictation regularly, what if anything would make them start. Twenty-seven participants responded, with many references to improving recognition accuracy (e.g., ``If it were more accurate and understand my stuttering speech better'' [P2-72]). Notably, however, seven \todo{IRR??} participants effectively responded that nothing would make them use dictation regularly. 
For example, [P2-44] said, \textit{``I can't think of anything. I much prefer to type''}, while [P2-51] said, \textit{``I'm not sure. As someone who stutters, and just situationally in my life, I can't imagine dictation regularly being a more convenient option than typing.''} 
These responses highlight that even with ASR improvements, some PWS may not wish to use dictation.

\paragraph{Speech recognition accuracy and errors}

With dictation, the user's speech is transcribed verbatim, in contrast to VA systems that predict the most likely command based on a spoken phrase. This difference and focus on specific words is reflected in participants' experiences with dictation errors. 
While 35.6\% (n=16 of 45 who had used dictation) felt dictation systems recognized their speech often and 2.2\% (n=1) said `always', a majority of participants encountered difficulties. Half the participants (51.5\%, n=23) felt dictation only `sometimes' recognized their speech accurately, and the remaining five (11.1\%) felt their speech was `rarely' recognized well. 
As a result of these errors, participants frequently need to revise or restate what they say, with about half of participants `always' (6.7\%, n=3) or `often' (42.2\%, n=19) have to repeat or revise what they say, and an additional 35.6\% (n=16) did so `sometimes'. 
%However, 28 participants also commented on how effective they felt this revision was, and most  this revision is not seen as working often, \note{not sure this is interesting enough to report on}

When asked an open-ended question about what types of errors tend to occur with dictation, a majority of participants \todo{IRR?? 71.1\%, n=32} described the dictation system generally transcribing wrong words (e.g., \textit{``Message contains different words than I intended''} [P2-5]). 
Some participants \todo{IRR?? (13.3\%, n=6)} also mentioned being cut off, although this was a much less common error than with VAs because many dictation systems do not use an automatic endpointer. 
A few participants mentioned punctuation, proper nouns, and slang. 
Finally, some participants mentioned specific stuttering characteristics and challenges, including repetitions being displayed
% (\textit{``Misunderstood due to repetition or actually repeats word''} [P2-46])
, the impact of blocks 
(\textit{``words that I have a block in the middle of will turn into a strange phrase''} [P2-51]) 
, and interjections being shown, as described by [P2-77]: \textit{``because I have blocks and use filler words, the fillers are listed on the text message all my disfluencies are written down and when I read over the text it makes no sense and I have to type it myself instead because I will never be fluent all the time.''} 

\todo{Need a couple of sentences summary/takeaway}

%[ASR]
%The biggest technical limitations are general speech recognition errors such as word insertions and miss recognized words. About 50\% of people report often or always needing to revise their input. With Dictation, what you say is written out verbatim whereas with a Voice Assistant the system will often filter your speech and identify the most likely command. 
%People do report being cut off, in particular when sending text messages, but it is much less common because many forms of dictation don’t have an explicit endpointer. 
%Some individuals note that blocks and partial word repetitions can turn into long strings of nonsense words and as-expected when someone has a word repetition dysfluency the word, indeed, is written multiple times. Other mentions include references to names or proper nouns being commonly miss recognized, filler words being included in a transcript, and several people mentioned punctuation being incorrect likely due to pauses in speech. One individual noted an emotional reaction to seeing their dysfluencies written out mid-dictation. 

%In addition, there should be the ability to re-start a sentence after you have already said half of it — one strategy to overcome a block is to repeat the first half of a sentence.  


%\note{stuff below here is copy/pasted from Quip and could perhaps be just removed at this stage}

%Responses for Dictation largely mirror Voice Assistants but with issues like repetitions and word errors emphasized more than being cut off. 
%Moreover, the time that it takes to revise dictation when incorrect can be a large burden. 

 
%[Usefulness]
%Some people were not familiar with dictation or hadn’t used it but on average usage was similar to voice assistants: 46\% of people use it at least weekly. 
%There is a slight reduction in people who find Dictation useful compared to Voice Assistants but this may not be statistically significant (62\% vs 67\%). 
%Many people again find it useful while driving and 
%for those who don’t find it useful it’s because of inaccuracies in the system, inefficiencies especially when needing to revise text, social acceptability, and the amount of effort needed to speak. The most common use case was sending a text message. 
%If Dictation were more accurate, people would want to use it for note taking, writing an email, and in a web browser.


%[Revisions]
%\todo{rewrite}Apple isn’t doing anything with Dictation explicitly for PWS, but it does have a corrections system that underlines “likely incorrect” words with a squiggle. When you click on the squiggle it gives you alternative word options. This can be much faster than deleting and typing out a new word. It’s unclear how often this is useful for stuttering; nobody mentioned it in their feedback. 


%[Other]
%People in the study are interested in Dictation for the same reasons as the general public: efficiency. In theory you can transcribe what you say quicker than by typing, and you can do so hands-free and without looking at the screen. In practice, for PWS, it is common to revise what you say, which means that you may need to spend more time fixing the text than to type it from scratch. These revisions are often typed, which means you need to use your hands and look at the screen. Some of the reasons study participants aren’t interested in Dictation are similar to the general population. For example, one participant noted that the way you speak is different than the way you typically type out a text message. 




%People say they would be more likely to use dictation if the issues above were improved. Moreover, based on what tasks they currently use and which ones they’re interested in using, if performance is better they may start using Dictation in a wider variety of situations including note taking, writing an email, and in a web browser.  


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.3 \paperwidth]{figures/Frequency of VA and dictation use.png} \includegraphics[width=0.3 \paperwidth]{figures/Interest in future technology.png}
    \caption{\note{Possibility for a simple figure, but also to demonstrate what I mean by a proportional bar graph (in reference previous bar graph figure comment).}}
    \label{fig:freqUseVAandDictation}
\end{figure}


% --------------------------------------------

\subsubsection{Future Technology}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.4 \paperwidth]{figures/Interest in future technology.png}
%     \caption{\note{Possibility for showing interest in speech tech if it recognized speech accurately}}
%     \label{fig:futureInterest}
% \end{figure}

\paragraph{An Ideal Speech Recognizer}
Participants were asked to imagine speech technologies that could accurately understand all of their speech. 
Within this context, most participants were at least `somewhat` interested in VAs (86.9\%, n=53): `extremely’ (n=25)`very' (n=13) `somewhat' (n=15) `not very' (n=7), `not at all' (n=1) and similar for dictation (See Figure~\ref{fig:freqUseVAandDictation} (right)). 
% In open-ended responses explaining their interest level, 
Positive responses reflected earlier feelings about VAs and dictation, notably increasing efficiency, ease and convenience, being able to do actions hands-free (including while driving), and generally having confidence in the system. 
For example, [P1-66], who currently uses VAs at least monthly and has not tried dictation wrote, \textit{``I would be extremely interested in this, especially knowing it's something I don't have to worry about the speech input being able to understand me. It would remove my hesitancy and frustration with my stuttering from the equation.''} 
Negative and neutral sentiments indicated a preference for typing, seeing no need for speech input, and value depending on context (e.g., \textit{``It would depend on the device''} [P1-64], who uses VAs weekly and dictation less than monthly). 

Additionally, some concerns around the effort required to speak and social factors arose, mirroring earlier responses and again emphasizing that speech input may not be relevant to all users even with substantial accuracy improvements. 
For example, commenting on the effort required to speak, [P2-73] wrote, \textit{``It's a nice thought but it's still easier for a person who stutters to type most of the time. Unless our hands are filthy or tied up''}, while [P2-87] wrote, \textit{``It still requires effort to speak even if it understand me perfectly, and I am good at controlling them manually.''} 
Some participants also expressed reluctance to use even such improved speech technology in a social setting, including [P2-1], who wrote, \textit{``It is easier but I would be reluctant to use voice commands in public because of my speech impediment''}, and [P1-58], who wrote, \textit{``I still would not use it at work. I would use it in spaces where I am alone, with my spouse or family.''}

%In general people would be more interested in Siri and related technologies if they did understand stuttered speech perfectly. People noted typical benefits such as efficiency and hands-free interactions. Some people were not interested because it can be effortful to speak or they don’t want other people to hear their stutter. Interest for Dictation is a little lower than a Voice Assistant while both are positive. 

\paragraph{Adaptive Tech}
Finally, we asked participants about two potential technologies that could improve accuracy for an individual user with atypical speech. 
The first was around a personalized speech recognition system that could  recognize the participant's speech well, \textit{``but you need to spend time teaching it, perhaps by reading a set of phrases into the device.''} Of the 58 participants who responded to this scenario, most (n=47) had some interest: `extremely' (27.6\% of 58, n=16), `very' (20.7\%, n=12), or `somewhat' (32.8\%, n=19). 
These 47 participants were roughly evenly split between being willing to spend only 1-5 minutes on training and spending 10-30 minutes on training; however, 12 were willing to spend even longer. One said they were not willing to spend any time. 
For the 11 participants who were either `not very' or `not at all' interested in training a system, the most common concern was the time and effort required. 
One participant, however, noted a potential issue, \textit{``My speech changes from day to day. In the middle of a bad speech day I don’t want to talk more''} [P1-55].

The second technology imagined a VA that works very well but only supports a small set of perhaps 10 to 20 high-value commands. Of the 59 participants who responded to this question, most (n=40) felt it would be useful: `extremely' (20.3\%, n=12), `very' (23.7\%, n=14), and `somewhat' (23.7\%, n=14). 
Some participants expressed the sentiment that they do not use many commands anyway, such as, \textit{``I usually only use my [device] for the same things over and over again so this would be useful''} [P2-73]. 
However, those who did not think this approach would be `very useful' (27.1\%, n=16) or `at all useful' (5.1\%, n=3) commonly had \textit{``no need for voice assisted technology''} [P2-44] or felt that \textit{``10-20 commands is not enough''} [P1-63].

% \todo{Need a couple of sentences summary/takeaway}

%We asked about participants interest in training a personalized model that could improve speech recognition. In general people were receptive to the idea, with almost half being “very” or “extremely” interested. There was a high variance in willingness to spend time training the device, their general interest in the technology, and how effective they thought it would be. Ultimately, one concern (noted by three people) is that someone’s speech characteristics may change over the course of the day or in different contexts, which may make it challenging to build a personalized model that works all the time. 

%About half of individuals were “very” or “extremely“ interested in a minimal Voice Assistant that only allows perhaps 10 to 20 commands but works better for the individual. Many proponents note that they only use a small set of commands regularly anyway so it wouldn’t be very different. There was interest in being able to customize the specific commands that you say versus having a predefined set. Some people that are not interested already use a Voice Assistant regularly with more than 20 commands and thus would view this as a regression. Others simply aren’t interested in speech technologies. 


% \begin{quote}
%     [P2-36] \textit{``It works for everyone but me. Even though I have virtually no interest in using them, it sucks that the option isn't even available to me.''}
% \end{quote}
% \begin{quote}
%     [P2-8] \textit{``The forcing of the technology on those that cannot navigate due to speech issues.''}
% \end{quote}

% --------------------------------------------
% \subsubsection{Implications on Speech Systems}


==> CHI2023 Stuttering/sections/3b-survey-findings.tex <==
\subsection{Survey Findings}
We present survey results including an overview of speech interaction and usage, challenges related to both VAs and dictation, and factors beyond technical considerations that could impact future adoption.

\subsubsection{Speech Interaction Usage and Utility} 
Most participants were familiar with speech recognition systems (VA: 100\%, n=61; DS: 90.2\%, n=55), although more had used VAs (96.7\%, n=59) than dictation (73.8\%, n=45).
%For those who were familiar with each technology, there was wide variability in how often they used it, as shown in Figure~\ref{fig:freqUseAndPerceivedAccuracyVAandDictation}; note that two participants did not report frequency of use, so this analysis includes 59 responses for VAs and 53 responses for dictation. 
Overall, among participants who were familiar with the given technology, VAs were used significantly more often than dictation (Mann-Whitney U test\footnote{We used a Mann Whitney U test because this is ordinal data and the data was not fully paired---not all participants who had used VAs had also used dictation. This analysis excludes the two participants who answered ``I don't know'' for their usage of VAs and dictation. Participants who were familiar with but had not used a given technology were combined with those who had used it but reported their current usage frequency as ``never,'' as shown in Figure~\ref{fig:freqUseAndPerceivedAccuracyVAandDictation}.}: $U=1937$, $n_1=59$, $n_2=53$, $p=.019$).
As shown in Figure~\ref{fig:freqUseAndPerceivedAccuracyVAandDictation}, about half of the participants familiar with VAs used one on a daily (32.2\%, n=19/59) or weekly basis (20.3\%, n=12/59),
% daily+weekly = (52.5\%, n=31/59)
whereas fewer used dictation on a daily (15.1\%, n=8/53) or weekly basis (24.5\%, n=13/53). 
%(39.6\%, n=21/53)
This VA usage rate is somewhat lower than recent estimates for the general population in the US that suggest 57\% use VAs daily and 23\% do so weekly \cite{npr_smart_audio}, perhaps reflecting the accessibility barriers faced by PWS. 
% survey- and interview-based study
%In their study, it was estimated that, from among 62\% of VA users in America, 57\% use one at least daily, 23\% at least weekly, and 20\% at least monthly.

Because past work has shown that stuttering severity affects speech recognition accuracy~\cite{mitra2021}, we further examined the relationship between A\&H severity ratings and reported dictation and VA usage. These results, shown in Figures~\ref{fig:usage_frequency_by_severity_future_tech} indicate no clear patterns based on graded severity. Kruskal Wallis tests did not reveal significant impacts of A\&H severity level (i.e., mild, moderate, and severe) on reported frequency of use for either VA usage or dictation usage.\footnote{A Kruskal Wallis test is a non-parametric equivalent to a one-way ANOVA, and is appropriate for ordinal data such as our frequency of use ratings (i.e., 1-At least daily, 2-At least weekly, 3-At least monthly, 4-Less than monthly, 5-Never). We conducted two separate Kruskal Wallis tests to examine the effect of the independent variable of A\&H severity level (mild, moderate, or severe) on the dependent variable of frequency of use for each of VA and dictation use. The tests were not significant at $p < .05$ for both VAs ($H(2)=0.57$, $p=.752$) and dictation ($H(2)=1.53$, $p=.465$). These analyses were conducted on $n=57$ participants (VA) and $n=43$ (dictation) who had reported experience with the given technology and frequency of use.} This lack of significance may be due to low statistical power related to our sample size and variability in how people rate their frequency of use, but we return to additional considerations in Section~\ref{sec:discussion}.

Turning to \textit{how} and \textit{why} participants adopted VAs and dictation, we first examined what platforms they used.
Among people with experience using VAs or dictation, phones were the most common platform (VA: 84.7\%, n=50/59; DS: 88.9\%, n=40/45) followed by smartwatches (VA: 25.4\%, n=15; DS: 24.4\%, n=11) and car infotainment systems (VA: 25.4\%, n=15; DS: 20.0\%, n=9). Smart speakers were also relatively common for VA use (47.5\%, n=28) but not used as much for dictation (9.0\%, n=4)---which is expected given that smart speakers are often communal devices and have fewer dictation use cases. Ten or fewer participants had used speech on tablets or traditional computers for both VAs and dictation.

\begin{figure}[h!]
    \centering
    %\subfloat[\centering label 1]{{\includegraphics[width=0.33 \paperwidth]{figures/truncation_rates_boxplot.png} }}%
    \subfloat[\centering ]{{\includegraphics[width=0.35 \paperwidth]{figures/Frequency_of_VA_and_dictation_use_with_labels.png} }}%
    \qquad
    \subfloat[\centering ]{{\includegraphics[width=0.35 \paperwidth]{figures/Frequency_of_speech_recognized_with_labels.png} }}%
    \caption{(a) Frequency with which participants \textit{who were familiar with} VAs and/or dictation use each technology, showing significantly greater use of VAs; two participants who responded ``I don't know'' are not included. (b) Frequency with which participants feel different recipients, including VAs, dictation, and other people, understand their speech accurately. For dictation and VAs, this analysis includes participants who had reported experience using each technology (n=44 for dictation because one participant did not answer this question). Overall, for both VAs and dictation, the majority of participants felt these systems understood their speech at best `sometimes,' in contrast to much higher comprehension rates when speaking to other people.}%
    \label{fig:freqUseAndPerceivedAccuracyVAandDictation}
    \Description{
    Figure (left): Bar charts for frequency of usage for VA and Dictation, ranging from had not used to daily use. See text in the paper for percentage breakdowns. 
    Figure (right): Bar charts for perception of how often recipient’s think systems (VA or Dictation) or people (strangers/acquaintances/friend & family) understand their speech. These rang from Never to Always. People tend to think that VAs understand their speech a little more often than Dictation (see paper for details). For around 93\% of PWS, friends and family always or often/usually understand them, which decreases to 74\% for acquaintances and around 67\% for strangers. In contrast, responses for sometimes, and rarely have similar patterns increase, meaning that PWS do not think they are understand as well by people they are less familiar with. The percentage of participants who are always or often/usually understood by VAs is around 46\% and this number is 39\% for
    Dictation.
    }    
\end{figure}
\begin{figure}[h!]
    \centering
    \subfloat[\centering ]{{\includegraphics[width=0.4
    \paperwidth]{figures/freq_use_by_severity_with_labels.png} }}
    \qquad
    \subfloat[\centering ]{{\includegraphics[width=0.30 \paperwidth]{figures/Interest_in_future_technology_with_labels.png} }}
    \caption{(a) Dictation and VA usage frequency based on A\&H severity ratings for participants \textit{who were familiar with} VAs (left) and those \textit{who were familiar with} dictation (right), showing varied usage frequency regardless of graded severity. Most respondents have reported use of VAs (n=59) and dictation  (n=53). Two respondents who said answered ``I don't know'' for VA and dictation frequency were not included in this analysis. 
    (b) Interest levels in future hypothetical speech technologies that can understand speech with dysfluencies accurately (n=61), showing high interest in general speech technology, as well as VAs and dictation.
    }
    \label{fig:usage_frequency_by_severity_future_tech}
    \Description{
Figure (left): Bar charts for “VA use by A&H severity” and “Dictation use by A&H severity” with values of Never/less than monthly/more than monthly/at least weekly/at least daily, broken down by mild/moderate/severe participants. There are a higher percentage of people with severe A&H severity ratings that chose ‘never’ than moderate, and more moderate that chose ‘never’ than mild. 
Figure (right): Bar charts for “Interest in Future Accurate Speech Technology” ranging from Not at all/not very/somewhat/very/extremely. See the paper for breakdowns, but generally people at least 50\% are extremely or very interested.
    }
\end{figure}






For why they use speech technology, a majority of participants find speech recognition systems to be at least ``somewhat'' useful; see Table~\ref{tab:perceived_utility}a for detailed utility ratings.
%(VA: 72.9\%, n=43/59; DS: 77.8\%, n=35/45)
% and many found them to be very or extremely useful (VA: 27.3\%, DS: 38.9\%)
%: `extremely' (VA: 10.2\%, n=6; DS: 8.9\%, n=4), `very' (VA: 30.5\%, n=18; DS: 31.1\%, n=14), and `somewhat' (VA: 32.2\%, n=19; DS: 37.8\%, n=17). 
% For VA users, common use cases mirror how the general population uses VAs~\cite{AmmariCHI21}, with tasks like listening to music (69.5\%, n=41), making phone calls (69.5\%, n=41), asking general questions (66.1\%, n=39), checking the weather (61.0\%, n=36), and setting alarms (52.5\%, n=31) and timers (50.8\%, n=30) being especially common. 
For those surveyed that use VAs, common use cases generally mirror those from the general population~\cite{AmmariCHI21}. 
For VA users (Table~\ref{tab:perceived_utility}b), participants most commonly reported listening to music, making phone calls, asking general questions, checking the weather, setting alarms and timers, and sending messages.
% For dictation users, common use cases included writing text messages (93.3\%, n=42/45), taking notes (37.8\%, n=17), writing email (18.0\%, n=11), and dictation within a web browser (16.4\%, n=10).
For dictation users (Table~\ref{tab:perceived_utility}c), the common use cases were writing text messages, taking notes, writing email, and dictation within a web browser.
However, about a quarter of participants familiar with each of the two speech technologies felt that they were `not very' 
%(VA: 15.3\%, 9/59; DS: 20.0\%, n=9/45) 
or `not at all' %(VA: 11.9\%, n=7; DS: 2.2\%, n=1) 
useful.
Overall, reasons were split between participants who saw no inherent value in VAs (e.g., \textit{``I haven't felt a need for them in my life''} [P2-51]) and those who encountered accessibility challenges due to stuttering (e.g., \textit{``[...] I often have to repeat myself so many times for it to understand me that it’s quicker and easier for me to just use my hands [...]''} [P2-64]). 
%and [P1-63] wrote, \textit{``It takes longer for me to speak/stutter [by] using voice assistants than it would for me to type what I need.''}
%The impacts of speech recognition errors and comparative efficiency of typing came up with dictation as well.
%As [P2-77] said, \textit{``because as a person who stutters I use fillers like umm, so, use a lot of repetitions, and also have frequent blocks and when I use dictation it writes down all my disfluencies that when I read the text it makes no sense.''} 
%For other participants, the utility of dictation depended on the words and length of the task, as reflected by [P1-60]: \textit{``When I am using words I can say well it works good, when I have to use words that I am unable to say clearly it does not work at all.''} 
We examine these and other challenges in more detail in the following sections.

\begin{table*}
% \hspace{-2em}
% \begin{subtable}[]{0.33\textwidth}
\begin{subtable}[]{0.33\textwidth}
    % \centering
    \begin{tabular}{|l|cc|cc|}
    \hline
    & \multicolumn{2}{c}{\textbf{VAs}} & \multicolumn{2}{|c|}{\textbf{Dictation}} \\
    % \textbf{Utility Rating } & \textit{n} & \textit{\% of 59} & \textit{n} & \textit{\% of 45} \\
    \textbf{Utility } & \textit{n} & \textit{\% of 59} & \textit{n} & \textit{\% of 45} \\
    \hline
    % Extremely useful & 6 & 10.2\% & 4 & 8.9\% \\
    % Very useful & 18 & 30.5\% & 14 & 31.1\% \\
    % Somewhat useful & 19 & 32.2\% & 17 & 37.8\% \\ 
    % Not very useful & 9 & 15.3\% & 9 & 20.0\% \\
    % Not at all useful & 7 & 11.9\% & 1 & 2.2\% \\
    Extremely & 6 & 10.2\% & 4 & 8.9\% \\
    Very & 18 & 30.5\% & 14 & 31.1\% \\
    Somewhat & 19 & 32.2\% & 17 & 37.8\% \\ 
    Not very & 9 & 15.3\% & 9 & 20.0\% \\
    Not at all & 7 & 11.9\% & 1 & 2.2\% \\
    \hline
    \end{tabular}
    \caption{} \label{capA}
\end{subtable}
\hfill
\begin{subtable}[]{0.32\textwidth}
    % \centering
    \begin{tabular}{|l|cc|} \hline
    \textbf{VA Uses}        & \textit{n} & \textit{\% of 59}  \\ \hline
    Music                        & 41         & 69.5\%              \\
    Phone calls                   & 41         & 69.5\%              \\
    General Q\&A            & 39         & 66.1\%              \\
    Weather                      & 36         & 61.0\%                \\
    Alarms                       & 31         & 52.5\%              \\
    Sending messages & 31 & 52.5\% \\
    Timers                       & 30         & 50.8\%              \\ \hline 
    \end{tabular} 
    \caption{} \label{capB}
\end{subtable}
% \\
\hfill
\begin{subtable}[]{0.25\textwidth}
    % \centering
    \begin{tabular}{|l|cc|} \hline                             
    \textbf{Dictation Uses} & \textit{n} & \textit{\% of 45} \\ \hline 
    Texting                      & 42         & 93.3\%              \\
    Notes                        & 17         & 37.8\%              \\
    Email                        & 11         & 24.4\%              \\
    Web browser                    & 10         & 22.2\%             \\ \hline 
    % \end{tabular}
    \end{tabular}
    \caption{} \label{capC}
\end{subtable}
\caption{(a) Perceived utility ratings from survey participants who had experience with VAs and dictation. Most found VAs and dictation to be at least ``somewhat'' useful, although about a quarter found them to be ``not very'' or ``not at all'' useful. (b and c) The most common use cases reported by at least 50\% of participants who had experience with VAs and by at least 20\% of participants who had experience with Dictation.  
}
\label{tab:perceived_utility}
\end{table*}

\subsubsection{Voice Assistant Challenges}
To understand the range of challenges PWS face when using VAs, we asked about what factors prevented participants who were familiar with VAs from using them more often. The most common were `voice assistants cut off my speech before I finish talking' (61.0\%, n=36/59) and `voice assistants don't understand my speech well enough' (57.6\%, n=34). Indeed, as shown in Figure~\ref{fig:freqUseAndPerceivedAccuracyVAandDictation} (b), a majority of participants (54.2\%, n=32) felt VAs only recognized their speech `sometimes' or worse. As a result, many participants (37.3\%, n=22) reported `often' or `always' attempting to revise what they say due to inaccuracies in speech recognition. 
%Of 33 people who reported on how often revision is effective, only 42.4\% (n=14 of 33) said `always' or `often,' while an additional 45.5\% (n=15 of 33) said `sometimes.'  
%In addition, 52.4\% of individuals cannot `often' invoke a wake word. 
Other concerns, however, were not purely technical. 
Twenty-two participants (37.3\%) reported not wanting other people to hear them talking to the VA, reflecting a social consideration that past work has also identified~\cite{bleakley2022exploring}. 
As well, many participants (22.0\%, n=13) cited that it takes `too much physical effort for me to speak.' 
Only six participants (10.2\%) responded that perceived utility of voice assistants prevented them from using the technology more often. 
%Below, we elaborate on experiences with endpointing and invocation, both of which are more important for VAs than dictation, as well as on the experiences of non-adopters.

Concern with endpointing---being cut off too soon---is typically more relevant to VAs than dictation, and was identified as a challenge in Bleakley et al.'s~\cite{bleakley2022exploring} interviews on VA use with 11 PWS. Our data demonstrates the pervasiveness of this problem: almost half of participants stated that VAs cut them off `always' (3.3\%, n=2) or `often' (37.7\%, n=23), while an additional 31 participants (50.1\%) reported being cut off `sometimes' or `rarely.' For the 57 participants who had at least some experience being cut off, when asked if they knew why it happened, by far the most common explanation was that there was a pause or block in their speech and the system thought they had finished speaking (77.2\%, n=44 of 57). 
% For example, participants wrote: \textit{``[The VA cuts me off] Because I have a break in speaking due to stuttering''} [P2-49] and 
% \textit{``They cut me off because they don't realize I'm blocking''} [P2-29]. 
Being cut off could also have consequential impacts, such as a poor user experience described by [P2-42]: \textit{``The [smart speaker] which I use most often does not like any hesitations in speech. It assumes the slightest pause means the person is done speaking. So I get cut off often. It creates a sense of having to rush which makes my speech worse.''} And, as [P2-77] described, impacts can also be emotional: \textit{``I block a lot on my name and vowel words so when I take time to talk it is frustrating when they cut me off [...] I have to deal with people often trying to speak for me and having a voice assistant doing that because I can't have one who understands my speech rhythm makes me not want to use it even more.''}
We address endpointing errors in Section~\ref{sec:endpointer} and significantly reduce the problem on our dataset of speech samples.

Some smartphones (e.g., Apple iPhone) offer an alternative to automatic endpointing, where the user can push down a button (physical or virtual) while speaking and only release it when done.
%, although this is not available on screen-free devices like smart speakers. 
Twenty-seven participants (44.3\%) reported using a device that supports this functionality. Of those 27, almost all found being able to press a button and speak to be useful: 51.9\% (n=14 of 27) `extremely useful,' 18.5\% (n=5) `very useful,' and 29.6\% (n=8) `useful.' Reasons provided for this utility were most commonly that it eliminates being cut off, but some participants also explicitly referred to a psychological impact of feeling less rushed or worried, such as: \textit{``I can fully get my phrase in without worrying about blocking''} [P1-62] and \textit{``I don't feel rushed to finish what I need to say''} [P1-45]. 

%\paragraph{Invocation}
Another potential issue unique to VAs is invocation.
% \note{A note to remind bringing this up in Discussion} 
Most VAs use a wake word like ``Alexa,'' ``OK Google,'' or ``Hey Siri'' for invocation, which can be difficult for some PWS to use. Almost half of participants reported that these wake words `always' (11.5\%, n=7) or `often' (36.1\%, n=22) worked for them. 
But, problematically, 17 participants (27.9\%) reported wake words only working `sometimes' and 8 participants reported `rarely' or `never' (13.1\%); the remaining participants had not used a wake word. 
While we did not ask participants to elaborate on their use of wake words, a handful of responses to other open-ended questions referred to challenges with wake words, including [P2-1] who stated \textit{``Problem with wake words is my biggest frustration. I would want to change it to something I can say easily''}. 
While popular consumer systems do not allow for arbitrary wake words, some offer multiple options (e.g.,
% One potential solution is to allow users to change the wake word---
Alexa has at least five options and Google Assistant has two). 
% Although multiple options is progressive to be potentially more inclusive, these responses indicate that current choices for wake words can be improved. 
% , and Siri has one.
Additionally, a few participants mentioned that pressing a button to talk (as described above) eliminated issues with wake words by allowing an alternative explicit signal that the user is ready to talk. [P1-28] noted \textit{``It's [Hold/Squeeze to Speak is] useful on my phone to bypass the lag that occurs when [the VA] does not recognize me using the wake phrase''}, and [P1-73] uses it \textit{``Because it knows when to start listening and when I'm done.''}

%In summary, PWS desire VA systems to be more accommodating of stuttered speech patterns, especially the pauses that can result in being cut off mid-utterance, and in increased overall speech recognition accuracy.


\subsubsection{Dictation System Challenges} 
As with VAs, we aimed to broadly understand what factors impact dictation adoption for PWS. When asked what reasons prevent them from using dictation more often, 56.4\% (n=31) of the 55 participants who were familiar with dictation noted that `dictation tools don't understand my speech well enough.' Of those who had used dictation, a majority (59.1\%, n=26 of 44 who answered this question) felt the ASR only recognized their speech accurately ``sometimes'' or less (Figure~\ref{fig:freqUseAndPerceivedAccuracyVAandDictation}, right). As a result of these errors, participants reported attempting to revise or restate what they say, with about half of participants doing so `always' (6.7\%, n=3/45) or `often' (42.2\%, n=19), and an additional 35.6\% (n=16) doing so `sometimes.'
Finally, and similar to VAs, participants also commonly cited non-technical reasons for not using dictation more, most notably the physical effort it takes to speak (32.7\%, n=18 of the 55 familiar with dictation) and not wanting other people to hear them dictate to the device (30.1\%, n=17). Additionally, 11 participants (20.0\%) reported that low utility prevented them from using dictation more often, and 12 (26.7\%) felt that they use more refined language when they type than when they speak. 
%Here, we elaborate on experiences with speech recognition errors, which are more prominently surfaced to the user with dictation compared to with VAs, and on the experiences of non-adopters.

In contrast to VA systems, which predict the most likely command based on a spoken phrase, with dictation the user's speech is transcribed verbatim. This difference is reflected in participants' experiences with dictation errors. 
%While 37.8\% of the 45 participants who had used dictation felt these systems recognized their speech `always' (n=1) or `often' (n=16), a majority of participants encountered difficulties. Half the participants (51.5\%, n=23) felt dictation only `sometimes' recognized their speech accurately, and the remaining five (11.1\%) felt their speech was `rarely' recognized well. 
When asked an open-ended question about what types of errors tend to occur with dictation, by far the most common response, mentioned by a majority of participants, was errors in the ASR transcription (e.g., \textit{``Message contains different words than I intended''} [P2-5]). 
Some participants (13.3\%, n=6) also mentioned being cut off, although this was a much less common error than with VAs because many dictation systems do not use an automatic endpointer. 
A few participants mentioned poor performance with punctuation, proper nouns, and slang. 
Finally, some participants mentioned specific stuttering characteristics and challenges, including their repetitions being displayed in the transcribed text
(\textit{``Misunderstood due to repetition or actually repeats word''} [P2-46]), the impact of blocks 
(\textit{``words that I have a block in the middle of will turn into a strange phrase''} [P2-51]), and interjections being shown, as described by [P2-77]: \textit{``because I have blocks and use filler words, the fillers are listed on the text message all my disfluencies are written down and when I read over the text it makes no sense and I have to type it myself instead because I will never be fluent all the time.''} 


% \paragraph{What would make uninterested participants interested?}
\subsubsection{Beyond Technical Considerations} 
% \paragraph{An Ideal Speech Recognizer}
The findings above suggest that technical improvements in invocation, endpointing, and ASR accuracy should be welcomed by many PWS and ultimately increase adoption of speech technologies by this population. However, future adoption also depends on factors beyond technical improvements, 
% as touched on already by references to
such as social concerns and the physical difficulty of speaking, emphasizing that speech input may not be relevant to all users even with substantial accuracy improvements. 

%Lastly, in open-ended responses, multiple people noted that being misunderstood can be stressful or induce negative emotion. 
%    [P2-77] \textit{``I want it to be inclusive to all individuals who stutter, stammer clutter [...] we should be able to feel confident speaking in any devices and not feel inferior because [...] it was made for the population that doesn't have a speech impediment.''}, 
%    [P2-36] \textit{``It works for everyone but me. Even though I have virtually no interest in using them, it sucks that the option isn't even available to me.''}, 
%    and [P2-8] \textit{``The forcing of the technology on those that cannot navigate due to speech issues.''}

To begin to understand what future adoption might look like,
% assuming technical improvements can be made,
we asked participants to imagine speech technologies that can accurately understand their speech. 
Within this context, most participants were at least `somewhat` interested in VAs (86.9\%, n=53/61): `extremely’ (n=25), `very' (n=13), `somewhat' (n=15), `not very' (n=7), `not at all' (n=1) and similar for dictation (Figure~\ref{fig:usage_frequency_by_severity_future_tech}, right). 
% In open-ended responses explaining their interest level, 
Positive responses reflected earlier feelings about VAs and dictation, notably increasing efficiency, ease and convenience, being able to do actions hands-free (including while driving), and generally having confidence in the system. 
For example, [P1-66], who currently uses VAs at least monthly and has not tried dictation wrote, \textit{``I would be extremely interested in this, especially knowing it's something I don't have to worry about the speech input being able to understand me. It would remove my hesitancy and frustration with my stuttering from the equation.''} 



%\begin{figure}[t!]
%    \centering
%    %\includegraphics[width=0.3 \paperwidth]{figures/Frequency of VA and dictation use.png} 
%    \includegraphics[width=0.33 \paperwidth]{figures/Interest in future technology.png}
%    \caption{Interest levels in future hypothetical speech technologies that can understand speech with dysfluencies accurately %(n=61), showing high interested in general speech technology, as well as VAs and dictation.}
%    \label{fig:futureInterest}
%\end{figure}

However, the negative and neutral reactions to this future technology scenario indicated a preference for typing, seeing no need for speech input, and value depending on context (e.g., \textit{``It would depend on the device''} [P1-64], who uses VAs weekly and dictation less than monthly). 
% they are not interested in speech technology
This preference for typing by some participants also arose in other responses throughout the survey, reflecting in some cases the physical effort required to speak. 
% (which had been a concern of some participants, as reported earlier). 
For example, \textit{[P2-73] said, ``It's a nice thought but it's still easier for a person who stutters to type most of the time. Unless our hands are filthy or tied up''} and \textit{[P2-87] ``It still requires effort to speak even if it understand me perfectly, and I am good at controlling them manually.''} 
In addition, 9.8\% (n=6) stated  `voice assistants don't seem useful.' 
while [P2-51] said, \textit{``I'm not sure. As someone who stutters, and just situationally in my life, I can't imagine dictation regularly being a more convenient option than typing.''} 

Additionally, social factors may influence future adoption, a consideration touched on in past work with PWS~\cite{bleakley2022exploring}. 
While the survey did not explicitly ask participants about the social context of speech technologies, as already noted, many participants felt that having to speak in front of other people limited their willingness to use speech technology. For example, [P2-1] wrote \textit{``[...] I would be reluctant to use voice commands in public because of my speech impediment''}, and [P1-58] wrote, \textit{``I still would not use it at work. I would use it in spaces where I am alone, with my spouse or family.''} 
Some participants also commented on how anxiety affects their stuttering, which translated to speech technology use in different ways. [P2-88], for example, expressed that \textit{``...before I am about to use voice recognition I get a bit nervous because I think that I have to speak without stuttering for it to work''}---a concern that could be alleviated with improved ASR. 
At the same time, some participants expressed that speaking to devices  reduces anxiety compared to speaking to other people, including: \textit{``I don't stutter much when talking to myself so I usually don't experience this problem [dictation errors]''} [P2-15] and \textit{``I usually stutter in high anxiety situations not when I'm by myself''} [P2-70]. Depending on the individual person and the context of use, these social factors could prove to be barriers to adoption.

%\note{We removed the Adaptive Tech section(commented out below) entirely, do we still want to bring it up in Discussion?}

\subsection{Summary}
This survey shows that many PWS are using speech technology on a regular basis, albeit at lower rates than the general population (at least for VAs). However, accessibility challenges include being cut off or misunderstood by VAs, and having stuttering events such as repetitions and prolongations result in transcription errors with dictation. Many participants were interested in using future technologies that could recognize stuttered speech accurately, but other responses suggest that a subset of PWS would still choose not to use such technology due to the physical effort of speaking and social considerations.


%\subsubsection{Adaptive Tech \todo{consider removing these two paragraphs}}
%Finally, we asked participants about two potential technologies that could improve accuracy for an individual user with atypical speech. 
%The first was around a personalized speech recognition system that could  recognize the participant's speech well, \textit{``but you need to spend time teaching it, perhaps by reading a set of phrases into the device.''} Of the 58 participants who responded to this scenario, most (n=47) had some interest: `extremely' (27.6\% of 58, n=16), `very' (20.7\%, n=12), or `somewhat' (32.8\%, n=19). These 47 participants were roughly evenly split between being willing to spend only 1-5 minutes on training and spending 10-30 minutes on training; however, 12 were willing to spend even longer. One said they were not willing to spend any time. For the 11 participants who were either `not very' or `not at all' interested in training a system, the most common concern was the time and effort required. One participant, however, noted a potential issue, \textit{``My speech changes from day to day. In the middle of a bad speech day I don’t want to talk more''} [P1-55].

%The second technology imagined a VA that works very well but only supports a small set of perhaps 10 to 20 high-value commands. Of the 59 participants who responded to this question, most (n=40) felt it would be useful: `extremely' (20.3\%, n=12), `very' (23.7\%, n=14), and `somewhat' (23.7\%, n=14). Some participants expressed the sentiment that they do not use many commands anyway, such as, \textit{``I usually only use my [device] for the same things over and over again so this would be useful''} [P2-73]. However, those who did not think this approach would be `very useful' (27.1\%, n=16) or `at all useful' (5.1\%, n=3) commonly had \textit{``no need for voice assisted technology''} [P2-44] or felt that \textit{``10-20 commands is not enough''} [P1-63].


==> CHI2023 Stuttering/sections/4b-findings-asr.tex <==
% \section{Speech Recognition Experiments}\label{sec:asr_results}
\section{Speech Recognition Technology: Data \& Experiments}\label{sec:asr_results}

% \todo{in paper intro, mention detailed annotations}

Building on findings from the survey, we turn to recorded speech data from 91 PWS (53 of whom also completed the survey). We quantify how dysfluencies in speech from PWS manifest in the types of recognition errors encountered by survey participants. We also investigate changes to three stages of the speech pipeline introduced in Section~\ref{sec:rw-speechrecsystems} that address issues identified in the survey. 
We focus on interventions that build on pre-trained production-grade models, as oppose to training from scratch, so we can optimize on relatively small amounts of data from PWS: 
\begin{enumerate}
    \item \textit{Tuning the endpointer model} using speech from PWS, to reduce speech truncations (cut-off speech).
    \item \textit{Tuning the decoder in the ASR model} using speech from PWS, to increase ASR accuracy. 
    \item Applying posthoc \textit{dysfluency refinements} to ASR transcriptions to remove dysfluencies such as repeated words.
\end{enumerate}
%Here we introduce the stuttered speech data, perform baseline speech recognition experiments, with emphasis on endpointing and speech transcription, and investigate areas for improvement through ASR Tuning and Dysfluency Refinement. 


\subsection{Speech Data Collection}\label{sec:speech_data}
% Survey (61): Counter({1: 12, 2: 31, 3: 18})
% Phase 1: (50): Counter({1: 25, 2: 18, 3: 7})
% Phase 2 (41): Counter({1: 2, 2: 12, 3: 27})
% Intersection of (S, P1, P2) (99): Counter({1: 25, 2: 48, 3: 26})
% Intersection of (P1, P2) (99): Counter({1: 25, 2: 44, 3: 22})

Participants were asked to record themselves speaking 121 VA commands and up to 10 Dictation phrases that they could imagine saying to a smart speaker or device.
An initial cohort of 50 participants (Phase 1: 25 mild; 18 moderate; 7 severe)\footnote{A\&H severities were computed using the same process as with the speech survey.} was collected starting in Summer 2020 and 41 additional (Phase 2: 0 mild; 26 moderate; 15 severe) in 2021.\footnote{65 participants successfully recorded 131 utterances, 2 recorded 130 utterances, and 24 only recorded 121 VA commands.} 
% 65x - 131; 2x - 130; 24x - 121
VA phrases were based on prompts where participants came up with their own utterance to accomplish a given task. 
This was designed to prevent participants from simply reading pre-defined phrases in a monotone manner, 
and some examples include ``Find out when a place you might want to visit will open,'' ``Find the lyrics to a song that you like,'' and ``Ask a question about something that is not well known.''
Dictation phrases consisted of fake text messages that they might send to a friend. 
% Participants were asked to record 121 clips that they could imagine saying to a smart speaker or device using Voice Assistant related prompts. 
% Most individuals (67 of 91) were also asked to record 10 clips consisting of fake text messages that they might send to a friend, which are more appropriate for the Dictation use case. 
% Our initial cohort of 50 participants (Phase 1: 25 mild; 18 moderate; 7 severe)\footnote{A\&H severities were computed using the same process as with the speech survey.}
% \note{zifang: All Phase 2 participants have 131 audios except one who has 130 audios. 24 participants in Phase 1 have 121 audios, 25 has 131 audios, and 1 has 130 audios. For later IER report, Phase 2 IER can be seen as average by itself.}
% An additional 41 participants (Phase 2: 0 mild; 26 moderate; 15 severe) recorded the same 121 Voice Assistant related prompts and an additional 10 clips consisting of fake text messages that they might send to a friend, which are more appropriate for the Dictation use case. 
Audio clips were captured using a smartphone on their own in a quiet environment where participants were asked to speak naturally. 
% while holding the device or placing in front of them two to three feet from their head. 
% and were told not to include personal or identifiable information (PII). 
The median utterance length was 6 words. 

% An outside SLP assessed each participant's severity as part of the screening process. 
% Participants were asked to read paragraphs and have free dialogues for the severity ratings and these are not part of the collected data.
% A complete set is included in the Supplemental Material \note{Can we include?}. 

% This study was carried out in two phases with 50 participants in Phase 1 (25 mild; 18 moderate; 7 severe) and 41 in Phase 2 (0 mild; 26 moderate; 15 severe).
All audio clips were manually transcribed with both the articulated phrase with dysfluencies (e.g., ``wh-(at) wh-(at) what is [...] the weather'' and the phrase that annotators believed the participant intended to say (e.g., ``what is the weather''). For each phrase, one human transcriber created an initial transcript and a second person reviewed the transcript; additionally, a random ~15\% of transcripts were spot checked by a third independent reviewer for quality control and were redone if needed.
% The ``intended phrase'' was determined by an annotator, where and in most cases 
For the 41 participants in Phase 2, which has a larger percentage of those with moderate or severe dysfluency rates, the transcripts were annotated with detailed dysfluency labels.
%that allowed us to assess the impact of dysfluency type on recognition performance. 
Specifically, for each phrase, an annotator segmented each dysfluency event by marking the start and end frames, and added one of the following five dysfluency labels: part-word repetition (e.g., ``ha- ha- ha- happy''), whole word repetition (e.g., ``I I I''), sound prolongation (``wasss''), blocks (audible and inaudible), and interjections (e.g., ``uh'', ``um'').
% , ``you know'', but not ``like'' because it is commonly also used as a standard word). 
These annotations also went through a similar QA process where dysfluencies with incorrect timestamps or labels were marked as wrong. 

Across all clips with dysfluency annotations,  58.6\% of utterances contain one or more part-word repetitions, 5.5\% contain one or more whole word repetitions, 36.4\% prolongations, 38.7\% blocks and 2.8\% interjections.
Interjections were very common with one participant but less prevalent more broadly.
The rarity of interjections may be due to the short utterance lengths.
%This is in contrast with  --  likely due to the short utterance lengths and nature of the prompts\note{is this clear to the audience that it means PWS don't need buffers in such cases?}. 
%along with results from Section~\ref{sec:asr_baselines}. 
In general, the distribution of dysfluency types varies greatly on a per-participant basis. Some individuals frequently block but have few repetitions whereas others have frequent repetitions but few blocks. 
We look more at connections between dysfluencies and WER throughout our speech recognition experiments.

%Dysfluency rates chart
%Figure~\ref{fig:dysfluency_rates} depicts the rates of different types of dysfluencies, which varies substantially across participants, where we define dysfluency rate as the number of dysfluencies of that type per participant divided by the number of intended words. 
%This figure, while complicated, is intended to highlight two pieces of information. First, this depicts, quantitatively, how the distribution of dysfluencies varies across participants. \note{maybe this's redundant, I find it helpful to point out: On a higher level(by looking at each sub-graph horizontally), part-word repetitions, prolongation and blocks are more prevalent across all participants.} The order of participants in each sub-figure is the same, so by looking across graphs one can characterize dyfluency prevalence per-person. 
%For example, some people tend to have much higher rates of part-word repetitions, prolongations, or blocks. 
%Second, this connects dysfluency rates with word error rates using the baseline results discussed later in Section~\ref{sec:asr_baselines}, where participant results are sorted left-to-right based on their average WER from best-to-worst.
%Interestingly, the people with the highest WERs (e.g., participants P53 - P8 on the right) all have different distributions of dyfluency types. 
%We look more at connections between dysfluencies and WER throughout our speech recognition experiments.


% Speech from each participant was graded by the same speech language pathologist as in the survey using the Andrew and Harris Scale (A\&H) Scale~\cite{AndrewsHarris1964} on conversational speech and utterances that were not part of the recording process. 
% \todo{check that we actually introduce A\&H somewhere}
% \note{move as we don't use here} A second speech language pathologist estimated stuttering severity (no stutter, mild, moderate, severe) for each participant using the Andrew and Harris Scale (A\&H) Scale~\cite{AndrewsHarris1964} by grading 100-300 word audio clip samples.
% \textbf{Do we have an explanation for this?: Eight survey respondents did not have annotated data and were not included in the evaluation of speech recognition models.}.

% \note{move to discussion?}The process of creating these audio recordings -- which were done at an individual's convenience while by themselves -- undoubtedly biased the prevalence and severity of dysfluencies, as these are each variables that are known to impact stuttering \cite{tichenor2021variability}.
% For some users events were likely higher because they knew they were being recorded and for others were likely lower because they could do it when they felt most comfortable. 
% The setting or environment, current mood/stress level, communication partners, or other variables can impact stuttering \cite{tichenor2021variability}.

% \todo{Add paragraph talking about how dysfluency rates. See Figure \ref{fig:dysfluency_rates}}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.7 \paperwidth]{figures/DysfluencyPerWord_vs_WER_Spearman}
%     % \includegraphics[width=0.7 \paperwidth]{figures/DysfluencyPerWord_vs_WER}
%     \caption{
%     % \todo{TBD. One plan is to update this to 5 small scatter plots and maybe a box plot graph with one ``box'' for each dysfluency type. Move full participant detail to supplementary materials}
%     \note{CL: I commented out the text for this plot for the time being.}
%     Dysfluency rates by type and baseline speech recognition performance (WER) per Phase 2 participant. (top) WER and part-word repetition rate per participant. (middle top) WER and whole word repetition rate per participant. (middle bottom) WER and prolongation rate per participant. (bottom) WER and block rate per participant. 
%     Note that the distribution of dysfluency rates varies significantly per-participant. Spearman's rank correlation for each relates WER and dysfluency rate per type. 
%     % \todo{(1) middle fig: in tge legend, refering the overall WER number as Mean may not be right? (2)bottom fig: Only used Phase2 results. All numbers should be kept single digit.}
%     % \todo{reference in text}
%     % \todo{the r and p values are slightly different in our calculations, I may adopt Colin's as it's harder to make changes in figures and as the differences are very small}
%     }
%     \label{fig:dysfluency_rates}
%     \Description{
%         Figure: This is a set of 5 grouped bar charts showing per-participant Word Error Rates and Dysfluency Rates.* Each bar chart shows the rate of a specific dysfluency type and Word Error Rates where the x-axis are participant IDs sorted in order of increasing Word Error Rates and the left y-axis is the Word Error Rate and the right y-axis is the rate of a specific disfluency type. The Word Error Rates are the same for all the charts where there is a left-skewed long-tailed distribution and values range from 0.02 to 0.50. 
%         These charts show that not all disfluency types are correlated with Word Error Rate and that the distribution of dyfluencies are quite diverse, where some participants have much higher rates of blocks and others have higher rates in part-word repetitions. 
%         The first bar chart shows Word Error rate and part-word repetition rates. Part-word repetition rates range between 0 to 0.6 and positive correlations between Word Error Rate and Part-word repetitions can be observed as the height of the bars jointly increase. 
%         The second bar chart shows Word Error rate and whole word repetition rates, where similar positive correlations are observed, except there is one participant with a disproportionately high disfluency rate compared to WER rate. The values follow a long tail distribution where most values are below 0.025 and the rest are between 0.025 and 0.125.
%         The third bar chart shows Word Error rate and prolongation rates, where there is not a clear correlation as higher disfluency rates do not correspond to higher Word Error rates.
%         The fourth chart shows Word Error rate and blocking rates, where similar to prolongations, there is not a clear correlation.
%         The fifth chart shows Word Error rate and interjection rates, where there is not a clear correlation and not all participants have observable interjections. The participant who has the highest interjection rate also has the highest Word Error Rate and their interjection rate is over 5 times higher than the second highest interjection rate.
%     }
% \end{figure}


% \subsubsection{Speech Recognition Results}

% We used production-like models similar to what are deployed for Siri on iOS. Specifically, the endpointer, ASR model, and intent recognition component of the NLU model. 

% \todo{what details can we use? look at how we did it for the Interspeech paper. }


% Specifically, the endpointer, ASR model, and intent recognition component of the NLU model. 
% \todo{what details can we use? look at how we did it for the Interspeech paper. }

% The performance of a standard speech recognition models and models modified to better recognize  stuttered speech were evaluated on speech recordings collected from participants.  


% ----------------------------------------------------------------------------------------------------
\subsection{Speech Recognition Results}


In this section we present baseline performance for both endpointer and ASR models on our dataset, as well as results from the three interventions that address issues that arose in the survey: (1) endpointer tuning to address the problem of being frequently cut off by VAs, (2) ASR decoder tuning to improve the ability to understand stuttered speech, and (3) refining dysfluencies in the transcribed speech that is output from the ASR model to improve dictation experiences for PWS. We also place these findings in historical context by investigating how ASR performance on speech from PWS has changed over the past five years, using archived consumer-grade ASR models that were publicly available from 2017-2022.

The baseline models are from the 
Apple Speech framework~\cite{SpeechFramework}, which uses a hybrid deep neural network architecture for the ASR system.
% ~\cite{hinton2012HybridASR}. 
See \cite{huang2020sndcnn} for ASR model details, which at a glance is composed of an acoustic model, a language model, and a beam search decoder. %~\cite{freitag2017}. 
The acoustic model maps audio to phone- or word-like intermediate representations, a language model encodes the probability of word sequences and acts as a prior over what words or phrases someone may have said, and a beam search decoder that 
% model maps the acoustic outputs to 
efficiently computes candidate transcriptions.
% \begin{figure}
% \paperwidth]{figures/Simplified Workflow and Components of ASR}
% \end{figure}

% , sometimes with with a grapheme-to-phoneme model, 
% , which at a glance contains an acoustic model which picks up on low-level phoneme-like vocalizations, a language model which 
% with a self-normalizing acoustic model~\cite{huang2020sndcnn}, error-driven n-gram language model~\cite{gondala2021error}, and Beam Search decoder. 
% \note{consider moving some text from Background section to here}

% In addition, we share insights from clinical assessment of the data and the perceived role different stuttering characteristics play on performance. 

% The endpointer is comparable to that of [X] \etal~\cite{?}, the ASR models are a hybrid deep neural network architecture with a self-normalizing acoustic model~\cite{huang2020sndcnn}, error-driven n-gram language model~\cite{gondala2021error}, and Beam Search decoder. We also evaluate intent recognition performance using an NLU system comparable to that described by Chen \etal~\cite{chen2019active}. 
% In addition we analyze characteristics of the data and relate ASR performance to dysfluency rates, survey data, and clinical severity. 
% We then provide analysis on a baseline ASR and NLU system and show improvements after tuning the system our PWS using the approach of Mitra \etal~\cite{mitra2021}. 

% \note{This paragraph was moved from earlier; merge or delete.}
% At a high level, common consumer ASR models are often composed of three parts: an acoustic model that maps audio to phone- or word-like intermediate representations~\cite{huang2020sndcnn}, a language model that encodes the probability of word sequences and acts as a prior over what words or phrases someone may have said~\cite{?}, and a decoder model maps the acoustic outputs to words, sometimes with with a grapheme-to-phoneme model, typical using Beam Search to efficiently compute the TopK candidate phrases with highest probability~\cite{?}. 
% At a glance, many ASR systems use a hybrid ASR architecture (e.g., \cite{?}) composed of an acoustic model, a language model, and a decoder.
% Modern acoustic models are built using typical deep learning architectures such as ResNets or Transformers and output phone probabilities or latent embeddings~\cite{?}.
% A common approach is to use a hybrid ASR architecture(e.g., \cite{?}), which is composed of an acoustic model that detects thousands of context-dependent phones, a language model which learns associations between consecutive words, and a decoder that maps them together. 
% phones to graphemes. 
% In a hybrid ASR  then these components may be explicit or in an end-to-end system (e.g., \cite{?}) they may be implicit, however the overarching ideas are the same. 
% In a hybrid model, the input audio is first run through an acoustic model which takes the audio, in spectral form, and computes 1000s of context-dependent phones. 
% A language model encodes the probability of word sequences and acts as a prior over what words or phrases someone may have said~\cite{?}.
% These are regularly trained on large datasets with millions of documents, but may be biased towards words frequently uses for Voice Assistants. 
% The ASR used for VAs and DSs are conceptually the same, but typically optimized for specific tasks. For example, the decoder my bias a VA to output phrases commonly used for VA tasks. 
% The decoder model maps the acoustic phone outputs to words, with a grapheme-to-phoneme model, typical using Beam Search to efficiently compute the TopK candidate phrases with highest probability. 
% This decoder model can be tuned to optimize for different tasks so that the same Acoustic and Language models can be reused for VA, DS, and other systems.
% We look at the impact of optimizing a decoder in Section~\ref{sec:asr_results}.
% for PWS.
% There are many decoder parameters associated with Beam Search, for example to adjust the tradeoff between confidence in the acoustic and language models, the tradeoff of computational cost and candidate phrases, and even penalize for word insertions.


% First, we analyze the endpointer. 
% perform baseline speech recognition results using...

% --- Structure --- 
% * Endpointer
% * ASR Experiments. Baseline & Tuned ASRs
% * -- ?Metrics (Sentence-level WER, Dataset-level WER, Intents, WER<10)
% * -- dictation experiment
% * -- ASR over time
% * Analyses
% * -- WER vs severity, survey, dysfluency types
% * -- Clinical-guided analysis
% * Open questions
% Most existing speech systems are tuned on audio clips from people without known speech disorders (labeled \textit{non-PWS}), which contains mostly fluent speech. As such, we show improved baselines tuned specifically on a subset of our dataset from PWS. 

\subsubsection{Endpointer Model Performance} \label{sec:endpointer}
% Endpointer “model-feature-list": "num-trailing-sil,end-of-sentence,num-of-words,pause-counts,silence-posterior",
An endpointer model identifies when the user stops speaking, and must balance the desire for a low truncation rate (i.e., what percent of utterances are cut off too early) with the desire for a minimal delay after speech (i.e., time from the end of the utterance to when the VA stops listening). 
% \todo{Add mini model description}
Our base model is trained on completed utterances from the general population, and predicts the end of a query using both auditory cues like how long the user has been silent as well as ASR cues like the chance a given word is the final word of an utterance.
% non-PWS speakers.
% \footnote{Here we define non-PWS as data from the general population, which is assumed to have very little data from PWS.}
% https://compass.scv.apple.com/confluence/display/SiriPerception/Endpoint+Feature
% Here we use an endpointer that is comparable to that of [X] \etal~\cite{?}.
For each input frame (time window), the model outputs the likelihood of utterance completion. 
Once the output exceeds a defined threshold, the system stops listening and moves on to the next phase of processing.
% When tuned on non-stuttered speech these models tend to disproportionately cut off the speech of people who stutter. 

\paragraph{Baseline endpointer.} The baseline likelihood threshold from the model we used was set such that 97\% of utterances from the general population data are endpointed correctly (i.e., truncation rate of 3\%). When evaluated on our data from PWS, which is likely poorly represented in general population data, a much higher portion of data is truncated early. 
Across the 41 Phase 2 participants,\footnote{For consistency across later experiments where we use Phase 1 data to tune models, we only report performance here for Phase 2 data.} the baseline endpointer model truncates on average 23.8\% of utterances ($SD$=19.7, $Median$=16.8, $IQR$=29.0); see Figure~\ref{fig:boxplots_endpointer_and_wer}(a). Truncation rates also vary substantially per person---for 7 of 41 participants over 50\% of utterances are cut off early. This high truncation rate reflects the survey findings, where a majority of participants reported that early truncation was a key issue.
% preventing increased VA adoption.  

\begin{figure}[t!]
    \centering
    %\subfloat[\centering label 1]{{\includegraphics[width=0.33 \paperwidth]{figures/truncation_rates_boxplot.png} }}%
    \subfloat[\centering ]{{\includegraphics[width=0.33 \paperwidth]{figures/truncation_rates_boxplot.png} }}%
    \qquad
    \subfloat[\centering ]{{\includegraphics[width=0.33 \paperwidth]{figures/wer_asr_boxplots.png} }}%
    \caption{(a) Endpointer and (b) ASR performance for Phase 2 participants (N=41). In both cases, the tuned models are trained on Phase 1 data. The $\times$ symbol marks the mean in each box, whereas the solid internal line is the median. (a) Truncation rates are substantially lower than the baseline for all tuned thresholds, and the moderate threshold results in a rate of less than the 3\% targeted for the general population.  
    (b) For WER, the ASR decoder tuning and the dysfluency refinements significantly improve performance compared to the baseline, and the combination of the two results in a further significant improvement.  
    %\todo{Detailed WERs per participant can be found in Supplementary Material. CL: for the sake of time/effort maybe don't add this to the Supp?}
    }%
    \label{fig:boxplots_endpointer_and_wer}
     \Description{
    Figure (left): Box plot for endpointer truncation rate, with four boxes each representing baseline endpointer model and tuned models on speech data from participants with mild, moderate and severe A&H ratings. The tuned models reduce truncation rates from about 24\% to below 5\%.   
    Figure (right): Box plot for ASR performance (WER), with four boxes representing baseline ASR and tuned ASR models with or without dysfluency refinements. The ASR decoder tuning improves performance significantly,  for the third quartile. The dysfluency refinements further improve performance compared to the baseline for both the baseline and tuned ASR.
    }  
\end{figure}


Our hypothesis, based on the literature and understanding of stuttering, is that blocks, which are often expressed as inaudible gasps, cause most endpointing errors. 
We validated this using the dysfluency annotations by computed Spearman's rank correlation\footnote{\label{spearman_footnote}Spearman's rank correlation is used to correlate variables that are not distributed by a Gaussian distribution 
% such as data that is highly skewed, multi-modal, or discrete and ordinal.
such as our data that is highly skewed.}
% , multi-modal, or discrete and ordinal.Figure~\ref{fig:dysfluency_rates} and Figure~\ref{fig:WER} respectively shows dysfluency rates and WER across participants are multi-modal and thereby, is not Gaussian-distributed, hence we use Spearman's rank correlation.} 
and found truncation rates are significantly positively correlated with rates of blocks ($r(39)=.64$, $p<.001$), part-word repetitions ($r(39)=.44$, $p=.004$), and interjections ($r(39)=.48$, $p=.002$). Correlations with prolongations ($r(39)=.17$, $p=.301$) and whole word repetitions ($r(39)=.18$, $p=.271$) are not statistically significant. 

% \todo{ZF: Did we mention somewhere that why it's 39 out of the 41 Phase2 participants? CL: 39 is the number of degrees of freedom for the correlation, not number of users}. 
% \todo{CL: I think this was moved from elsewhere. Either rephrase or remove? re: zfh: This's from the previous Sec 4.2.5 Dyfluency Rates vs Usage. I integrated pieces from that para to 2 other places: The first is here. Second is in Dyfluency Refinement, second sentence in that the first para "This is shown by a moderately negative correlation between whole word repetitions ( r(20) = −.47, r = .013) and self-reported dictation usage." Ideally, I'd like to also mention something in the Baseline ASR para, but there's nothing to mark there --- I left a note there (top Page 16).  If we were to remove this here, we'll also remove the sentence in the Dysfluency Refinement paragraph.}
% \note{Extending this analysis to correlations between the rates of different dysfluency types and self-reported VA usage in the survey, we found that higher dysfluency rates typically occurred with lower usage frequency, with a significant moderate correlation for blocks ($r(29)=-.37$, $p=.024$), and no significant correlations with other dysfluency types. 
% The correlation with blocks resonates with the survey finding, and indicates that people are discouraged to use VA when they're cutoff }
% \note{Maybe we also want to include how the correlation is calculated: we use Spearman's rank correlation to compare usage, consisting values of \{\textit{1-At least daily}, \textit{2-At least weekly}, \textit{3-At least monthly}, \textit{4-Less than monthly}, \textit{5-Never}\}, with the average frequency of dysfluency events per utterance.}

% Intuitively, these correlations are expected, given the often inaudible gasp during blocks, and sometimes unintelligible vocalizations during part-word repetitions or interjections. 


%\note{Probably also a sentence or two explaining why certain types are more related: i.e., when there's an absence of (speech-like) sound, which happens when a PWS block, have a bad part-word repetition, or interject with less non-word sounds (mm, um..), then the endpointer tends to believe the speech is over.} 
%\note{Maybe to mention VA usage here -- in the current section 4.2.5, usage correlates highly with blocks likely due to PWS get cutoff when they block. Similarly, with baseline ASR performance, we can also describe the correlation with usage, though I find it hard to make any meaningful remarks}. 


% Ideally, this model would also be trained from scratch on large amounts of data including people with different speech characteristics, but getting sufficient amounts of data may not be feasible. 
% In the absence of such large-scale data, 


\paragraph{Tuned endpointer threshold (Intervention \#1)}
To improve the VA experience for PWS, we investigate performance of three new thresholds that could reduce truncations for people with different rates of dysfluent speech. 
% to achieve lower truncation rates
% \todo{Colin, pls confirm correctness of this para}
Specifically, using the Phase 1 data, we compute three new, higher threshold values that target an average 3\% truncation rate for participants with different levels of A\&H severities: a \textit{mild} threshold based on the 25 Phase 1 participants with mild ratings, a \textit{moderate} threshold based on the 18 moderate participants, and a \textit{severe} threshold based on the 7 severe participants. By definition, increasing the threshold will always reduce or at worst maintain the same truncation rate as a lower threshold, at the cost of incurring a longer delay before the system responds. We evaluate these thresholds on the Phase 2 participant data.

As shown in Figure~\ref{fig:boxplots_endpointer_and_wer}(a), the new thresholds substantially reduce the truncation rate for PWS compared to the baseline. Even the smallest threshold increase, ``mild'', reduces the truncation rate to a per-participant average of 4.8\% ($SD$=6.4, $Median$=1.5, $IQR$=6.5), while the moderate threshold achieves our goal of under 3\% on average ($M$=2.5\%, $SD$=3.6, $Median$=0.8, $IQR$=3.1). 
Table~\ref{tab:endpointer} shows these results averaged across all Phase 2 utterances 
% in the dataset rather than per participant---as is standard in the speech literature---
and includes metrics to capture how much delay occurs after the user finishes speaking. 
Here, $P50$ and $P95$ refer to 
%the median amount of time passed after someone in 
the $\mathrm{50^{th}}$ (median) and $\mathrm{95^{th}}$ percentile delay between when a speech utterance ends and when the system stops listening. 
% (Note: due to minor differences in the amount of data from each participant, the average truncation rates in this table are not exactly the same as those already reported across participants).
% \todo{CL: can we replace numbers in the table so they're per-participant? I checked the raw files and don't think it's trivial to get per-participant delays. -- LF: Certainly would be cleaner for the writeup, but depends on the effort required.} 
This analysis shows that the improvements in truncation rate come with a modest median delay of an additional 1.2 seconds over the baseline in the mild case and a 1.7 second increase in the moderate case. While the severe threshold is successful for 99.2\% of utterances, it causes a median delay of over 3 seconds. We return to these tradeoffs in the Discussion.

\begin{table*}[t!]
% \begin{tabular}{|l|c|ccc|}
\begin{tabular}{|l|c|cc|}
\hline
\textbf{Endpointer Tuning} & \textbf{Truncation Rate} (\%) & \textbf{P50 Delay (ms)} & \textbf{P95 Delay (ms)} \\
\hline
General Population &  23.8                 & 450          & 1,270         \\
Stutter (mild) & 4.9                  & 1,670         & 2,750         \\
Stutter (moderate)  &2.5                  & 2,190         & 3,170         \\
% Stutter 3 & 0.9998    & 1.8                  & 2,430         & 3,330         \\
Stutter (severe) &  0.8                  & 3,100         & 3,840        \\
\hline
\end{tabular}
\caption{Endpointer truncation rates and delays in milliseconds on all utterances in the Phase 2 dataset (n=5370 utterances) with threshold values tuned for different stuttering severities. There is a substantial decrease in truncations when moving from the endpointer tuned on the general population to one tuned on PWS who have mild stutter, then further reductions with tuning on moderate and severe; these reductions are consistent for every participant. P50 refers to the
$\mathrm{50^{th}}$ percentile (i.e., median) delay and P95 is the
$\mathrm{95^{th}}$ percentile delay. 
% \note{table and figure results are a little different. e.g., 23.5 vs 23.8}
}
\label{tab:endpointer}
\end{table*}


%These results are consistent with the data and anecdotes in the speech survey, in which people frequently complained about being cut off.
% As expected, the highest correlation between truncation errors and dysfluenc

% Spearman  
        % * Part Word Repetition (rho=0.44 p= 0.004)
        % * Whole Word Repetition (rho=0.18 p= 0.271)
        % * Prolongation (rho=0.17 p= 0.301)
        % * Stop (rho=0.64 p<.001)
        % * Interjection (rho=0.48 p= 0.002)

% Part Word Repetition 0.4290950739740652 0.005119332663315101
% Whole Word Repetition 0.0037841328507166247 0.9812665935144183
% Prolongation 0.1356299018836538 0.3978234652840198
% Stop 0.6215918035209798 1.441150074941624e-05




% In the survey, people noted that they are typically cut off when they block. 
% These baseline results are consistent with the data and anecdotes in the speech survey, in which people frequently complained about being cut off, and it is promising that increasing the endpointer threshold can significantly reduce these errors.




% The default value using a production speech system has a 23.5\% truncation rate on Phase 2 data with an average delay of 0.45 seconds. 
% Truncation rates for people who do not stutter are around 3\%. By increasing this threshold to the ``long'' setting there is a 79.1\% reduction in truncation with 1.22 second additional delay. ``Longer 1'' has a truncation rate that is the same as for people who do not stutter with a 89.3\% reduction in truncation rate and 1.74 second increase in delay. 
% Note that the truncation rates vary substantially per-person as shown in Figure~\ref{fig:WER} where for users with the longest blocks over 50\% of utterances are truncated early with the default setting. 







%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.7 \paperwidth]{figures/TruncationRates}
%    \includegraphics[width=0.7 \paperwidth]{figures/WER_IER_per_pid}
%    \includegraphics[width=0.7 \paperwidth]{figures/WER_per_pid_improvement_all.png}
%    \caption{Speech recognition results per Phase 2 participant for baseline and improved models. (top) Endpointer truncation rates with various tuned values, (middle) Word and Intent Error Rates for our baseline VA model, (bottom) Word Error Rates for VAs tuned on data from the general population and data from PWS. 
    % \todo{what to do about the last two entries which are >100\%}
%}
%    \label{fig:WER}
%    \Description{
%    Figure (all): This is a set of 3 bar charts as described in the caption with per-participant results. All bars are displayed in ascending order based on the baseline results.
%    Figure: (Top) Truncation rates using the baseline system gradually increase from near 0% to around 68%. There is a significant drop that is consistent across uses in the model tuned for ‘mild’, where rates drop to around 25% in the most severe cases. For the moderate model, truncation rates are near zero for most individuals but go up to about 11% for the most severe cases. 
%   Figure: (Middle) This bar chart shows WER and Intent Error Rate per participant. WER gradually increases from less than 5% to around 10% for over half of individuals, and then increases more quickly for around 15 users to a maximum of about 110% WER. The trend for Intent Error Rates is similar, with some exceptions where WER and Intent Error are not correlated, with maximum Intent Error of about 40%.
%    }    
%\end{figure}

% ----------------------------------------------------------------------------------------------------

\subsubsection{Baseline \& Improved ASR Model Performance} \label{sec:asr_baselines}
Next, we evaluated baseline ASR performance and compared the results to an approach that tunes the ASR decoder using dysfluent speech. For this analysis, we use the Apple Speech framework~\cite{SpeechFramework} and report on results from an ASR model trained on voice assistant tasks and speech from the general population. For completeness, we also examined baseline performance with a model trained on dictation tasks; the pattern of results was similar and thus results are omitted for clarity.
%, which likely does not include a substantial amount of speech from PWS. 
% This model
% consists of a hybrid deep neural network architecture with a self-normalizing acoustic model~\cite{huang2020sndcnn}, error-driven n-gram language model~\cite{gondala2021error}, and Beam Search decoder. The ASR model is comparable to that in the Apple Speech framework~\cite{SpeechFramework}.
% We use a baseline ASR models comparable to those in

%For voice assistants, we generally care if the correct action is carried out and for Dictation we want to know that they transcribed the intended speech. 
Our primary evaluation metric is Word Error Rate (WER), as widely used within the speech recognition community. 
%  to evaluate the speech recognition system used by both VA and DS
% which is an approximy metrix to evaluate VAs performance. 
% \todo{confirm if we want to use all three}. 
\textit{Word Error Rate} is computed by counting the number of substitutions, insertions, and deletions in the transcribed text, and dividing by the total number of intended words.
For example, the intended phrase ``Add apples to my grocery list'' may be spoken ``A-(dd) a-(dd) add apples to my grocery list'' and be recognized as ``had had balls to my grocery list''. With two insertions and one misrecognized words, the WER is 50.0\%.\footnote{We report WER by first calculating each participant's individual WER, then computing averages across participants. This approach is common in the HCI community because it provides an understanding of the distribution of how individual users may experience the system. In contrast, the speech community often reports WER across an entire dataset without grouping by participant. Thus, for completeness and in line with the speech community's reporting, the baseline WER for all 91 participants' data combined is 19.9\%; for only Phase 2, all data combined yields baseline WER of 25.4\%. These numbers end up being close to the averaged WERs presumably due to similar number of phrases that each participant recorded.}
%\note{CL:this sounds wonky using both averaging methods. I vote we stick with one or the other. \note{LF: I removed the reference to using both. I left the footnote since it seemed like it might be useful for a speech person reading the paper. What do you think?}}\note{CL: yeah, sounds good} 
% For overall WER and results per-participant, we calculate per-clip and then averaged across 131 clips per person.
For some experiments, we also look at Thresholded WER, as used in work by Project Euphonia~\cite{green2021automatic,tobin2022personalized}, to assess VA performance for people with speech disabilities. This is computed as the percentage of utterances, per person, with WER below 10\% or 15\% (as specified). These values have been suggested as potential minimums for VAs to be useful depending on domain.
Lastly, we look at
%  as suggested by Green \etal \cite{green2021automatic} and as Tobin and Tomanek\cite{tobin2022personalized}
% \todo{change this to 15\% .
% per \url{https://arxiv.org/pdf/2110.04612.pdf}} 
\textit{Intent Error Rate} (IER), which captures whether the VA carries out the correct action in response to an utterance. To compute Intent Error Rate, we run the ASR output on the NLU model from Chen \etal~ \cite{chen2019active} which also relied on models used by the Apple Speech Framework.
%\todo{A few extra words to describe and/or justify Chen et al's model would be good}\note{re: An NLU component needs to be run to compute Intent Error Rate. In the VA system, NLU takes the transcribed string (and other information such as the user's on device information) as input to formulate the user's intent. In our work, we run the NLU model from Chen \etal~ \cite{chen2019active} which also relied on models use by the Apple Speech Framework\note{LF: I think it's good now. Someone made a small but effective edit}}.
\footnote{
While intent recognition is not the final response of the VA, it approximates what action would be performed and can be treated as an upper bound on command accuracy.
Recall that intents are used by VAs and encode the grammar of the VA command.
For example, the query ``What day is Christmas?'' may have the intent structure \lstinline{clock[clockDate + clockNoun(date) + clockVerb(finddate)]} where \textit{date} is Christmas and \textit{finddate} is an action. 
The VA would then execute and return the date: December $\mathrm{25^{th}}$. 
}

% For the NLU model we evaluate using Intent Errors Rate (IER). 
% For example, the query ``What day is Christmas?'' is part of the \textit{clock} domain and has the intent structure \lstinline{clock[clockDate + clockNoun(date) + clockVerb(finddate)]}.

\paragraph{Baseline ASR}
% # Baseline
% # P1 WER < 10: (35/50 = 70.0)
% # P1 WER < 15: (37/50 = 74.0)
% # P2 WER < 10: (20/41 = 48.8)
% # P2 WER < 15: (25/41 = 61.0)
% # P1+P2 < 10:  (55/91 = 60.4)
% # P1+P2 < 15:  (62/91 = 68.1)
% # Both
% # P1 WER < 10: (42/50 = 84.0)
% # P1 WER < 15: (46/50 = 92.0)
% # P2 WER < 10: (27/41 = 65.8)
% # P2 WER < 15: (33/41 = 80.5)
% # P1+P2 < 10:  (69/91 = 75.8)
% # P1+P2 < 15:  (79/91 = 86.8)
% We also evaluate intent recognition performance using an NLU system comparable to that described by Chen \etal~\cite{chen2019active}. 
Table~\ref{tab:baselineWERbySeverity} shows baseline ASR performance. Across participants in both phases, the average baseline WER is 19.8\%, %($SD$=31.7, $median$=7.1, $IQR$=20.2)
which is much higher than the $\sim$5\% reported for consumer VA systems \cite{Xiong2016HumanParityASR, Stolcke2017HumanMachineComparison, Xiong2018MicrosoftASR}.   
% with more recent models claiming lower WER~\cite{Baevski2020wav2vec2}. 
The WER distribution is also highly skewed, with many participants having low WERs but also a long tail of participants with much higher WERs.
For people with mild A\&H severity, the average WER was 4.8\%, which is similar to what is expected for people who do not stutter, whereas moderate and severe had average WERs of 13.6\% and 49.2\%, respectively. Moreover, 84.0\% of participants with mild severity had a WER of less than 10\% (i.e., Thresholded WER) and the average Intent Error Rate for this group was 4.9\%, suggesting that many people with mild A\&H severity ratings would likely be able to use off-the-shelf VA systems, which echos the VA usage reported in survey presented in Figure ~\ref{fig:usage_frequency_by_severity_future_tech}(left).For moderate and severity grades, Intent Error Rates are 7.3\% and 18.4\% respectively. 
Overall, this analysis both confirms the ASR accuracy difficulties described in the survey, as well as reflects the varied experiences that survey participants reported in how well VAs understood them (Figure~\ref{fig:freqUseAndPerceivedAccuracyVAandDictation}). 
 
% \todo{need to add a citation to support claim that mild rate is similar to non-PWS.}
%mild is 5.0\%, moderate is 13.6\% and severe is 49.0\%. 
%  (SD=6.6),  (SD=16.5),  (SD=48.0)
%\todo{CL:move IER here?} Finally, Intent Error Rate is 7.4\% \todo{Check this number, found unexpected large variance between weighted avg and avg}.

\begin{table*}[t!]
\begin{tabular}{|l|cccc|cc|cccc|}
\hline
& \multicolumn{4}{c}{\textbf{Word Error Rate (WER) (\%) }} & \multicolumn{2}{|c|}{\textbf{Thresholded WER (\%) }} & \multicolumn{4}{|c|}{\textbf{Intent Error Rate (IER) (\%) }} \\
\textbf{Participant Subset} & \textit{Mean} & \textit{SD} & \textit{Median} & \textit{IQR}  & \textit{WER<10} & \textit{WER<15} & \textit{Mean} & \textit{SD} & \textit{Median} & \textit{IQR} \\
\hline
Mild (n=25) & 4.8 & 6.7 & 2.4 & 1.8 & 84.0 & 88.0 & 4.9 & 4.2 & 6.1 & 6.9 \\
Moderate (n=44) & 13.6 & 16.7 & 8.5 & 12.2 & 63.6 & 75.0 & 7.3 & 6.8 & 5.0 & 9.0 \\
Severe (n=22) & 49.2 & 49.2 & 47.0 & 61.1 & 27.3 & 31.8 & 18.4 & 15.6 & 19.8 & 28.4 \\
\hline
All (n=91) & 19.8 & 31.7 & 7.1 & 20.2 & 60.4 & 69.2 & 9.3 & 10.5 & 6.1 & 9.9 \\
Phase 2 (eval set; n=41) & 25.4 & 28.7 & 10.8 & 33.8 & 48.8 & 61.0 & 10.4 & 10.8 & 5.3 & 13.4 \\
\hline
\end{tabular}
\caption{Baseline ASR model performance, broken down by severity level for all 91 participants, and overall for all 91 and for only Phase 2 participants. Participants with a mild A\&H rating had WERs on par with the general population, whereas more moderate and severe dysfluency speech greatly affects WER. Because we used Phase 1 for tuning our models, much of the analysis focuses on performance for the Phase 2 participants, who all had moderate or severe A\&H severity ratings.
}
\label{tab:baselineWERbySeverity}
\end{table*}


%For Phase 2 data, which we focus on later, WER is 25.4\%. 
%For Phase 2 data only, which has a higher portion of participants with moderate or severe A\&H grades, the average per-participant WER is 25.4\%. 
%($SD$=28.7) and median is 10.8 ($IQR$=33.8).

%\todo{are we removing figure this refers to?} See Figure~\ref{fig:WER} (bottom) for WERs per-participant.
%As expected, these numbers are higher than for the whole dataset because Phase 2 focused on participants with moderate or severe stuttering severity.
% (SD= 28.4)
% (median of 10.8\% and interquartile range of 33.8\%). 
% Baseline: Phase 2
% STD: 28.38052664981537 VAR: 805.4542929208803
%Many people had very low WER, as emphasized by Thresholded WER: 48.7\% (N=20 participants) had WER$<$10\% and 60.9\% (N=25) had WER$<$15\%, suggesting that VAs may be accurate enough to be useful for about half the participants in Phase 2. 
% While many participants had WER less than 10\%, many also had very high WER, including one with a WER of 110.8\%.
%Intent Error Rate is 10.4\% 

%\note{CL: maybe remove IER from each paragraph and add one paragraphs discussing the results?}\todo{needs to be split as average across participants, if we include it. In general, I wonder if we even want to report it}. 

% Baseline: Phase 2
% Mean:25.44 median:10.84 Q1:6.52 Q3:40.35 Q3-Q1:33.83

To understand how different types of dysfluencies affect WER, we examined the Phase 2 data, which includes detailed dysfluency annotations (see Section~\ref{sec:speech_data} for rates of each dysfluency type). Note that Phase 2 only included participants with moderate and severe A\&H ratings, so on average has somewhat higher WER (25.4\%) than the full set of participants (bottom row of Table~\ref{tab:baselineWERbySeverity}). 
For these Phase 2 participants, we found high Spearman's rank correlations\textsuperscript{\ref{spearman_footnote}} between WER and part-word repetitions ($r(39)=.85$, $p<.001$) and between WER and whole word repetitions ($r(39)=.60$, $p<.001$). The correlations were not significant for prolongations ($r(39)=.3$, $p=.056$), blocks ($r(39)=.21$, $p=.181$) or interjections ($r(39)=.15$, $p=.347$). 
This indicates that part-word and whole word repetitions tend to increase word error rates, and that blocks, prolongations and interjections
% ~\note{remove interjections from this sentence, but maybe good to still mention it here to cover all types as it's the first time such analysis results are listed} 
have less of an impact even if they are frequent. 
% \note{No meaningful correlations  between self-reported VA usage and the types of dysfluency rates, }
%We see a higher correlation between Part Word Repetition Rate and WER; implying that a higher frequency results in worse ASR performance.
%Interestingly, blocks don't necessarily impact WER, even if they are frequent or long in duration.

%     * Spearman:
        % * Part Word Repetition: r: 0.85 p: 0.0
        % * Whole Word Repetition: r: 0.6 p: 0.0
        % * *Prolongation: r: 0.3 p: 0.056*
        % * Blocks: r: 0.21 p: 0.181
        % * *Interjection: r: 0.15 p: 0.347*


Among all errors the ASR system made in Phase 2, 80.9\% were word insertions, 17.5\% substitutions, and only 1.6\% deletions. The high rate of word insertions has a strong correlation with part-word repetitions ($r(39)=.73$, $p<.001$) followed by whole word repetitions ($r(39)=.60$, $p<.001$).
This echoes survey reports that part-word or whole word repetition can lead to misrecognized words being inserted in their transcription. 
A trained speech-language pathologist characterized insertion errors from part-word repetitions and found that in many cases insertions come from individual syllables being recognized as whole words (e.g., the first syllable in ``become'', vocalized as ``be-(come) be-(come) become''). 
% may be recognized as multiple words. 
In contrast, a sound repetition on /b/ in ``become'' is less likely to lead to word insertions. 
% Furthermore, part-word repetitions tend to occur on initial sounds~\cite{hubbard1998stuttering}, however, 
Furthermore, some people demonstrated part-word repetitions between syllables in multi-syllabic words, such as the word ``vocabulary'' may result in spurious insertions, such as ``vocab cab Cavaleri.''

% Lastly, a trained speech language pathologist performed detailed analysis of part-word repetitions. Syllable repetitions were parsed out from sound repetitions and noted to lead to increased word insertions as compared to single sound repetitions.  
% In many cases, this was due to individual syllables being recognized as whole words.  
% For example, if someone produces a syllable repetition on the first syllable in ``become'' (e.g., ``be... be... be...come''), it may be recognized as multiple words. Whereas, if someone produces a sound repetition on /b/ in "become" (e.g., ``b... b... become''') word insertion errors are less likely.  
% People who produce part-word repetitions tend to do so more frequently on initial sounds, which was also reflected in this data~\cite{hubbard1998stuttering}. However, some people also demonstrated part-word repetitions or blocks between syllables in multi-syllabic words.  For example if someone produced a block mid-word in the word “dis...able,” it could be recognized as two words “this” and “able.” If someone produced a repetition mid-word in the word “vocabulary" (vocab..cab.. cabulary) it may break the word down into "vocab cab Cavaleri." These relatively rare occurrences appeared to produce more word insertions. 
% Similarly, audio from participants who interjected ``uh'' between words or those that produced an audible block with vowel like sounds resulted in higher WER. These vowel sounds resulted in word insertion errors. 
% Interjections show a moderate low correlation ($r=0.27$, $p=0.089$) with WER, by examing ASR transcriptions we notice ASR does not transcribe filler words such as  “um”, “eh”, “hmm”, “uh”, and other minor variations. 

%     * Spearman
        % * Part Word Repetition r: 0.73 p: 0.0
        % * Whole Word Repetition r: 0.6 p: 0.0
        % * Prolongation r: 0.13 p: 0.428
        % * Blocks r: 0.07 p: 0.679
        % * Interjection r: 0.18 p: 0.256



%\note{bring back survey thoughts}
% Correlation between Insertion Error Rate and Dysfluency Types
% Part Word Repetition 
%   r: 0.75   p: 1.7776342158497337e-08
% Whole Word Repetition 
%   r: 0.48   p: 0.0013586859494377351
% Prolongation 
%   r: 0.04   p: 0.7832423659946212
% Stop 
%   r: 0.1   p: 0.5141140383708009
% Interjection 
%   r: 0.27   p: 0.08887331303380591

% -- ZFH: removed DS-tuned result and commented out below  -- 
% Recall that the DS and VA share the same underlying ASR models, but the DS is biased towards open-ended language and the VA is biased towards common VA queries. 
% Most of our phrases are VA-related, which likely explains why the VA-tuned model performs better. 
% -- commented out by ZFH -- 

% Voice Assistants may bias towards common VA queries whereas Dictation may bias towards open-ended language. 

% Dictation Systems frequently use the same ASR model as VAs, however there may be variation in the underlying language model. 

% This is not unexpected, given that The improvement in the VA model is likely due to bias in the language model to prefer VA-like queries. 
% Error characteristics tended to be the same between systems, so we omit more detailed analysis.
% \note{The average WER for people with a mild stuttering severity is [X], moderate is [Y], and severe is [Z]. }

% With Phase 2, we notice that there is a gradual increase in WER for individuals up to $P50$ and then a steep increase after that. \todo{why?}
% \todo{any other interesting observations?}
% \todo{Maybe: proper noun analysis}

% \note{Moved this to correlations with disfluency (\sec:dysRates-correlation ):
% The Pearson correlation between WER and dysfluency types is: part word repetitions ($r=0.80$), whole word repetitions ($r=0.55$), prolongations ($r=0.29$), and blocks ($r=0.10$). 
% This implies that the largest room for ASR improvement could come from improving detection or mitigation of part-word or whole word repetition errors. 
% There is a moderate correlation between the average duration of dysfluencies within an utterance and WER ($r=0.39$).


% All WER/Intent results unless otherwise specified were done without an endpointer, which is equivalent to using ``Hold to Talk'' on an iOS device. 
% Predictions from the ASR model are inserted into the NLU model of Chen \etal \cite{chen2019active} to get intent error rates, with results shown in Figure~\ref{fig:WER}.



\paragraph{ASR Decoder Tuning (Intervention \#2)}
% \underline{Intervention \# 2 (ASR Decoder Tuning)}:
Consumer ASR systems are commonly trained on thousands of hours of speech from the general public; an amount far larger than can likely be obtained from PWS.
% The baseline ASR and NLU models were trained on data from people in the general population, not centered on PWS. 
% Again, given the relatively small amount of stuttering data available, it is unrealistic to train ASR models from scratch with speech from PWS. 
% , it is challenging to train end-to-end ASR models for PWS.
However, an initial investigation by Mitra \etal~\cite{mitra2021} on 18 PWS has shown it may be possible to tune a small number of ASR decoder parameters to improve performance for PWS. 
% , so similar to the endpointing experiments we tuned the ASR decoder model on Phase 1 data of PWS. Specifically, 
Here, we validate this approach on our larger dataset and find even greater gains when tuning on our 50 participant Phase 1 subset.
% We use Mitra \etal's~\cite{mitra2021} tuning approach, which was only validated on speech from 18 PWS. 
While we defer to that paper for details,  
% which was also for stuttered speech and used their recommended
in brief the approach increases the importance of the language model relative to the acoustic component in the decoder and increases the penalty for word insertions.
% which biases the model to have shorter transcriptions. 
These changes reduce the likelihood of predicting extraneous low-confidence words often caused by part-word repetitions and bias the model towards more likely voice assistant queries. 
% For Phase 1 of the Stuttering EDC, we created separate ASR Tuning Profiles per severity. Results below show performance using the Severe profile from Phase 1 as applied to the Phase 2 data. 
We used Phase 1 data to tune these parameters and report results on Phase 2. 

The average WER for Phase 2 participants jumps from the baseline of 25.4\% to 12.4\% ($SD$=12.3, $median$=6.1, $IQR$=13.1) with the tuned decoder, which is a relative improvement of 51.2\%. A Wilcoxon signed rank test shows that this improvement is statistically significant. 
See Table~\ref{tab:WERbyExperimentAndbyDysfluencyType} for more metrics and to understand how WER improves as a function of dysfluency types. For example, the WER lowers (improves) in 43.2\% of utterances with part-word repetitions and increases (worsens) 3.9\% of the time. For ASR tuning, WER improves the most in utterances that have whole word repetitions, part-word repetitions, and interjections and least for those with prolongations or blocks.
% For 12 of 27 PWS the Intent Accuracy improved by over 10\% absolute.
% and for 5 of 27 severe stutters it improved by over 20\%. 
%After tuning, Spearman's rank correlation between WER and part-word repetitions reduced from $r(39)=.85$ to $r(39)=.78$ ($p<.001$), 
% interjections reduced from $r=.53$ to $r=.37$ ($p=.019$), 
%and the other correlations were either similar as before or not significant.
%ASR tuning is more effective in mitigating part-word repetition errors relative to Dysfluency Refinement, however, overall recognition of phrases with part-word repetitions remains to be a challenge.
%\note{This sentence needs revise as we moved Dysfluency Refinement to a later paragraph. More importantly, I wonder do we still report spearman corr to argue the ASR tuning is more effective in mitigating part-word repetition errors or point readers to the above table to read that the percentage of utterances that see improvement or deterioration}. 
% ~\note{add a sentence for conclusion}
% However, the fact that this correlation is high indicates a need for more effective approaches, which is discussed in Section~\ref{sec:discussion}.
% \note{I'm not sure 'does not have filler words' is correct; the vocabulary for both models is the same, we're just changing the bias. Zifang: Will said Siri ASR does not transcribe such fillers.} 
% Interestingly, we also find that tuning also removes many interjections, largely because ASR's vocabulary do not have filler words such as ``um'' and ``eh,'' when a PWS use such fillers, ASR often misrecognizes them as something else, for example, ``uh'' as ``a''. And ASR tuning can effectively remove such low confidence words.
% We find that the types of errors that ASR tuning fixes (i.e., part-word repetitions) are largely different from the types of errors that the Dysfluency Refinement fixes (i.e., whole words and interjections).

%     * Spearman
        % * Part Word Repetition r: 0.78 p: 0.0 (0.85)
        % * Whole Word Repetition r: 0.62 p: 0.0  (0.6)
        % * Prolongation r: 0.28 p: 0.075* (0.3)
        % * Blocks r: 0.23 p: 0.145 (0.21)
        % * Interjection r: 0.13 p: 0.408* (0.15)


% Tuned
% Part Word Repetition 
%   r: 0.73   p: <0.001
% Whole Word Repetition 
%   r: 0.72   p: <0.001
% Prolongation 
%   r: 0.17   p: 0.27615051653593675
% Stop 
%   r: 0.16   p: 0.3246814300029299
% Interjection 
%   r: 0.37   p: 0.018776720925452774

% Tuned+Refined
% Part Word Repetition 
%   r: 0.74   p: <0.001
% Whole Word Repetition 
%   r: 0.47   p: 0.0018827021692546058
% Prolongation 
%   r: 0.33   p: 0.03349110215263842
% Stop 
%   r: 0.19   p: 0.2383781338970239
% Interjection 
%   r: 0.34   p: 0.030177897467017177
  
% We find that the types of errors that this repetition removal fixes (i.e., whole words and interjections are largely different than the types of errors that ASR Tuning fixes (i.e., partial word repetitions). 



% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.6 \paperwidth]{figures/WER_per_pid_overTime}
%     \caption{ASR WER breakdown by participant over time}
%     \label{fig:ASROverTime}
% \end{figure}

% Similar heuristics are applied to the actual articulated speech and that gives WER of 3.89\%. This means if filler words and repeated words/phrases removed, for an average human ear, for this dataset, if ignoring annotation error, what the best possible WER could be. \note{mention the articulation transcript version as upper bound? or will it be confusing? - probably confusing. If we have a comparison of the human recognition WER for general population, might be interesting to see, but I don't find such numbers.}We also experimented with a state-of-art open source masked language model to recover words where a part-word-repetition occur, and that only gave marginal gain.


% * Baseline WER (ASR WER for all data - phase1+phase2; SiriQuery+Dictation): 19.71%
% * Improved ASR WER: 13.03%  (33.89% relative improvement)
% * Improved annotation/articulated transcription WER: 3.89% (this’s close to the best WER we can get when ignoring annotation errors, and if VA reaches to human speech recognition ability)


% Figure~\ref{fig:my_label}

% \subsubsection{Understanding severity, dysfluency rate, and WER}

% \note{Move to discussion: talk about disconnect between severities and ASR results; in particular because severity is a function of all dysfluency types and ASR is more correlated with the rate of specific dysfluencies.  } 

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.6 \paperwidth]{figures/Metrics Table.png}
%     \caption{\note{To be updated with a table format. Inserted for early reference as there're many comments/TODOs now pointing to this table.}}
%     \label{fig:ASROverTime}
% \end{figure}


% \begin{table}[]
% % \resizebox{\columnwidth}{!}
% % \usepackage{array}
% % \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} |cc|cc|cc|cc|cc|}
% \begin{tabular}{|l|cc|cc|cc|cc|cc|}
% % \begin{tabular}{|m p{0.5cm}|c p{0.15cm} c p{0.15cm}|c p{0.15cm} c p{0.15cm}|c p{0.15cm} c p{0.15cm}|c p{0.15cm} c p{0.15cm}|c p{0.15cm} c p{0.15cm}|}
% \hline
% & \multicolumn{2}{c}{\textbf{Part-word Repetition}} & \multicolumn{2}{|c|}{\textbf{Whole-word Repetition}} & \multicolumn{2}{|c|}{\textbf{Prolongation}}  & \multicolumn{2}{|c|}{\textbf{Stop}} & \multicolumn{2}{|c|}{\textbf{Interjection}} \\
% \textbf{Experiment} & \textit{Improve} & \textit{Regress} & \textit{Improve} & \textit{Regress}  & \textit{Improve} & \textit{Regress} & \textit{Improve} & \textit{Regress} & \textit{Improve} & \textit{Regress} \\

% ASR Decoder Tuning & 43.2 & 3.9 & 64.0 & 3.0 & 30.9 & 5.1 & 31.4 & 5.2 & 53.3 & 5.0\\
% Dysfluency Refinement & 25.2 & 0.0 & 64.7& 0.3 & 12.9 & 5.0 & 17.7 & 0.1 & 30.9 & 0.0 \\
% Combined & 47.6 & 3.5& 81.1 & 2.0& 32.8& 0.1 & 34.6 & 5.0 &57.2 & 4.6  \\
% \hline
% \end{tabular}
% % \end{tabular*}
% \caption{Performance Improvement from Each Intervention. For data of each dysfluency type, the percentage of utterances that sees WER improvement and deterioration from each and combined experiment.}
% \label{tab:WERbyExperimentAndbyDysfluencyType}
% \end{table}


\begin{table*}[]
\begin{tabular}{|l|cc|cc|cc|}
\hline
& \multicolumn{2}{c}{\textbf{ASR Decoder Tuning}} & \multicolumn{2}{|c|}{\textbf{Dysfluency Refinement}} & \multicolumn{2}{|c|}{\textbf{Combined}}  \\
\textbf{Dyfluency Type} & \textit{Improved} & \textit{Regressed} & \textit{Improved} & \textit{Regressed}  & \textit{Improved} & \textit{Regressed} \\
\hline
Part-word Repetition & 43.2\% & 3.9\% & 25.2\% & 0.0\% & 47.6\% & 3.5\%\\
Whole Word Repetition & 64.0\% & 3.0\% & 64.7\% & 0.3\% & 81.1\% & 2.0\% \\
Prolongation  & 30.9\% & 5.1\% & 12.9\% & 5.0\% & 32.8\% & 0.1\% \\
Block & 31.4\% & 5.2\% & 17.7\% & 0.1\% & 34.6\% & 5.0\% \\
Interjection & 53.3\% & 5.0\% & 30.9\% & 0.0\% & 57.2\% & 4.6\%\\
\hline
\end{tabular}
\caption{Percentage of utterances labeled with a given dysfluency type that result in \textit{improved} WER or \textit{regressed} (worsened) WER with: ASR decoder tuning, dysfluency refinement, or the combination of the two. Generally, the improvements come with few regressions.}
\label{tab:WERbyExperimentAndbyDysfluencyType}
\end{table*}

\subsubsection{Dysfluency Refinement (Intervention \#3)}
According to our survey, PWS are often displeased when seeing repeated words, phrases and filler words in their dictated notes and texts. 
% This is shown by a moderately negative correlation between whole word repetitions ($r(20)=-.47$, $p=.013$) and self-reported dictation usage.
%Recall that WER has a moderate to high correlation with Interjection, Part Word and Whole Word repetitions, 
%Here we propose strategies for reducing WER focusing on typical errors arising from these dysfluencies.
To address this issue, we refine the transcribed text using two strategies.
% , which reduced WER for these dysfluency types.
% This was evident by looking through the ASR predictions as well. 
% We see this in the ASR predictions as well, where repeated words and fillers (e.g., ``uh'' and ``um'') are especially common. 
%We experimented with two heuristics to refine ASR transcriptions.
First, we look at filler words such as ``um,'' ``eh,'' ``ah,'' ``uh'' and minor variations.
% ``hmm,'' 
Many of these filters are not explicitly defined in the language model (i.e., by design ``eh'' is never predicted), however, in practice, short fillers are frequently transcribed as the word ``oh.'' As part of our approach, we remove ``oh'' from predictions, unless ``oh'' is used to represent the number zero.
% , except when predicted next to a number (i.e., one oh one for the number 101).
We considered others such as ``like'' and ``you know,'' which are common in conversational speech, but they did not appear as fillers in our dataset, likely because the utterances tend to be short and more defined than free-form speech. 
% instances. 
% The first is to remove fillers from the ASR transcriptions including  and minor variations. 
% Interestingly, we find that fillers such as ``uh,'' ``eh,'' ``ah'' and variants are transcribed as ``oh,''
% While participants rarely use more complex filler words such as ``you know,'' ``like'' in short utterances such as our recordings, we found utterances with interjections sometimes have extra ``oh''s inserted and we remove these while keeping the case ``oh'' as number zero untouched.
% we found utterances with interjections sometimes have extra ``oh''s inserted and we remove these while keeping the case ``oh'' as number zero untouched.
% Ultimately, we found that the ASR often ignores these, as this only improves WER from 19.9\% to 19.5\% with respect to intended speech, which does not include these interjections. 
% ["um", "uh", "uhh", "uhm", "huh", "hmm", "eh" ]
Second, we remove repeated words and phrases. This is more challenging because words may naturally be repeated (e.g., ``We had had many discussions'').
In our refinement approach, we take all adjacent repeated words or phrases in a transcript and compute the statistical likelihood that they would appear consecutively in text using an n-gram language model that is similar to~\cite{Heafield2013LM}. 
% So for all adjacent repeated words we look at the likelihood using a 
If the probability is below a threshold,\footnote{The threshold $\tau$ was chosen based on early experiments on Phase 1 and non PWS-centered datasets.} i.e., $\mathrm{P}(\textsc{substring}_1, \textsc{substring}_2) < \tau$, then we remove the duplicate.
%\todo{consider adding note on how tau was chosen}
% caused by repetitions while applying an ARPA language model to filter out the highly likely correct repetitions in an utterance. 
% Repeated words in a sentence such as "We had had many discussions" is gramatically correct and though rare in a VA query, there is a possibility that we may naively condense an intended repeated words. 
% The ARPA language model computes the sentence as well as the repeated two words (2-gram) probability, and as long as $P(sentence) > 1e-07$ or $P(2-gram)>2e-4$ we believe that repetition is acceptable. 
% This has been working well in practice for our dataset. 
Note that these two strategies---interjection removal and repetition removal---can be applied to any ASR model output, thus we evaluated our dysfluency refinement approach in combination with both ASR models from Section~\ref{sec:asr_baselines}: the baseline model and the model with the tuned decoder.

As shown in Figure ~\ref{fig:boxplots_endpointer_and_wer}(b), dysfluency refinement reduces WER for the Phase 2 data compared to both the baseline and tuned ASR models. The average WER goes from a baseline of 25.4\% to 18.1\% ($SD$=19.2, $median$=6.1, $IQR$=22.8) after dysfluency refinement---a 28.7\% relative improvement on average. This improvement is significant with a Wilcoxon signed rank test ($W$=839, $Z$=5.43, $p$<.001).
As shown in Table~\ref{tab:WERbyExperimentAndbyDysfluencyType}, across the entire Phase 2 dataset, 64.7\% of utterances that contain whole word repetitions see a WER improvement and only 0.3\% regress. For those with interjections, WER improves in 30.9\% and regresses in none of the utterances. 
% Interjections have a relative reduction of 33.7% and WWR have a relative reduction of 41.3% (Baselined -> refined)

% Remaining word repetitions, and most part-word repetitions, are likely transcribed as distinct words. (e.g., ``al-(arm) alarm'' is predicted ``all alarm'') and thus are not detected by our approach.
% Some remaining filler words may be integrated 
% Remaining repetitions, especially partial-word repetitions, are likely transcribed as distinct words. (e.g., ``al-(arm) alarm'' is predicted ``all alarm'') and thus are not detected by our approach, but could be addressed with fuzzy matching in future work.
% We again looked at the correlation between WER for the improved model and dysfluency rates. Part-word repetitions are approximately the same ($r(39)=.84$, $p<.001$). Whole word repetitions reduced slightly from $r(39)=.6$ to $r(39)=.55$ ($p<.001$). 
% [old] and interjections reduced from $r(39)=0.53$ to $r(39)=0.50$ ($p<0.001$) 
% [old]~\note{this sentence}which indicates that many of these dysfluencies are no longer appearing in the transcript. 
% [old]Prolongations ($r=0.27$, $p=0.09$) and Blocks ($r=0.18$, $p=0.27$). 
% [old]This reduction from $r=0.56$ to $r=0.44$ for whole word repetitions, which indicates that many of these dysfluencies are no longer appearing in the transcript. 
% Interjections still have no significant correlation ($r(39)=.15$, $p<.361$), partially due to its extremely low appearance in all participants speech except one.

    % * Spearman
    %     * Part Word Repetition r: 0.84 p: 0.0 (0.85)
    %     * Whole Word Repetition r: 0.55 p: 0.0 (0.6)
    %     * Prolongation r: 0.32 p: 0.041
    %     * Blocks r: 0.23 p: 0.15
    %     * Interjection r: 0.15 p: 0.361

% Refinement
% Part Word Repetition 
%   r: 0.76   p: 9.268073976402722e-09
% Whole Word Repetition 
%   r: 0.44   p: 0.004079876862273337
% Prolongation 
%   r: 0.27   p: 0.09365909914024474
% Stop 
%   r: 0.18   p: 0.2729767871737259
% Interjection 
%   r: 0.5   p: <0.001

% The only repetition that is incorrectly kept is ``Hey hey [name]'' which should have been ``Hey [name].''
% While this approach is intended for DS, we also tested this approach using the VA results on Phase 2 and found that WER improved from \note{X\%} as baseline, to \note{X\%} with ASR Tuning, and to \note{X\%} with VA Tuning and our intelligent Dysfluency Refinement. 
% (And in our dataset, the only one passed (that shouldn’t pass) this criteria is the clip "hey hey Siri". 
% Also, we don't condense any repetitions in numbers. Examples: Call three three two five eight seven seven two one, set an alarm at six six thirty. 

Applying dysfluency refinement to the output from the tuned ASR model further reduces WER, from on average 12.5\% with the tuned model alone to 9.9\% ($SD$=8.8, $median$=5.3, $IQR$=10.3) for the tuned model plus dysfluency refinement. Compared to the baseline ASR model, this tuned model plus dysfluency refinement combination is an average 61.2\% improvement across participants. 
Wilcoxon signed rank tests show that these improvements are statistically significant both when appended to the baseline ASR model output ($W$=741, $Z$=5.37, $p$<.001) or appended to the tuned ASR model output ($W$=595, $Z$=5.08, $p$<.001).
The percentage of participants with WER$<$10\% increases from 48.8\% to 65.9\%
%and for WER$<$15\% from 61.0\% to 80.5\%. 
and the average Intent Error Rate improved from 10.4\% ($SD$=10.8, $median$=5.3, $IQR$=13.4) to 5.4\% ($SD$=5.8, $median$=3.1, $IQR$=7.2). 
% \todo{either give an explanation or remove IER from the ASR tuning experiment}
% Old: WER is 25.4\%, Thresholded WER is 48.7\% (WER$<$10\%) and 60.9\% (WER$<$15\%)
% Both: WER is 9.9\%, Thresholded WER is 65.8\% (WER$<$10\%) and 80.4\% (WER$<$15\%)
% , and Intent Error Rate is 10.4\%.
% \todo{remove this sentence about the figure} Figure~\ref{fig:WER} (bottom) highlights WER changes for participants with WER$\geq$10\% using the baseline model.
% Out of these 29 participants, 17 of them now see WER below 15\%. \todo{change the following example to phase 2}
Such improvements may enable a VA to be usable for many of our participants when the baseline is not; for example, P2-21's WER improves from 40.4\% (baseline) to 13.0\% (tuned ASR + dysfluency refinements) and IER improves from 19.1\% (baseline) to 4.6\%.
%,  go from not being understood by the system to being able to use a VA with reasonable success rate. 
% For subjects such as P1-29 whose WER was 62.8\% before the experiments, and now 11.0\%, meaning from not understood by the system to be able to use a VA with decent success rate. 
% of them see WER reduction of more than 80\%. 
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.6 \paperwidth]{figures/Tuning_WER_per_pid}
%     \caption{Relabel. Tuned for general public vs Tuned for PWS. !!! Remove "production" and relabel non-PWS Tuned and PWS Tuned !!!}
%     \label{fig:TuningASR}
% \end{figure}

% ----------------------------------------------------------------------------------------------------
% \subsubsection{Dictation System} 

\subsubsection{ASR Results Over Time}\label{sec:asr_over_time}
The above analyses assess the effectiveness of three changes to an existing speech recognition system that require little data from PWS to implement. 
At the same time, there has been substantial progress in general speech recognition models in recent years, with some accounts claiming WERs of 5\% or less using consumer voice assistants~\cite{Xiong2018MicrosoftASR}. Theoretically, these general improvements could also result in improvements for PWS. 

To understand how these changes over time impact performance on dysfluent speech,
% There is a common perception within the ASR community that innovations in speech architectures and general WER improvements will effect everyone, and as such it is not necessary to target specific populations e.g., for people who stutter or have other speech disabilities. 
% We evaluated ASR results with the same speech recognition system trained at different points between Fall 2017 and Spring 2022 on our data. 
we use the Apple Speech framework to run all Phase 1 and 2 data through archived ASR models that had been publicly available between Fall 2017 and Spring 2022; these experiments were conducted in Summer 2022.
Figure~\ref{fig:ASROverTime} shows WER across all utterances in the dataset every 6 months across the five years. The utterance-weighted WER was 29.5\% for the Fall 2017 model, fell consistently for the following eight time periods, and ended at 19.9\%. This is a 32.5\% relative reduction in WER from the start to the end of the 5-year time span. 
Differences at each time point may be attributed to what data was used in training, the convolutional architecture, and/or the language model. 

% For mild severities WER reduced 53.3\% (4.3 to 2.0\%), for moderate it reduced by 31.1\% (10.9 to 7.5\%) and for severe by 23.0\% (28.2 to 21.7\%).
% Moderate: 10.909 → 7.52 (31.06% WER reduction)
% Severe: 28.26 → 21.75 (23.03% WER reduction)
% [Intent Accuracy (2017 vs 2022)]
% Mild: 94.65 → 97.32 (49.90% error reduction)
% Moderate: 84.79 → 89.69 (32.21% error reduction)
% Severe: 61.64 → 71.40 (25.44% error reduction)
For Phase 2 utterances, we further examined changes in how specific types of dysfluencies manifest in WER performance between the Fall 2017 to Spring 2022 models. For part-word repetitions, the WER improved 43.5\% of utterances (worse 12.2\%), those with whole word repetitions 46.8\% (worse 14.5\%), prolongations 36.9\% (worse 10.3\%), blocks 36.0\% (worse 9.4\%), and interjections 65.8\% (worse 10.4\%).
The improvements with part-word repetitions are especially interesting, because these errors are more challenging to correct using our strategies. 
% While the overall WER results even in Spring 2022 are still far from the $\sim$5\% claims on general population data,
%---and may not be representative of performance on other subpopulations in the general public---
% the absolute numbers are in line with results on atypical speech efforts like Project Euphonia~\cite{projecteuphonia} and show a notable improvement over the years. 
See the Discussion (Section~\ref{sec:discussion}) for further implications of these findings. 
% These are substantive improvements, but indicate that \todo{how to write this?? }
% Part Word Repetition
% better 43.53, worse 12.15, same 44.32
% Whole Word Repetition
% better 46.8, worse 14.48, same 38.72
% Prolongation
% better 36.95, worse 10.29, same 52.76
% Stop
% better 36.01, worse 9.38, same 54.62

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4 \paperwidth]{figures/ASR_Perf_Over_5yrs.png}
    \caption{
    Performance of the speech recognition system as trained at different points between 2017 and 2022. There is a significant improvement in part- and whole word repetitions. Note that absolute WERs and their improvements may not be representative of performance on other sub-populations in the general public, which has been documented to be as low as 5\% WER (e.g., \cite{Xiong2018MicrosoftASR}). 
    }
    \label{fig:ASROverTime}
    \Description{This bar chart shows ASR performance over 10 points in time, from Fall 2017 to Spring 2022. Results gradually decrease from 29.5\% to 19.9\%, with a low of 19.6\% in the second most recent time point.
    }
\end{figure}
% ----------------------------------------------------------------------------------------------------

% \subsubsection{Speech Recognition Analyses} 

% ------ CL - I commented out the net few paragraphs for R&R ----------
% \subsubsection{Speech Data and User Perceptions} 
% \todo{Need to decide what analyses to include here. The dysfluency types vs. usage is very specific, whereas overall WER isn't included. And the severity breakdown is similar to an analysis reported in 4.2.2. One possibility is to pepper in a few small analyses earlier in 4.2. Like in 4.2.1 put the correlation between truncation and reported usage or something. Or relationship between truncation rates and whether someone said early cutoff was a barrier to use}
% \note{CL: agreed. probably best to merge the first part of this section with earlier content and remove the latter paragraph (as LF suggested)} \note{zfh: Yeah! (agreed with both decisions)}
% In this section we analyze correlations between the survey data and audio recordings. \todo{need to clarify what participants this is on. N=53?
% }
% % speech recognition results, dysfluency rates, and survey results.
% % Specifically, we look at correlations between (1) usage and dysfluency rates, (3) perceptions and ASR performance and (3) severity and ASR performance
% % (2) usage and ASR performance, 
% % , survey findings, and clinical severity. 
% These are performed with acknowledgement that stuttering is situational and varies based on the environment, stress levels, and other conditions~\cite{tichenor2021variability}.
% We explored other correlations, such as between WER and self-reported perceptions on VA understanding and did not find strong correlations. 

% \paragraph{Dysfluency Rates vs Usage}
% As shown in Figure~\ref{fig:dysfluency_rates}, the distribution of dysfluency types varies greatly across participants.
% % We found correlations between the dysfluency rate distribution and self-reported VA and Dictation usage. 
% % and found low-to-moderate association between frequency of speech recognition use with blocks and interjections\note{we don't use interjections elsewhere}.
% We extend this analysis to investigate how rates of different dysfluency types are correlated with self-reported VA and dictation usage. Again, we use Spearman's rank correlation to compare usage, consisting values of \{\textit{1-At least daily}, \textit{2-At least weekly}, \textit{3-At least monthly}, \textit{4-Less than monthly}, \textit{5-Never}\}, with the average frequency of dysfluency events per utterance. Note that only the \todo{X} Phase 2 participants who filled out the survey and recorded audio data are included in this analysis due to the need for fine-grained dysfluency annotations. 
% For VAs, higher dysfluency rates typically occurred with lower usage frequency, with a significant moderate correlation for blocks 
% ($r(29)=-.37$, $p=.024$
% ), and no significant correlations 
% % and interjection($r_\tau$=-0.19, $p$=0.09) 
% for part-word repetitions ($r(29)=-.16$, $p=.206$), whole word repetitions ($r(29)=-.27$, $p=.075$), and prolongations ($r(29)=.47$, $p=.996$). 
% The significant  correlation with blocks resonates with the largest survey concern, which is that people are routinely cut off by a VA when they block. 

% ----------------------------------------

% For dictation usage, there are moderate but significant negative correlations for whole word repetitions ($r(20)=-.47$, $p=.013$) and prolongation ($r(20)=-.41$, $p=.028$), while no significant correlations were found for blocks ($r(20)=-.33$, $p=.065$) or part-word repetitions ($r(20)=.00$, $p=.503$). 
% The significant correlation with whole word repetitions is also congruent with the survey, in which people highlighted words being repeated in their transcriptions. 
% and interjection dysfluency rates. 
% Interestingly, blocks, which is not significant correlated with WER, have a moderate correlation with usage, and again, this is likely due to being cut off when PWS block. 


% \paragraph{WER vs Severity}
% We found moderately-high correlations between A \& H severities and WER ($r_{\tau}$=0.43, $p$<0.001) using Kendall Rank Correlation, which indicates that ASR performance decreases as severity of stuttering increases. 
% We correlated baseline ASR  to stuttering severity with A\&H ratings.
% In this analysis, Spearman Rank correlation was computed since 
% \todo{Colin, what do you think of removing this para since it's redundant with earlier in Sec 4} \note{CL:yes, remove}Recall, A\&H severity is an ordinal variable with values of \{1-\textit{Mild}, 2-\textit{Moderate}, 3-\textit{Severe}\}. 
% No statistically significant correlations between graded A\&H severity and participants perceptions were found,
% however, there were significant positive correlation between severity levels and WER ($r(39)=.52$, $p<.001$) and negative correlation between severity and Thresholded WER<10 ($r(39)=-.50$, $p<.001$).
% Note that none of the Phase 2 participants with survey data were listed as `mild'.


% The ASR model tuned on PWS had better Thresholded WER performance and less variability in model performance for participants with 'moderate' and 'severe'.
%\todo{do we have statistical significance? is Pearson the right test? Bring back Dianna's Kendall number that is commented out? LF: Kendall's tau is probably better, yes. Also, I'm assuming severity was coded as 1-mild, 2-moderate, 3-severe, but this could be clarified. DY: Yes, That's correct. I kept the severity coding the same as what was shared by Colin.}

%\paragraph{Metrics for A\&H Severity} Recall, these A\&H severity ratings are coarse characterizations of how people stutter and simply put people into bins based on overall dysfluency rates (c.f., Section~\ref{participants}, independent of prevalence or duration of each dysfluency type.
% We find that there is a higher correlation between WER and dysfluency rates of specific types -- instead of overall dysfluency rate -- as blocks and prolongations are included in the A\&H scale but do not have statistically significant correlation with WER. 
%Refer back to Figure~\ref{fig:dysfluency_rates} for correlations between WER per participant alongside the rate of each dysfluency type. \todo{move to discussion?}
% (Figure \ref{fig:model_improvement_and_graded_severity}).

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.6 \paperwidth]{figures/WER_Baseline_vs_Tuned_Phase2_avg_and_threshold2.png}
%     \caption{Comparison of baseline and tuned ASR model performance on Phase 2 participants, grouped by survey responses describing voice assistant accuracy.  The improved model had better performance (higher mean fraction of utterances per participant with a low WER) and less variability in model performance for participants with both mild and sever stutters.}
%     \label{fig:model_improvement_and_graded_severity}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.4 \paperwidth]{figures/boxplots_severity_and_wer_metrics.png}
%     \caption{\todo{remove? we show these number elsewhere}Performance of evaluated speech recognition system grouped graded severity. There was a significant, moderate positive correlation between graded severity and average WER ($r=0.36$ \textit{p}: .0080) and a significant, strong negative correlation between graded severity and the average fraction of utterances with a WER <=10 ($r=-0.60$ \textit{p}: 2.57e-6)  }
%     \label{fig:wer_and_graded_severity}
% \end{figure}
%Jaya: Added this in a parallel plots to the ones on self-reported accuracy.  But there is no data on mild stutters for Phase 2, and it may be too much of the same.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.4 \paperwidth]{figures/boxplot_model_improvement_by_severity.png}
%     \caption{\todo{remove?} Comparison of baseline and improved (tuned endpointer) ASR model performance on Phase 2 participants, grouped by survey responses describing voice assistant accuracy.  The improved model had better performance (higher mean fraction of utterances per participant with a low WER) and less variability in model performance for participants with both mild and sever stutters.}
%     \label{fig:model_improvement_and_graded_severity}
% \end{figure}


% ----------------------------------------------------------------------------------------------------
% \paragraph{Correlations with dysfluency annotations}\label{sec: dysRates-correlation}
% To further investigate ASR performance in terms of WER with dysfluency types, we correlated WER and dysfluency types and found that part word repetitions ($r$=0.80, $p$<0.001), whole word repetitions ($r$=0.54, $p$<0.001), prolongations ($r$=0.29, $p$=0.07) had significant correlations, while blocks ($r$=0.10, $p$=0.5) had moderate insignificant correlations. This implies that reducing WER is congruent to improving ASR performance for many dysfluencies and that the largest room for WER reduction could come from improving detection or mitigation of part-word or whole word repetition errors. 

%\todo{This paragraph is to be removed. Discussed with Colin yesterday.}

% We found correlations between dysfluency types but this is not widely known in speech pathology; not sure if this is too big of a claim to make at the moment.
% Also co-occurring dysfluency types:
% Part word repetition rates correlates with whole word repetition ($r$=0.5, $p$=8.4e-4), blocks ($r$=0.38, $p$=0.01), interjections ($r$=0.29, $p$=0.07)
% [TODO:analysis]  how does this impact performance?

% \subsection{Correlations with Survey}\label{sec: survey-results-correlation}
% \subsubsection{Correlation between surveys and results}\label{survey-results-correlation}

%% possible discussion point/finding: can we use correlations between survey and model performance to define a performance metric that better relates to usability/adoption?

% \todo{consider correlations with endpointer}

% Interestingly, the type of dysfluency may have different effects on VA and dictation usage. Comparing to dictation, VA handles a smaller vocabulary and it has a NLU part which helps to recognize the user intent better.

%\todo{key points to make:Performance may be worst and usage may be lower for some dysfluencies. It seems like WER is not strongly correlated to blocks, but blocks are highly correlated to VA usage?}


% \paragraph{ASR performance and reported usage}\label{sec: WER-usage}

% \note{to be removed:} We correlated WER of the baseline system with responses from the survey. 
% As expected, performance was worst for people who reported that their speech was `rarely' understood by VAs (\note{\%}), compared to `often' (\note{\%}) or `sometimes' (\note{\%}) understood. 
% \todo{Colin: Remove? I'm not sure I agree with how these are being discretized; seems confusing}

% We correlated average participant WER of the baseline system with A \& H severity, survey responses on ASR performance and usage. 



% \todo{remove?}
% The following analysis uses Kendall Rank Correlation where stuttering severity is discretized as moderate or severe, performance is defined as how often the participants felt understood by VA assistants and is discretized as "Always/Often", "Usually/Sometimes", "Rarely/Never" as in \ref{fig:understanding_comparison} and usage is discretized as in the `Usage and Utility` analysis in \label{subsec:VAs}. The nominal values assigned to these discrete ordinal variables increase with frequency.
% \note{WER vs Severity}
% We looked at correlations between WER and self-reported VA understanding using Kendall Rank Correlation and found moderate correlation ($r_\tau$=-0.18, $p$=0.10). 
% Similarly, dictation usage has moderate correlation ($r_\tau$=-0.23, $p$=0.08). 
% These results above have P>.05

% \note{WER vs Usage}
% Correlation between WER and reported VA usage is not as strong or significant. 
% The stronger correlation between WER and DS usage may be due the performance of dictation is highly dependent on how accurately speech is transcribed verbatim, whereas VAs have a more abstract task of mapping speech prompts to the correct context and subsequent response. Additionally, from the open-ended responses in our survey, VA usage may not be completely determined by ASR performance, but other personal preferences and characteristics like preferring tactile interfaces, requiring large efforts to speak, or avoidance of speaking in public.

% \paragraph{Perceptions of Speech Recognition Systems\todo{see note}}
% \note{Thresh WER vs Perception}
% Generally, speech recognition systems with WER of 10\% or fewer are considered to have acceptable performance \cite{green2021automatic}.
% Defining the mean fraction of utterances per participant with a WER of ten or less as Thresholded WER, and the average per participant as Average WER, 
% Average WER and Thresholded WER have a strong correlation ($r$=-0.71,  \textit{p}<0.001)
% , but the fraction of utterances with a WER of ten or less is less sensitive to outliers. 
% Thresholded WER also captures how often the speech recognition worked well for a given user, which may more directly relate to usability. 
% \todo{CL: revisit with Jaya's quip on Tuesday https://quip-apple.com/a9BNAzvUAwJC}
% It was observed that there is general tendency that higher WER is correlated with a decrease in perceived ASR performance.
%  as seen in Figure \ref{fig:wer_and_self_reported_va_understanding}, 
% and as described in Section~\ref{sec:survey_results}. 
% We found that Thresholded WER correlated with self-reported VA understanding \todo{add result from below but not sure what test was used}
% 
% average WER and VA understanding: ($r_\tau$=-0.18, $p$=0.10)
% KendalltauResult($r_\tau$=0.18, $p$=0.10)
% threshold WER and VA understanding:
% KendalltauResult(correlation=0.17, pvalue=0.12) 
% 
% \note{WER vs Perception}
% Average WER had a low, non-significant correlation with self-reported voice assistant performance ($r=-0.16$, \textit{p}= 0.26) and 
% Specifically, Thresholded WER (<10\%) had a moderate, significant correlation with self-reported voice assistant performance ($r=0.30$, \textit{p}=0.031).
% grouped by participants' ratings of how often voice assistants understood their speech. 
% For instance, a user for whom a speech recognition system had all but a few utterances with low WER may find the system usable but may have a high average WER if the failure cases had high WERs.  A user with a moderate WER may find a system very unusable if the speech recognition system is consistently not good enough despite having a borderline WER, rarely has a low enough WER to accurately capture their intention.
% \note{Start with this paragraph?}
%\todo{zifang-do this using the tuned model}
% Latest version for Jaya (sept 12)
% Figure \ref{fig:wer_and_self_reported_baseline_and_improved} compares the baseline and tuned ASR model performance on Phase 2 participants, grouped by survey responses for \todo{??}. The improved model had a markedly higher (worse) WER for PWS whose speech were `rarely' understood by the VAs, and the Tuned ASR model is able to significantly improve WER for all three response choices. \todo{@Jaya, do we have statistical significance?}
% Thresholded WER ($<$10\%) had a markedly lower WER for participants who reported that voice assistants for all response choices, especially for PWS whose speech were `rarely' or `sometimes' understood by VA.  This indicates that the model improvements improve performance for those users for whom voice assistants currently do not understand well significantly, especially for people with moderate and severe stuttering.  \todo{@Jaya, do we have statistical significance?}



% With the baseline model for Phase 2 participants only, there was a moderate, negative correlation between average WER and self-reported VA performance (Pearson correlation coefficient -0.34, \textit{p}: 0.069) and a moderate, positive correlation between mean fraction of utterances per person with a WER of ten or less and self-reported VA performance (Pearson correlation coefficient, 0.35, \textit{p}: 0.058).  With the improved baseline model for Phase 2 participants only, there was a moderate, negative correlation between Average WER and self-reported VA performance (Pearson coefficient, -0.37, \textit{p}: 0.044) and a moderate, positive correlation between mean fraction of utterances per person with a WER of ten or less and self-reported VA performance (Pearson coefficient, 0.40, \textit{p}: 0.027).


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.6 \paperwidth]{figures/boxplots_va_understanding_and_wer_metrics.png}
%     \caption{Performance of evaluated speech recognition system grouped by survey responses describing voice assistant accuracy.  Average WER had a low, non-significant correlation with self-reported voice assistant performance ($r=-0.16$, \textit{p}: 0.26) and Thresholded WER (WER$<$10) had a moderate, significant correlation with self-reported voice assistant performance ($r=0.30$, \textit{p}: 0.031).}
%     \label{fig:wer_and_self_reported_va_understanding}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.7 \paperwidth]{figures/boxplots_va_and_dictation_baseline_and_tuned.png}
%     \caption{Comparison of baseline and Tuned ASR models performance on Phase 2 participants, grouped by survey responses describing voice assistant accuracy.  Due to the small number of respondents selected 'Never' (n=0 VA, n=2 dictation) and 'Always (n=2 VA, n=0 dictation), 'Never' and 'Rarely' are presented as a single group and 'Often' and 'Always' are presented as a single group.  The tuned model has better performance for  overall WER (averaged across all words per participant) particularly for participants who reported that voice assistants 'Rarely' or 'Never' understood their speech. 
%     }
%     \label{fig:wer_and_self_reported_baseline_and_improved}
% \end{figure}


% ----------------------------------------------------------------------------------------------------

% \paragraph{Qualitative Error Analysis\todo{LF: see note--tldr is this is interesting but not at required rigor level to warrant inclusion IMO}}\label{sec: clinical-component}

% % \note{consider adding more findings from Lauren's quip Stuttering analyses \url{https://quip-apple.com/lAdnAnuKbaXt} Section: "Cross-subject findings"}

% Lastly, a trained speech language pathologist performed detailed analysis of part-word repetitions. Syllable repetitions were parsed out from sound repetitions and noted to lead to increased word insertions as compared to single sound repetitions.  
% In many cases, this was due to individual syllables being recognized as whole words.  
% For example, if someone produces a syllable repetition on the first syllable in ``become'' (e.g., ``be... be... be...come''), it may be recognized as multiple words. 
% Whereas, if someone produces a sound repetition on /b/ in "become" (e.g., ``b... b... become''') word insertion errors are less likely.  
% People who produce part-word repetitions tend to do so more frequently on initial sounds, which was also reflected in this data~\cite{hubbard1998stuttering}. However, some people also demonstrated part-word repetitions or blocks between syllables in multi-syllabic words.  For example if someone produced a block mid-word in the word “dis...able,” it could be recognized as two words “this” and “able.” If someone produced a repetition mid-word in the word “vocabulary" (vocab..cab.. cabulary) it may break the word down into "vocab cab Cavaleri." These relatively rare occurrences appeared to produce more word insertions. 
% Similarly, audio from participants who interjected ``uh'' between words or those that produced an audible block with vowel like sounds resulted in higher WER. These vowel sounds resulted in word insertion errors.  
 

% ------------------------------------------------------------------------------------------------
\subsection{Summary}

This performance analysis mirrors the primary concerns raised by survey participants and identifies promising directions for improving speech recognition performance for PWS. 
With baseline production-grade models, data from PWS resulted in high truncation rates (23.8\%), often due to blocks, as well as high WER rates (19.8\%), which were dominated by insertion errors. 
Correlating these errors with dysfluency annotations highlighted how different stuttering characteristics can impact different types of errors. 
% Analysis of how specific dysfluency types (e.g., whole and part word repetitions) manifest in ASR transcripts also emphasizes survey participants' concerns about seeing dysfluencies written in their transcribed speech.
%Quantitative results echoed survey findings of PWS being frequently cutoff by VAs due to blocks. 
Fortunately, the three interventions investigated offer improvements for PWS, and can be implemented with limited data and changes to an ASR system. By tuning the endpointer detection threshold on data from PWS, truncation rates on Phase 2 data had a relative average drop of 79.1\% (``mild'') with minor additional system delay of 1.2 seconds.
% \note{or, 96.6\% drop with 2.7 seconds delay} 
% 79.8\% truncation error reduction with 1.2 seconds delay.
%Similarly, we showed that performance of speech recognition systems is worse for many PWS relative to the general population and that transcription errors are dominated by word insertions. Thanks to our fine-grained dyfluency annotations we found that these are highly correlated with part-word repetitions and whole word repetitions.
% and moderately correlated with interjections.
 % PWR($r=0.75$), WWR  ($r=0.48$), Int ($r=0.27$)
Both ASR decoder tuning and dysfluency refinement improve WER compared to the baseline ASR model transcriptions, and combining the two offers a further reduction in WER (relative drop of 61.2\% compared to the baseline ASR model alone for Phase 2 data).

% are especially effective at reducing errors due to whole word repetitions and interjections.
%filler words(Interjection) can be removed with heuristics, ASR tuning alleviates interjections as well but is less effective on part-word repetitions, which calls for future technical ASR work in this area focusing on part-word repetitions. 

%We show two approaches that do not require large amount of speech data from PWS and increase ASR performance remarkably (WER sees a 61.3\% relative improvement with 50.9\% median WER reduction and 70.7\% interquartile range reduction). 
%While Word Error Rates for many users are below a suggested 10\% limit to be considered useful [28] (60.4\%;
%n=55 of 91), performance is far improved for most others.  By refining dysfluency events and tuning ASR decoder, 7 of 21 Phase
%2 participants who were above that limit now see their WER below 10\%.

%While stuttering severity measurements are commonly used for clinical assessments, they only provide a coarse understanding of the interplay between stuttering and speech recognition. For future technical work and data collection efforts, there should be emphasis on prevalence of specific dysfluency types, rates, durations, and vocal characteristics.




==> CHI2023 Stuttering/sections/5-discussion.tex <==
\section{Discussion}
\label{sec:discussion}


Our findings demonstrate the contrasting experiences that PWS encounter with speech technologies, and an overall strong interest in improved speech input accessibility from most survey participants. Off-the-shelf VAs and dictation work reasonably well for many people with mild stuttering severity. The survey shows that many PWS use speech recognition regularly (32.2\% daily), albeit at a lower rate compared to the general population ~\cite{npr_smart_audio}. Moreover, the performance analysis shows that most (84.0\%) participants with mild stuttering severity had word error rates of less than 10\%, a suggested threshold below which VAs can become usable~\cite{green2021automatic}. 

At the same time, participants with more moderate to severe speech dysfluencies often encountered serious technical barriers to adoption. Being cut off too early (with VAs) and ASR accuracy (both VAs and dictation) were primary technical concerns reflected in both the survey and baseline speech analysis: for the Phase 2 participants, truncation rates were substantially higher than the targeted general population rate (23.8\% vs. 3\%) and average word error rate was 25.4\%. We investigated three promising interventions (two new and one previously introduced) to address these issues: (1) tuning the endpointer threshold on moderate dysfluent speech reduces truncations for PWS to below the target of 3\%, (2) tuning the ASR decoder (approach from \cite{mitra2021}) significantly reduces word error rate, and (3) applying dysfluency refinements to the ASR output further significantly reduces word error rate regardless of whether we are using the baseline ASR model or the tuned ASR model. Also of importance, however, our survey highlights that regardless of how well speech technology works, some PWS will still not be interested in it due to perceptions of utility, the physical effort required to speak, and not wanting to use speech input around other people.

Overall, this work is the first to quantify user experiences for PWS, connect those experiences to performance across a range of stuttering severities, and propose and show the impact of multiple technical improvements to support PWS in using speech technology.
We reflect on these findings and potential future research in technical improvements for dysfluent speech and in the design and user experience of such systems. We also cover limitations of the work.

\subsection{Technical Improvements for Dysfluent Speech} 

Our approach has been to identify technical improvements that integrate with rather than replace existing systems, by offering relatively small adaptations to the speech recognition pipeline---changing an endpointer threshold, tuning the ASR's decoder model, and inserting a post-processing step to refine dysfluencies. Moreover, the techniques require very little data compared to what would be needed to train endpointer and ASR models from scratch, and are thus in contrast to many recent papers that replace existing systems with large ASR models trained on dysfluent speech (e.g., \cite{shonibare2022enhancing,alharbi2018lightly,Mendelev2020}) or personalized ASR models that require large amounts of data from a specific person (e.g., \cite{green2021automatic} which requires 15 - 120 minutes of speech). 
% \note{LF: should we mention something here (or is that what cites in previous sentence are?) about personalization work to support people with atypical speech as an alternative to what we've done. specifically how much data have those other approaches used etc.}

% do we want to say anything about end to end models?

% The motivation behind our approach was that our solutions could be complementary to the huge progress in recent end-to-end ASR models. 
% This was validated in Section \ref{sec:asr_over_time} (ASR Results Over Time) where we showed that general ASR advances have a higher have largely improved errors due to part word repetitions whereas our approaches improved more errors due to whole word repetitions and interjections. 
% In recent years, there has been increased interest in enabling speech recognition for PWS or people with other speech differences. 
% Given that our approach can be tacked on to existing models, it is easy to leverage other non-PWS modeling improvements as described in Section \ref{sec:asr_over_time}. 

% Based on analysis in
As shown in Section \ref{sec:asr_over_time}, general ASR improvements do improve performance for PWS, but a substantial gap remains between current and desired performance. While this gap may continue to narrow over time, concerns unique to PWS will likely persist. 
For example, multiple respondents, unprompted, highlighted how word repetitions and interjections in their transcriptions lead to ``errors'' and can result in increased stress or emotional response. 
General ASR modeling innovations typically transcribe verbatim, thus including these unintended words.
As such, human-centered ASR approaches like ours are likely necessary for improving the overall speech recognition experience for PWS. 
% This is also true for endpointing where, to our knowledge, no academic work has gone into improving endpointing due to blocks. 

%While this final results improved performance on our dataset from 25.4\% to 9.8\% for VAs, there are two fundamental limitations. 
The techniques we investigated, while promising, also come with tradeoffs that benefit some users but may degrade performance for others. 
For example, a user who frequently experiences blocks may be happy to increase a VA system's delay in responding if it means that they will be able to use the system more effectively, whereas someone who rarely blocks may be annoyed by the slower response time.
While ideally a single ASR system could apply to all users, one short-term approach is to offer individuals an option to opt-in to specific settings that may benefit them. 
% Although ideally  these tradeoffs mean that any system implementing these techniques should ask users if they want to opt into using them. 
In this case, allowing users to choose between a small set of endpointer options may be useful. 

For ASR decoder tuning, tradeoffs may exist between improved recognition of dysfluent words (e.g., due to part-word repetitions) and a possibly increased error rate for rarer words due to the higher language model weight.
%have \todo{some tradeoff\note{ZH: Similar to the endpointer work, our tuned profile will result in WER for gen-pop increase from ~4\% to ~8\%. We did this evaluation in early 2022. Running both ASR models with SearchOrMessaging (VA task) and Dictation task on 45 standard Siri test datasets, and we see the perf. mentioned above. Maybe we need to consider stating this early on. -- LF: Zifang, those results aren't published though, are they? So maybe we need to say it more hypothetically here}}, 
And, for dysfluency refinement, the system could inadvertently eliminate some words that appear to be dysfluencies but were intentional on the user's part (e.g., removing the duplicate ``so'' in ``I am so so happy'').
% For the latter, for example, a user could say ``I am so so happy'', intentionally repeating ``so'' to indicate emphasis, but that could be corrected to a single ``so'' depending on how the dysfluency refinement is implemented. 
In the short-term, ASR decorder tuning and dysfluency refinement could also be enabled as opt-in features, though future work should investigate how to seamlessly integrate them into general ASR systems. 
For example, an improved dysfluency refinement approach could learn to distinguish dysfluent from intended repetitions, handle partial word repetitions in addition to whole word repetitions and interjections, and even learn filler word patterns unique to a given person. 
% Ultimately, however, there may still tradeoffs that would be acceptable to some users but not to others who already experience strong baseline system performance.

We focused on endpointing and ASR solutions, but two additional technical concerns that arose with less frequency in the survey data are wake words (e.g., ``Alexa'', ``Hey Siri'') and automatic punctuation. Offering multiple wake word alternatives, custom wake words, or flexibility in the pause length between words so as to accommodate blocks could improve accessibility for these users. 
%An alternative is to improve performance of existing wake words for PWS. For example, for multi-word phrases, there should be flexibility in the duration of pauses between words.
% \note{see hidden technical bits}
% From a technical standpoint, recent wake word models are frequently based on 1D convolutional networks (e.g., \cite{X,Y,Z}), which generally have a maximum detection window, meaning if it takes longer than 1 second to say the wake word then it will not fire. 
% For multi-word phrases, such as ``OK Google,'' if someone blocks between words then the wake word likely will not fire. New investigations could identify how to dynamically recognize these words with dysfluencies. 
For automatic punctuation, multiple respondents mentioned punctuation being inserted incorrectly during pauses in speech. 
% \todo{find a few papers?}
Effort should be made to understand how blocks and pauses impact current punctuation models and if there are ways to avoid incorrectly inserted punctuation.

\subsection{Additional Design and User Experience Considerations}

%[personalization]
%One line of future work is to investigate how this tuning can be adjusted on-the-fly depending on an individuals needs. 

%Our approaches significantly reduce WER in utterances with blocks, word repetitions, and interjections, however, part word repetitions are still especially problematic. 
%In Section \ref{sec:asr_over_time}, we saw that general improvements to ASR systems do appear to improve these errors. 
%Automatically detecting part word repetitions is challenging and often results in word insertion errors. 
%To improve these, end-to-end models or more sophisticated approaches that leverage sub-word repetitions may be necessary. 

% In addition, it may be possible to learn or add new words to the list of interjections, on top of ``um'' and ``uh,'' to improve error rates even more. Filler words unique to the person

%More work should be done to identify efficacy for non-PWS on enabling methods that work well for both PWS and non-PWS. 


% \note{modeling: keep it simple! end to end models may improve partial words, but these things have a large impact and can be glued onto other systems}


% In our experiment, we normalized text before calculating WER, i.e.  minor discrepancies between numbers and their Arabic numerals format, pluralizations, and etc. 


%\paragraph{The interplay between stuttering characteristics and speech recognition }

A key next step will be to validate our speech experiments by incorporating the three technical improvements into a fully interactive system to evaluate with PWS. Such an evaluation will allow us to understand the extent to which the offline experiments here translate to impacts on user experience and satisfaction with speech input---fully closing the loop with the subjective experiences reported in the survey. Understanding how users feel about the tradeoffs described above (e.g., truncation rate vs. response delay) and what dysfluencies they want to have refined in their transcribed speech will be important. Preferences may vary greatly across individuals, for example, with some not wanting the system to ``fix'' their transcribed speech.

In addition to the above model-side improvements for PWS, there is potential for some challenges to be addressed through more interactive approaches. One possibility is for users to provide feedback directly to the system, training it to better support their own stuttering patterns and to accommodate their desire for different types of refinements. For dictation and screen-based VAs, this type of feedback could occur by displaying the transcribed speech and allowing the user to manipulate it through direct touch to indicate error words that should be removed or corrected \cite{dictation_user_expectations}. 
% \todo{CL: Dianna, I think you had a citation for something like this? DY: as suggested, I tried to find citations related to VA and dictation. See adjusted text in this paragraph}. 
Perhaps the first time a pattern is encountered, such as a suspected full or partial repetition of a specific word or a transcribed interjection from a list of common interjections (e.g., ``um'', ``like''), the system could prompt the user to indicate that it should hide or repair future similar dysfluencies from transcripts. 
% Correction feedback for purely voice-based interaction such as on screenless voice assistant devices is more difficult, because unlike screen-based devices the user may not see what words were predictd. 
%\todo{LF: need to discuss. I don't know that these speech-only techniques designed for non-PWS would necessarily work well for PWS who are experiencing dysfluencies already }For a hands-free experience, findings from user studies\todo{LF: with non-PWS?} suggest a preference for using Text To Speech (TTS) technology to vocalize the transcription so that the user could hear if dictation was correctly transcribed and issue corrections through voice commands \cite{dictation_user_expectations} whereas for VAs, correction can be done through natural conversation through clarifying questions \cite{repairing_VA_errors}. 

Correction feedback on screen-free voice assistant devices is more difficult, because the user may not see what words were predicted; they may only receive notification of what VA action was performed.  
% , and the characteristics of the errors themselves are not as evident because they are not typically explicitly shared back but rather manifest in VA response errors. 
% One possibility could be to expect that speakers might rephrase the command using words that are less likely to make them stutter, and this rephrasing could be used to help the system learn from the previously incorrectly interpreted command.
One possibility would be to learn how speakers rephrase their command when the voice assistant suggests a wrong action, which could be useful if an individual intentionally chooses new words that they are less likely to stutter on. 
Some current systems also allow users to review the recognized text on another device (e.g., Alexa's smartphone app), and could potentially be extended to allow users to correct the transcription. 
Any of these forms of correction could ultimately be incorporated into the system to personalize speech recognition.
%design of a user-friendly error feedback interface for PWS. reviewers asked for design of a user-friendly error feedback interface for PWS. Maybe this could refer to existing captioning error feedback and dictation error feedback approaches, but also mention customization so that people could choose to hide dysfluencies if they want overall, and perhaps tap to unhide. Maybe also some kind of personalized component where people can click an error and also specify that it's a common error pattern for them that the system should learn and hide in the future. \note{DY: The findings from \cite{remote-co-design-captions} suggest that ASR errors should be clearly visualized, such as by adding underlined color, symbols, or changing the boldness or colors of the font. To correct the error, different UI designs were suggested such as including a small pop-up with options for repeating verbally or fixing manually with typing or tapping from a selection of suggested words. Once corrected, the corrected words should also have a visual indication. Some suggested an insertion of asterisk, colored text or a [CORRECTED] tag.}


The design of any speech interface for PWS will need to also account for non-technical contextual factors around use. As demonstrated in survey responses, some PWS may find their ability or desire to use speech technology will differ depending on whether other people are around (some respondents did not want others to hear them speak). Further, some participants reported that their stuttering severity varied based on their history with the device, for example, increasing following a negative interaction with the device. Both of these scenarios emphasize the importance of supporting PWS in seamlessly transitioning from speech to text-based input as needed, and ensuring that speech is never the only means of accomplishing a task.

Emphasizing the utility of combining multiple modalities of input for PWS, most survey participants (84.7\%) used VAs on a smartphone, and some responses pointed to the accessibility benefits of doing so. Speech affordances vary greatly on smartphones versus smart speakers, with smartphones offering alternative invocation mechanisms such as holding a physical button to speak or pushing a virtual button on-screen.
In addition, holding a button (e.g., on iOS)
%at least\note{LF: does anyone know on Android devices?\note{In Sec 2 Related Wrok, we had a sentence saying "Instead of using a speech-based invocation mechanism on a phone or tablet, a user may hold down a button on the side of the device (``Hold to Speak'' on iOS) or squeeze the side of the phone (some Android devices)."}\note{LF: okay, does that mean 100\% that the endpointer is disabled? I don't have experience with it on Android}}, if this button is held down long enough the 
can disable the endpointer, meaning a user will not be cut off mid-utterance. 
These features are also available on some smartwatches, but not at-a-distance devices like smart speakers. 
%For some users, the dictation experience may be easier on a smartphone or other device with a screen, as the transcription may be displayed for the user to visually review. And if there is an on-screen keyboard they can revise this transcription by hand. 
Future work should investigate alternatives that improve these experiences on screen-free devices. 


\subsection{Beyond Fluency}
While the primary focus of this paper is on stuttering, the interventions may improve speech recognition for people with other types of communication disabilities. 
For example, endpointer improvements may improve performance for people with hypokinetic dysarthria that experience unpredictable silences (e.g., Parkinson's Disease) or hyperkinetic dysarthria that experience intermittent aphonia or voice stoppages in their speech (e.g., Tourette syndrome) \cite{duffy2019motor}.
% Similarly, people with hyperkinetic dysarthria may experience intermittent aphonia and voice stoppages \cite{duffy2019motor} which could also be recognized as the end of a phrase when not intended.  
These improvements may also affect individuals with expressive aphasia who take longer to come up with a target word \cite{evans2020much}.
% may also be cut off early.  
% In terms of removing or increasing time before endpointing, people with hypokinetic dysarthria (e.g., some people with Parkinson's Disease) experience unpredictable silences in their speech \cite{duffy2019motor} which could then cut them off when using ASR.  
% Similarly, people with hyperkinetic dysarthria may experience intermittent aphonia and voice stoppages \cite{duffy2019motor} which could also be recognized as the end of a phrase when not intended.  Individuals with expressive aphasia who take longer to come up with a target word \cite{evans2020much} may also be cut off by an early endpointer.  
Dysfluency refinement could improve WER for individuals with spasmodic dysphonia and hypokinetic dysarthia as they may produce part- or whole word repetitions~\cite{goberman2010characteristics,juste2018frequency}.
% \cite{tichenor2021variability}
People with spasmodic dysphonia may present with an increase in interjections \cite{cannito1997disfluency}, which could be removed with Dysfluency Refinement or ASR Tuning. 
% Removal of short interjections such as ``u'' could improve WER.  

Other speech, voice, or language differences not addressed by this work include:
% speech, voice, dysfluency, and language differences that include characteristics such as:
breathy breaks mid-word that can cause word insertions and substitutions (e.g., in cases of spasmodic dysphonia \cite{murry2014spasmodic}), 
% prolonged and 
distorted vowels which could result in word substitutions  (e.g., in cases of ataxic and hyperkinetic dysarthria \cite{duffy2019motor}), 
pitch breaks (e.g., in cases of flaccid dysarthria and some voice disorders \cite{duffy2019motor}),  
atypical rhythm and stress (e.g., in cases of flaccid and hypokinetic dysarthria \cite{darley1969differential}),
speech characteristics that deteriorate or change over time (e.g., in cases of Amytrophic Lateral Sclerosis (ALS), some voice disorders, and some dysathrias), and 
vowel neutralization and differences in resonance (e.g, in cases of speech from Deaf/Hard of Hearing individuals \cite{subtelny1992spectral}).

\subsection{Limitations and Potential Biases}
\label{discussion_limitations}

%\paragraph{Audio Recordings}
Speech characteristics can vary with time and with settings, as noted above and in the literature (e.g.,~\cite{tichenor2021variability,bleakley2022exploring}), so our collected audio data does not provide a full view of speech characteristics for each participant. 
Recordings were done at an individual's convenience, while by themselves, which likely impacted the prevalence and severity of dysfluencies.
Some users may have had more dysfluencies because they knew they were being recorded, while others may have had less because they could do it when they felt most comfortable. 
One improvement on our methodology would be to ask participants to record commands at different times of the day, in different environments, and perhaps different situations where their dysfluency patterns might be different. We also focused solely on speech accessibility and did not ask participants if they had other accessibility needs for computing devices---which could impact the effectiveness of some solutions like pushing a button to invoke a voice assistant.
% Most participants reported in the survey that their speech characteristics varied with time -- of the 61 surveyed participants, only one said that their speech was 'always' the same.  
% Other participants reported that their speech varies throughout the day (n=17), varies day-to-day (n=25), or changes progressively over weeks or months (n=18).

The fine-grained dysfluency annotations enabled detailed analysis of how rates vary per-person, however, there were two types of annotator errors that we estimate to have impacted a small percent of clips. 
%Despite each annotator being given training on how to best label each dysfluency type, we found some inconsistencies. 
We found that some dysfluency types conflated for one-another. For example, some sound or part-word repetitions (e.g., ``s-s-snake'') were conflated with prolongations (e.g., ``ssssnake'') and vice versa. 
This means that there may be discrepancies between our reported dysfluency correlations and the actual correlations. 
% ... \todo{tips for better annotations?}
Second, with the transcript annotations, people were asked to label both the articulated and the ``intended'' speech. Ideally, the intended speech would have been verified by participants; instead it was labeled with an annotator's best guess based on context. 
In a small percentage of clips we found likely discrepancies and in many cases improved with an annotation refinement pass. 

Quality of ASR results varies significantly as a function of uniqueness; common VA queries or dictation phrases may be more likely to be accurately recognized and rare words or phrases are less likely. 
This is even more the case with our ASR tuning approach, which biases the language modeling priors over the acoustic information. 
Given that the majority of the audio recording prompts were VA-related---albeit with proper nouns such as musician names---our WER may be lower than what one might expect in the real-world, especially for dictation which is more open ended. As emphasized above, a key step for future work will be to evaluate the improvements proposed here with PWS using a fully interactive system. 

The findings in Section \ref{sec:asr_results} are derived using an ASR system with a hybrid architecture, specifically with the Apple Speech Framework. 
ASR systems trained with different data or architectures could exhibit different model biases, as seen in our analysis in Section \ref{sec:asr_over_time}, where each model exhibited different performances and biases toward certain dysfluency types. Nonetheless, our general findings of poor WER performance for stuttered speech is congruent to similar WER analysis conducted on other ASR systems using different architectures \cite{shonibare2022enhancing, AlharbiWOCCI17,alharbi2018lightly}. 






==> CHI2023 Stuttering/sections/6-conclusion.tex <==
\section{Conclusion}

In this paper, we described survey findings from 61 people who stutter and performed speech recognition experiments on a 91-person collection. We found that some PWS already use speech recognition systems regularly, some state that they would never be interested, but regardless of existing performance over half of respondents would use speech technology more frequently if they were more accurate. 
While our speech recognition results indicated worse baseline performance relative to the general public, especially for people with higher rates of dysfluencies, our model tuning and dysfluency refinement solutions can drastically reduce endpointing and ASR error rates, and ultimately enable ``good enough'' (WER$<$15) performance for most users. 

\section*{Acknowledgements}
Thanks to Shrinath Thelapurath, Zeinab Liaghat, Hannah Gillis Coleman, Adriana Hilliard, Chris Maury, Carolyn Feng, Gautam Varma Mantena, and Leo Liu for various discussions and study related tasks. 

==> CHI2023 Stuttering/sections/old-method.tex <==
% \section{Methods}
% \note{likely integrate 'Methods' with other sections'}


% Our goal is to understand the experience of speech technology on PWS, how well existing systems work subjectively and quantitatively, where they break, and areas for improvements. 
% % We analyzed interest, usefulness, and performance of speech recognition systems for PWS in two ways. 
% We did this in two ways: through a comprehensive survey to understand the perception of PWS and through a user study where participants recorded hundreds of audio clips that could be used for Voice Assistant and Dictation tasks. 
% We performed baseline ASR, endpointing, and intent recognition experiments and report results in Section~\ref{sec:asr_results}. 
% % as well as production-oriented experiments that could be used to improve performance for PWS. 
% Most participants overlapped between the two data modalities so we also looked at correlations between system performance and survey results. 


% \subsection{Survey Design}\label{survey_design}

% Our survey was split into the following four primary sections and included up to \note{87} questions depending on conditional logic. For an expanded listing of survey questions see the Supplementary Material.\todo{verify we can release.}
% \begin{description}
%     \item[Background] Demographics (age group, gender, race/ethnicity); self-description of speech characteristics; intelligibility of speech to family/acquaintances/strangers; ownership and usage of smart devices.

%     \item[Voice Assistants] Usage, usefulness, and accuracy of VAs; why and when do they use VAs; when do they break and areas for improvements; awareness and effectiveness of features including endpointing, hold-to-speak, invocation models, and other common features. 

%     \item[Dictation Systems] Usage, usefulness, and accuracy of DSs; why and when they use DSs; when do they break and areas for improvements; awareness and effectiveness of relevant features, whether people revise or restate transcriptions upon error. 

%     \item[Future Ideation] Interest in VAs/Dictation if speech was perfectly transcribed; interest in personalizing/training models to improve performance; alternative speech-related features.

% \end{description}
% Many of these questions had multiple choice responses and open-ended text input to explain why they chose each response. For questions related to the endpointer and other technical material, layperson descriptions like "How often does a VA cut off your speech" were used. 

% Surveys were filled out online using a commercial survey website. Most participants took 30 to 45 minutes, which and the surveys were collected over a two-month period in Summer 2022. 

% \note{here we talk about did we need to discard any responses and why, how did we analyze the open-ended responses. If we do any statistical analysis we can describe that here.}


% \subsection{Speech Data Collection}

% Each participant was asked to record \todo{121 VA query + 10 dictation if they recorded any dictation messages} audio clips using a smart phone on their own in a quiet environment (SNR > 30 dB). The phone was located about two feet in front of them either in their hand or approximately in that position. Of these clips, 121 were based on Voice Assistant related prompts and others consisted of fake text messages that they might send to a friend, which are more appropriate for the Dictation use case. People were told not to include personal or identifiable information (PII) and this was verified by an outside group. 
% % Audio clips were single phrases or sentences and ranged from two to \_\_\_\_\todo{the range is 1 to 49 words, median is 6 and average is 5.8} words. 
% Audio clips were single phrases or sentences, with a minimum of two words an median of six words.

% Participants were asked to speak naturally. Instead of providing pre-defined phrases, they were given prompts where they came up with their own phrase to accomplish a given task. For example, they were asked to say a phrase to: ``Find out when a place you might want to visit will open,'' ``Find the lyrics to a song that you like,'' and ``Ask about a question about something not well known.'' A complete set is included in the Supplemental Material \note{Can we include?}. 

% All audio clips were manually annotated with the prompt, the phrase they intended to say (e.g., ``what is the weather'', the articulated phrase with dysfluencies (e.g., ``wuh-wuh-what is [...] the weather,'' and an annotation for each dysfluency including starting frame, ending frame, and type. Four stuttering events were noted: part word repetitions, whole word repetitions, sound prolongations, and audible and inaudible blocks.  Interjections were also noted.  A speech language pathologist estimated stuttering severity (no stutter, mild, moderate, severe) per participant using the Andrew and Harris Scale (A\&H) Scale~\cite{?} by grading 100-300 word audio clip samples. the Andrew and Harris scale

% % \textbf{Do we have an explanation for this?: Eight survey respondents did not have annotated data and were not included in the evaluation of speech recognition models.}.

% PWS vary in terms of how many and what types of dysfluencies they produce. This is fluid; someone may produce more or fewer dysfluencies depending on the setting or environment, current mood/stress level, communication partners, or other variables.  Some people stutter frequently when in a group but not when on their own. Some people stutter more when in front of a smart device because of ``pressure to perform.'' The process of creating these audio recordings -- which were done at an individuals convenience while by themselves -- undoubtedly biased the prevalence and severity of stuttering events. For some users events were likely  higher because they knew they were being recorded and for others was likely lower because they could do it when they felt most comfortable. 

% % \subsubsection{Speech Recognition Results}

% % We used production-like models similar to what are deployed for Siri on iOS. Specifically, the endpointer, ASR model, and intent recognition component of the NLU model. 

% % \todo{what details can we use? look at how we did it for the Interspeech paper. }


% \subsection{Participant Recruitment}
% Participants were recruited through social media, referrals from speech language pathology clinics, and word of mouth. Individuals self-identified as having a stutter. An SLP also screened the individuals by listening to their connected speech and by observing overt stuttering characteristics.\note{Colin mentioned there were 4 tasks the vendor's SLP used to screen and grade a participant)}
% The participants who presented as people who stutter were included and graded using A&H Scale into mild, moderate, and severe stuttering groups to ensure adequate severity distribution. In total \note{61} people filled out the survey and \note{91}  contributed audio recordings. 
% % \note{technically 100 people for audio, but we don't have annotations for 8}.
% % \todo{how do we want to discuss Phase 1 and Phase 2? should they be merged entirely? there are some protocol changes like the connected speech sample}
% Of these individuals, [X] were rated as mild (0-5\% of words have dysfluencies), [X] mild (6-20\% dysfluencies), and [X] severe ($\geq$20\% dysfluencies) using the A&H scale. 
% % \subsubsection{Dataset Overview \& Dysfluency Analysis}

% % * Mild: 0-5\% of words have a dysfluency (2 participants in Phase 2)
% % * Moderate: 6-20\% of words have a dysfluency (12 participants in Phase 2)
% % * Severe: >20\% of words have a dysfluency (27 participants in Phase 2)

% % \todo{Maybe add some distribution plots of annotations? Or wait and add correlations with WER and/or truncation rates?}.  %note: I added some plots of correlations with stuttering severity and WER to 4.3.2, they could be moved here


==> sections/2-relatedwork-old.tex <==
\section{Background \& Related Work}
\todo{swap sections; add some more details to ASR; move ASR related work to ASR background}

% \subsection{Background on Stuttering \todo{move or incorporate elsewhere}} 


% Individuals may develop reactions to speaking in various situations leading to avoidance of target words, sounds, or speaking situations and observable escape behaviors such as foot stomping or eye blinking. 






% Stuttering and cluttering are types of fluency disorders, defined by an interruption in the flow or fluidity of connected speech.  Stuttering is more common and may also be referred to as stammering~\cite{ward2011cluttering}.  Stuttering is a breakdown in speech fluency that can affect the rate and flow of speech and can include specific dysfluency types, such as sound (``p-p-pop'') and syllable repetitions (``be-be-become''), word repetitions (``mom, mom, mom``), sound prolongations (``mmmmmom''), and silent or audible blocks (inability to initiate target sound) \cite{sander1963frequency, SSI}. Frequent interjections (``um'', ``eh'') are also common.  

% PWS typically cannot control when their stuttering will occur and cannot control how people or technology perceive and respond to their dysfluencies. 
% The setting or environment, current mood/stress level, communication partners, or other variables can impact stuttering.  Some people stutter frequently when in a group but not when on their own \cite{tichenor2021variability}. Some people stutter more when in front of a smart device because of ``pressure to perform.'' 
% Individuals may develop reactions to speaking in various situations leading to avoidance of target words, sounds, or speaking situations and observable escape behaviors such as foot stomping or eye blinking.  
% Over time, a PWS may also experience negative psychological outcomes such as social anxiety, low self-esteem, and negative feelings about communication~\cite{boyle2015identifying}. This can be a cycle as increased anxiety may then lead to an increase in producing stutter events.  
% Stuttering may be developmental, neurogenic, or psychogenic \cite{roth1989clinical, seery2005differential}.  

% PWS vary in terms of how many and what types of dysfluencies they produce. 
% The frequency of dysfluencies, duration of dysfluencies, physical concomitants (i.e., stomping a foot, moving hands), and the impacts that stuttering has on participation in communication across settings varies significantly across individuals \cite{tichenor2021variability}. These overt cues are used in clinical settings to assess severity and changes over time~\cite{SSI,yaruss2006overall}. 
% In this work we used severity to recruit participants, but ultimately find a more nuanced understanding of the rates and characteristics of each dysfluency type and their impact on speech recognition technology.  


% Multiple factors are considered when clinically assessing stuttering severity including . 
% We are working to improve ASR so that PWS can be successful and more confident with use of speech recognition.   

% [\textbf{TODO}\textbf{: change citations and put in bibliography]}

% @article{boyle2015identifying,
%   title={Identifying correlates of self-stigma in adults who stutter: Further establishing the construct validity of the Self-Stigma of Stuttering Scale (4S)},
%   author={Boyle, Michael P},
%   journal={Journal of Fluency Disorders},
%   volume={43},
%   pages={17--27},
%   year={2015},
%   publisher={Elsevier}
  
%   @book{ward2017stuttering,
%   title={Stuttering and cluttering: frameworks for understanding and treatment},
%   author={Ward, David},
%   year={2017},
%   publisher={Psychology Press}
% }
  
%   @article{yaruss2006overall,
%   title={Overall Assessment of the Speaker's Experience of Stuttering (OASES): Documenting multiple outcomes in stuttering treatment},
%   author={Yaruss, J Scott and Quesal, Robert W},
%   journal={Journal of fluency disorders},
%   volume={31},
%   number={2},
%   pages={90--115},
%   year={2006},
%   publisher={Elsevier}
% }
% Riper~\cite{VanRiper1982}, SSI-4~\cite{SSI}, Andrew \& Harris~\cite{andrews1964syndrome}, Time-interval measurement~\cite{valente2015event,ingham1993time}.




% ------------------------------------------------------------------------------------

\subsection{Related Work} %HCI \& Technical Literature}
A wide range of people with disabilities use voice interaction which enables people with motor disabilities to control computing devices with speech commands (e.g.,~\cite{zhong2014justspeak, corbett2016can}). It is also an inherently accessible input modality for many blind and low vision users (e.g., ~\cite{pradhan2018accessibility, abdolrahmani2018siri}). However, this work often assumes that speech input itself is accessible.

% Focusing on studies with users who have atypical speech, 
Researchers have captured speech input challenges encountered by people with dysarthria~\cite{ballati2018assessing,projecteuphonia}, deaf or hard of hearing people~\cite{fok2018towards}, and people with aphasia~\cite{roper2019speech}. 
For stuttering specifically, there has been relatively little human-centered work~\cite{clark2020speech}. A recent exception comes from Bleakley et al.~\cite{bleakley2022exploring}, who report on interviews and a three-week diary study of smart speaker use at home with 11 PWS. 
%Usage followed patterns typical of the general population (e.g., music and information queries were most common). 
While participants had ``some success’’ in using the device, challenges included the device timing out, social pressure when using the device around other people, and difficulty with specific sounds (especially that could interfere with the wake word, i.e., ``OK Google’’). Participants reported repeating and reformulating utterances to overcome these issues. While this study provides an initial understanding of how PWS use voice assistants, it does not report the stuttering severity of the participants and does not provide an objective assessment indicating how well the smart speakers recognized their speech. In contrast, our study examines speech input technology more broadly (e.g., including dictation), and includes both quantitative subjective data from a larger sample of (n=61) PWS and system performance on stuttered speech samples collected from (n=91) PWS. 

% Beyond Bleakley et al.'s study on speech input accessibility and stuttering~\cite{bleakley2022exploring}, 
A few other human-centered projects have looked at supporting speech therapy for PWS and at managing stuttering in everyday life. Demarin et al.~\cite{demarin2015impact} and Madeira et al.~\cite{madeira2013building} both present apps to record stuttering experiences with the goal of increasing awareness and informing therapy decisions; small user evaluations included 2 and 5 PWS, respectively.
Focused on managing speaking situations, Fluent~\cite{ghai2021fluent} supports people in writing scripts that they will be more likely to read aloud fluently. The tool uses active learning to identify words that the user is likely to encounter issues with, and suggests alternative words that may be easier to speak; no user study has been reported. Finally, McNaney et al.~\cite{mcnaney2018stammerapp} employed a multi-stakeholder co-design process to design StammerApp, a mobile app that allows users to set goals, practice, and reflect on their experiences in especially challenging situations. While the project did not focus on speech input, it provides a qualitative understanding of a total of 39 participants’ experiences with stammering, including specific challenges (e.g., talking on the phone), and a general desire to be able to ``stammer openly and feel more confident and relaxed with their own voice''. Ultimately, our goal is for PWS to have this freedom and confidence when interacting not only with other people, but with speech input technology as well.


Technical work on improving speech assistants for PWS has focused on Automatic Speech Recognition (ASR) models~\cite{shonibare2022enhancing,Mendelev2020,gondala2021error,mitra2021,Tripathi2018,Tripathi2020,HeemanInterSpeech16}, stuttering detection~\cite{LeaStutterDetection2021}, dysfluency detection or classification~\cite{lea2021sep,kourkounakis2020detecting,Mahesha2016,DasNSRE2020,riad2020identification}, clinical assessment~\cite{BayerlTSD2020}, and dataset development~\cite{FluencyBank,UCLASS,lea2021sep,KSoF}.
% Much of this work has centered on dysfluency detection either as a standalone task or as part of an ASR system. 
% Three ASR-oriented approaches are as follows. 
Shonibare \etal \cite{shonibare2022enhancing} and Mendelev \etal  \cite{Mendelev2020} investigate training end-to-end RNN-T ASR models on speech from PWS. 
Shonibare \etal\ introduces a detect-then-pass approach that incorporates a dysfluency detector where audio frames with dysfluencies are ignored entirely by the RNN-T decoder. 
Examples in the paper demonstrate how this can be used to ignore some partial-word repetitions and blocks.
% The temporal context is very short (100 ms) so it is unlikely to generalize to whole word or phrase repetitions or to inaudible blocks mid-word. 
Mitra \etal \cite{mitra2021} describes a fine-tuning approach for Voice Assistant tasks that can be applied on top of existing ASR models, which does not require as much data as end-to-end solutions.
% which may be production-oriented 
% It is challenging to get large amounts of stuttered speech data and moreover dysfluency detection labels, so investigated 
% optimizing a small set of ASR decoder parameters on stuttered speech, such that the system is biases towards more common phrases and shorter phrases without repetitions.
%  for Voice Assistant task
Their system optimizes a small set of ASR decoder parameters on stuttered speech, such that the system is biased towards more common phrases and shorter phrases that remove sound and partial-word repetitions. 
% and Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly}
Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly} focused on stuttered speech from youths and incorporates the structure of repetitions and other dyfluencies into an augmented language model that is better at including dysfluencies in a transcription. 
% \note{[mention Mendelev which just trained an RNN-T model with a tiny amount of stuttered speech and tries replacing partial-word annotations with another symbol. ] [Neither paper uses absolute WER! only relative. ]} 
Efforts from Project Euphonia~\cite{projecteuphonia}, the largest atypical speech project to date, have included data from PWS but it has not been a core focus in publications.
% \todo{mention limitations and connections to our work}

\note{need to figure out whether to keep this content or not}Speech has also been explored as a form of input for augmentative and alternative communication (AAC) systems, which are traditionally controlled through touch, gaze or switch input. 
The VIVOCA project, for example, recognizes spoken input from users with atypical speech by training a personalized limited vocabulary speech recognition model that can activate pre-defined synthesized speech output~\cite{hawley2012voice}. Speech recognition has also been employed for speech therapy goals---including using both off-the-shelf systems such as smart speakers (e.g., \cite{smith2021smart}), and custom-designed games to increase enjoyment of speech therapy exercises, such as Apraxia World~\cite{hair2018apraxia}.


% There has been significant interest 
% [Project Euphonia has stuttering data as well but I can't remember seeing anything stuttering-specific that they've worked on.]



%%scratch (could remove)
% \subsection{Voice Assistant Usage}


% ------------------------------------------------------------------------------------------------------------------
\subsection{Background on Speech Recognition Systems}
% \todo{Refactor and trim this section.}

Our goal is not only to understand perceptions of speech technology for PWS, but to achieve a deeper understanding where existing pipelines break and technical avenues for improvement. 
% In this paper, we focus on two applications: . 
In this section we describe common pipelines for Voice Assistants and Dictation Systems and in Section~\ref{sec:asr_results} evaluate constituent models.
% \note{Should we mention why VA and DS versus any other tasks?}
% While these two systems are similar, their use cases and limitations 

% We chose VAs because they are ubiquitous in smart phones and speakers and can be an important access tool, especially for people with motor disabilities. 

\note{An attempt to describe ASR before we talk about VAs and DSs.} 

Voice assistants and dictation systems rely on automatic speech recognition (ASR) technology. On a high level, ASR uses machine learning algorithms to convert spoken language to text. Traditionally people use a Hybrid Approach to build an ASR~\cite{KelseyFoster}. It usually consists of a lexicon model that provides pronunciation knowledge, an acoustic model that models acoustic patterns, and a language model that gives information about word sequence likelihood, and finally a decoder that utilizes all above information to produce a transcription~\cite{gondala2021error}. With the emerging of deep neural networks recent years, components such as acoustic model in the hybird ASR adopts deep neural networks to improve ASR performance~\cite{AlexGraves} while an end-to-end deep learning approach of building ASR system sprung. An end-to-end ASR directly maps a sequence of input acoustic features into a sequence of words~\cite{AlexGraves}, instead of having separately trained acoustic, pronunciation and language model components, 

Though end-to-end systems reduce efforts needed from domain experts (for example for lexicon expert phoneticians need to handcraft a phoneme set for each language) and tends to outperform hybird models~\cite{AwniHannun}, hybird ASRs are still dominantly used in commercial VAs and DSs ~\cite{KelseyFoster}.
% though many companies are transitioning to an end-to-end approach. 

% TO be cited:
% Deep Speech: Scaling up end-to-end speech recognition. Awni Hannun
% Towards End-to-End Speech Recognition with Recurrent Neural Networks, Alex Graves
% Need to cite this properly: https://www.assemblyai.com/blog/what-is-asr/, Kelsey Foster

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6 \paperwidth]{figures/VA_Illustration.png}
    \caption{Simplified Workflow and Components of a Voice Assistant. Figure adapted from \cite{ranantha2020intent} 
    % \todo{to be updated}\todo{replace user head. I think this was taken from some random website based on a reverse image search}  
    }
    \label{fig:VA Illustration}
\end{figure}
% \note{colin: (1) Can "Behind the Scene" be renamed to "Voice Assistant Models, and (2) "When do I endpoint" be changed from a thought bubble to something else? It is a model... and thus there should be a blue box, but it's iterative so I don't know the best way to display with this graphic.}
\textbf{Voice Assistants} (e.g., Amazon Alexa, Apple Siri, and Google Assistant) listen for spoken questions or commands. For example, ``What is the weather?'' or ``Set a timer for five minutes.'' 
% They usually have a spoken response but some can also show visual information. 
A typical user flow is as follows and as shown in Figure~\ref{fig:VA Illustration} . 
A user may start by using an \textit{wake word}, such as saying ``Alexa'', ``Hey Siri'', or ``OK Google,'' to initiate a query. This may also be called \textit{Invocation}. 
% On most smart devices there is an always-running invocation model that attempts to recognize one of these phrases. 
They then start to vocalize their command. 
% \note{we usually call this payload... I see it mentioned below in text only so not sure we want to introduce term: trigger=wake-word + command=payload]}
% , such as ``What is the weather?'' 
As the user speaks, an \textit{ASR} model takes this speech and transcribes the words being said.
% , typically verbatim. 
Meanwhile the system tries to automatically detect when the user has finished their phrase using an \textit{endpointer} model. This can also be referred to as an end-of-speech detection model. 
% , which uses cues like how much time has elapsed since the last vocalization to know when to perform recognition.
Finally, a \textit{Natural Language Understanding (NLU)} model takes the predicted phrase and metadata output from the ASR and identifies the user's intent and how to respond. 
Based on the user's query, the VA may respond with information, perform a command, ask the user a follow-up question, or notify the user that the query could not be understood. 
% Note that a streaming version of the ASR model may be run while the user is still speaking, and the prediction may be displayed on-screen so the user gets feedback on what the system thinks the person is saying.

% No less than three models are run on this speech. An \textit{endpointer} model computes the likelihood that a person is finished speaking so the system knows when to respond. An \textit{Automatic Speech Recognition (ASR)} model takes the speech and attempts to identify the words being said. Finally, a \textit{Natural Language Understanding (NLU)} model takes the predicted phrase and metadata output from the ASR and identifies the users intent and how to respond. Based on the query, the VA may respond with information, perform a command, ask the user a followup question, or notify the user that the query could not be understood. Note that a streaming version of the ASR model may be run while the user is still speaking, and the prediction may be displayed on-screen so the user gets feedback on what the system thinks the person is saying. 

There are alternative ways of interacting with a Voice Assistant. Instead of using a speech-based invocation mechanism on a phone or tablet, you may hold down a button on the side of the device (``Hold to Speak'' on iOS) or squeeze the side of the phone (some Android devices). 
VAs can also be invoked using accessibility features such as Accessibility Menu on Android or Assistive Touch on iOS.
Instead of speaking, a user can type in a command using a keyboard using features such as ``Type with Alexa'' or ``Type to Siri''. This bypasses the ASR component and may directly process the input text through NLU. 



% This model may take multiple cues such as how much silence has elapsed since the last word, what was the last word that was said, and how many words have been said  to identify when someone is finished speaking. 
% Typically this is computed at a high sample rate (e.g., 100 hz)
Endpointers are optimized to balance the trade-off between cutting someone off too early and having a long delay after their speech, and rely on cues such as how much silence has elapsed since the last word. These are largely optimized using data from people who do not stutter and tuned to respond to the user as quickly as possible. It is very common for the endpointer model to cut PWS off before they are done speaking especially during blocks, where there may be a long pause or gasp, or even partial word repetitions, where the vocalization may be indecipherable. 

% https://www.forbes.com/sites/stevenaquino/2021/10/05/exclusive-amazon-adds-new-speech-setting-to-alexa-app-to-help-stutterers-finish-commands-queries/?sh=3380f1542b34
% This Alexa news may serve as a support for being cutoff.

ASR models are less certain on dysfluent speech with sound, syllable, or partial word repetitions and wrongfully detect words that are whole word repetitions and interjections, even if the user does not intend to say them.
%\note{pg: I think here we need a better explanation: Acoustics attempt to be faithful to the sound, so what you said is right, but also suffer when the sounds are not complete words. Language models on the other hand try to use predictability, which makes repetitions unlikely so they tend to substitute with more likely/similarly sounding words...}
For a VA, it may be inconsequential if someone stutters on unimportant words, but is fluent for important ones. The NLU may implicitly identify which words are important or use additional context to route a transcription with dysfluencies to the correct task. 
% For non-consequential words NLU models may 
% Word or phrase repetitions may not be problematic because of the fuzzy match, and errors on less important 
% Because of this fuzzy match, repetitions may not be very problematic. , however substitutions. 
%\note{pg:Above paragraph is confusing as to the point is trying to make, and doesn't make it accurately}

% \textbf{Dictation Systems}
\textbf{Dictation Systems} provide an alternative to using a keyboard to enter text and take a user's speech and convert to text for any use, such as composing messages, notes, or emails. 
% \note{pg: this sentence is unnecessary} 
%A common use case it to create a text with your voice while in a car. 
% To contrast with Voice Assistants, 
Dictation typically does not rely on a wake word; the user may initiate manually with a button click. 
Similarly, there is often no endpointer, as the user may push a button once they finish talking and users are often dictating multiple sentences at a time. 
While VAs and DS may rely on the same ASR system, a VAs model may be biased towards a smaller set of assistant commands, whereas the DS may be biased towards free speech from arbitrary topics. 
Dictation may have additional models for \textit{punctuation} and \textit{revisions}. The former attempts to add grammatical structure to spoken words, like adding commas and periods, and may do so using a combinations of linguistic and prosodic cues (i.e., pausing between sentences).
% (i.e., via a language model) or cues from prosody in the speech . 
A revision model may identify words or phrases for which the ASR has low confidence, highlight them for the user on-screen, and offer suggestions for replacement. 
In contrast, VAs may rely on speech communication to confirm requests in cases of uncertainty, either due to low recognition confidence (did user say ``set'' or ``said'') or conceptual ambiguity (e.g., is the alarm request for a.m. or p.m.?).
% Invocation of this system varies based on usage: in a text message or notes app you may click on a microphone button to initiate or in a car you may initiate a text with a VA query which then prompts the user for the body of the text. 
% In the car scenario there may be an endpointing model, but in many other situations the users presses a button once they are done composing a message. 
% A real-time/streaming version of an ASR model is often used, especially for long-form text entry like in notes or email, so the user sees what is being written as they speak. 

% Often the ASR transcription is used verbatim, but an additional \textit{revision} models may be used to overlay potential errors within the text. For example, words that have low ASR confidence may be underlined, and if you click on-screen, there are options to swap out the word with other options. These revisions systems may also include grammar checkers. 

% \textbf{Implications of Dysfluencies.}
% \todo{consider integrating this subsection into the previous section and maybe Section 4 (ASR)}
% \hfill\\
% Endpointer “model-feature-list": "num-trailing-sil,end-of-sentence,num-of-words,pause-counts,silence-posterior",
% https://compass.scv.apple.com/confluence/display/SiriPerception/Endpoint+Feature
% \textit{Endpointer}: 
% \note{mention implications on invocation and punctuations models?}

% For an overview


% \note{move} The definitive ASR evaluation metric is Word Error Rate (WER). In some papers on stuttering, there are separate metrics for intended speech and articulated speech and correspondingly metrics iWER and aWER. 
% Intended speech has all dysfluencies removed and articulated speech retains all spoken words included repetitions.  
% For PWS, partial-word repetitions and blocks tend to cause word substitutions and increase both iWER and aWER. 
% Word and phrase repetitions increase iWER but not aWER.
% Errors in the acoustic model may be caused by blocks, sound repetitions, or partial words. 
% Errors in the language model may be caused by repetitions. 
% And if the number of candidates in the Beam Search decoder is too small it may not have enough memory to smooth over partial word repetitions. 

% For Voice Assistants, an \textit{NLU} model routes a transcription to the correct VA command. 
% For example ``What what is the weather?'' and ``What is the weather?'' would map to the same ``weather'' action. 
% This can mask transcription errors in the ASR by doing selective word finding.
% In this work we look at the use of intents~\cite{GoogleConversationalAI} where an intent may be a slotted command like ``Search for the weather in [city] on [date]'' where ``[city]'' and ``[date]'' are filled in by the user. 
% We compute results for intent recognition using the ML-based NLU system described in~\cite{chen2019active}.
% These are used as an upper bound on final accuracy or ``usefulness'' of a VA system. 


% A commercial Natural Language Understanding \textit{(NLU)} model may route ASR predictions to Voice Assistant commands using \textit{domains}, \textit{intents}, and \textit{actions}~\cite{chen2019active}. A domain may be a category of commands such as ``weather'' or ``timers.'' 
% The action would be responding to the user with the weather on that day and in that city. 
% There may be multiple different phrases that can lead to the same intent and action. 
% Typically, there is a machine learning model that attempt to identify the domain and parameter inputs. This model may also use outside information, like contacts on your phone or your GPS location to determine the most likely response. 
% In traditional NLU models, the system must simply identify critical words
% , but there is more flexibility than in Dictation. 
% For example, there is often a fuzzy search which improves performance on proper nouns., \eg ``New New York City'' translates to ``New York City.'' 
% In addition, repetitions or inaccurate prediction of unimportant words may be skipped by the model and result in the same intent, such as ``what is the weather'' and ``what in is what is the weather.``
% \todo{turn google link into citation. do they have a paper describing?} \url{https://developers.google.com/assistant/conversational/overview}.
% Word or phrase repetitions may not be problematic because of the fuzzy match, and errors on less important 
% Because of this fuzzy match, repetitions may not be very problematic. , however substitutions. 

% \todo{revision model?}
% \todo{Should we mention other models like speaker recognition or Personalized HS?}

% \subsubsection{Impact of Stuttering Events on Speech Systems}



% [issues: repetitions and LM; partial word reps and beam search; sound reps and prolongations with AM; blocks and endpointing, etc.]





% ---------------------------------------------------------------
% \subsection{Related Work}

% \subsection{Technical Literature \note{integrate with Speech Tech section?}}

% \todo{THIS SECTION IS COPIED FROM MATERIAL IN OUR PREVIOUS PAPERS; COLIN WILL CLEAN UP/CONDENSE/ETC}

% Technical work on improving speech assistants for PWS has focused on ASR models~\cite{shonibare2022enhancing,Mendelev2020,gondala2021error,mitra21,Tripathi2018,Tripathi2020,HeemanInterSpeech16}, stuttering detection~\cite{LeaStutterDetection2021}, dysfluency detection or classification~\cite{lea2021sep,kourkounakis2020detecting,Mahesha2016,DasNSRE2020,riad2020identification}, clinical assessment~\cite{BayerlTSD2020}, and dataset development~\cite{FluencyBank,UCLASS,lea2021sep,KSoF}.

% Much of this work has centered on dysfluency detection either as a standalone task or as part of an ASR system. 
% Shonibare \etal \cite{shonibare2022enhancing} and Mendelev \etal  \cite{Mendelev2020} incorporate dysfluency detectors as part of training end-to-end RNN-T ASR models. Shonibare \etal introduces a detect-then-pass approach where audio frames with detected dysfluencies are ignored entirely by the RNN-T decoder. 
% Examples in the paper demonstrate how this can be used to ignore some partial-word repetitions and blocks.
% % The temporal context is very short (100 ms) so it is unlikely to generalize to whole word or phrase repetitions or to inaudible blocks mid-word. 
% Mitra \etal \cite{mitra2021} takes a production-oriented approach that can be applied on top of a pre-trained ASR model. 
% % It is challenging to get large amounts of stuttered speech data and moreover dysfluency detection labels, so investigated 
% % optimizing a small set of ASR decoder parameters on stuttered speech, such that the system is biases towards more common phrases and shorter phrases without repetitions.
% They show that for Voice Assistant task you can optimize a small set of ASR decoder parameters on stuttered speech, such that the system is biased towards more common phrases and shorter phrases that remove sound and partial-word repetitions. 
% % and Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly}
% Alharbi \etal \cite{AlharbiWOCCI17,alharbi2018lightly} focused on stuttered speech from kids that incorporates the structure of repetitions and other dyfluencies into an augmented language model that is better at including dysfluencies in a transcription. 
% % \note{[mention Mendelev which just trained an RNN-T model with a tiny amount of stuttered speech and tries replacing partial-word annotations with another symbol. ] [Neither paper uses absolute WER! only relative. ]} 
% Efforts from Project Euphonia~\cite{projecteuphonia}, the largest atypical speech project to date, have included data from people who stutter but it has not been a core focus in publications. 
% % There has been significant interest 
% % [Project Euphonia has stuttering data as well but I can't remember seeing anything stuttering-specific that they've worked on.]

% \todo{sort these}
% * "Systematic review ... detecting developmental stuttering." \cite{barrett2022systematic}. 
% * Machine learning for stuttering identification: Review \cite{sheikh2021machine}
% * Stuttering detection: Introducing ECAPA-TDNN and Wav2Vec2. 0 embeddings to stuttering detection. arXiv'22
% * “Identification of primary and collateral tracks in stuttered speech,” \cite{riad2020identification}
% * Automatic recognition of children’s read speech for stuttering application,” vol. WOCCI, 2017. \cite{AlharbiWOCCI17}
% * Intelligent processing of stuttered speech \cite{Czyzewski2003}
% * A lightly supervised approach \cite{alharbi2018lightly, AlharbiWOCCI17} 

% Stuttering Challenge (2022): \cite{schuller2022acm} uses the KSoF dataset. 

% KSoF: The Kassel State of Fluency Dataset--A Therapy Centered Dataset of Stuttering
% * " the ability to detect stuttering events and modifications in speech could help PWSs and speech pathologists to track the level of fluency"
% * " 5500 clips of PWSs. The clips were labeled with six stuttering-related event types: blocks, prolongations, sound repetitions, word repetitions, interjections, and – specific to therapy – speech modifications."



% Prolongations, or extended sounds, have been detected using short-window autocorrelations [16] and low-level acoustic models [10]. Word/phrase repetitions, if they are well articulated, are easily detected using LM- based approaches [19], with the caveat that single-syllable words such as in the phrase “I-I-I am” will often be smoothed into “I am” due to the underlying acoustic model and phrases like “I am [am]” may be pruned because the LM has never seen the word “am” repeated before. This is fine for speech recognition but bad for stuttering event analysis. Arjun et al. [16] addressed this repetition problem by segment- ing pairs of subsequent words and analyzing correlations in their spectral features. Interjections, including “um”, “uh”, “you know” and other filler words, are perhaps the easiest type to recognize with a language model if well articulated. Blocks, or gasps/pauses typically within or between words, are difficult to detect because the gasp for breath or pause is often inaudible. Sound repetitions are also challenging because syllables may vary in duration, count, style, and articulation (e.g.,“[moh-muh-mm]-ommy”).
% Efforts in HCI have sought out an understanding of speech recognition needs for users with speech impairments, which is critical for framing problems like ours [1, 2, 22].





==> sections/3b-survey-findings-old.tex <==

\paragraph{Usage and utility}
Most participants were familiar with dictation (90.2\%, n=55) and many had used it before (73.8\%, n=45). For 45 who had, a total of 26 reported regular use of at least monthly: `at least daily' (17.8\%; n=8 of 45), `at least weekly' (21.3\%; n=13), and `at least monthly' (11.1\%; n=5). These numbers are lower than for VA use, where 40 of the 61 participants reported regular use. Most people with experience using dictation had used it on the phone (88.9\%, n=40 of 45), while 24.4\% (n=11) had used it on the watch and 20.0\% (n=9) had used it in the car. Other less frequent platforms included traditional computers, tablets, and smart speakers. Common tasks included writing text messages (95.5\%, n=42), taking notes (37.8\%, n=17), writing email (18.0\%, n=11), and dictation within a web browser (16.4\%, n=10).
 
%Figure \ref{fig:usage_frequency_by_category_dictation} shows dictation usage by rated A\&H severity.  Respondents who reported that they have not heard of dictation (n=14) or did not know how how often they used dictation (n=2) were not included in the analysis.  Respondents with severe stutters had the highest proportion of users who reported they 'Never' used voice assistants, though respondents with severe stutters also had the highest proportion of daily users.
% For the 10 participants who were familiar with dictation but had not tried it, their reasons were split between concern about how well their speech would be recognized and not seeing value in dictation in general.

Most participants found dictation to be at least somewhat useful: `extremely useful' (8.9\%; n=4), `very useful' (31.1\%; n=14), and `somewhat useful' (37.8\%; n=17). The most common reasons people found it useful were for sending messages while driving, and general efficiency and ease. 
For people who reported that dictation is `not very useful' (20.0\%, n=9) or `not at all useful' (2.2\%,  n=1), the most common reasons were that it is inaccurate for their speech or inefficient compared to typing, due to having to fix errors. 
% \todo{need to decide if keeping this quote or the later similar one from this person}
As [P2-77], who did not find dictation to be useful at all, said, \textit{``because as a person who stutters I use fillers like umm, so, use a lot of repetitions, and also have frequent blocks and when I use dictation it writes down all my disfluencies that when I read the text it makes no sense.''} 
For other participants, the utility of dictation depended on the words and length of the task, as reflected by [P1-60]: \textit{``When I am using words I can say well it works good, when I have to use words that I am unable to say clearly it does not work at all.''}



% \subsubsection{Participant Background}
% These can be caused by the setting or environment, current mood/stress level, communication partners, or other variables can impact stuttering.  
% PWS vary in terms of how many and what types of dysfluencies they produce. 

% These assessments were performed 
% to ensure adequate severity distribution. The target was at least 30 from each group
% 12, 31, 18 = 61 (80% mod/severe)
% \todo{find target or final severity distribution for survey}

% Demographics were as follows. 
% There was a roughly even gender split between men (50.8\%, n=31) and women (49.2\%, n=30), with no participants reporting another gender. Most participants were under 40 years old: aged 18-19 (n=2), 20-29 (n=28), 30-39 (n=21), 40-49 (n=3), 50-59 (n=4), 60-69 (n=2), and 70-79 (n=1). Individuals identified as white (n=38), black or African American (n=12), Hispanic (n=5), Asian (n=2), American Indian or Alaska Native (n=1), or preferred not to answer (n=3).

% While we used the A\&H scale for recruitment, we wanted to better understand potential correlations with other speech patterns. For A\&H, 12 were rated as having a mild stutter, 31 as moderate, and 18 as severe. 
% When asked about whether people understood their speech, almost all participants (93.4\%, n=57) reported that friends and close contacts `always' or 'usually' understand their speech, however this was lower for acquaintances (73.8\%, n=45) and strangers (67.2\%, n=41). 
% Many individuals noted that their speech qualities change day-to-day (65.5\%, n=40) or throughout the day (55.7\%, n=34) and on top of typical dysfluencies such blocks, prolongations, and repetitions, their voice may be strained (42.6\%, n=26) or breathy (16.4\%, n=10). 
% Most individuals noted that speaking requires `some' physical effort (67.2\%, n=41) with fewer responses of `very high` (11.4\%, n=7) or `very low` (9.8\%, n=6).



% Survey (61): Counter({1: 12, 2: 31, 3: 18}) 1=mild, 2=mod, 3=severe
% Phase 1: (50): Counter({1: 25, 2: 18, 3: 7})
% Phase 2 (41): Counter({1: 2, 2: 12, 3: 27})
% Intersection of (S, P1, P2) (99): Counter({1: 25, 2: 48, 3: 26})
% Intersection of (P1, P2) (99): Counter({1: 25, 2: 44, 3: 22})


%%Note: explanation for the figure above.  This is mildly interesting, but the main points related to severity and accuracy may already be well covered elsewhere so maybe unnecessary...
% the number of surveyed participants who use voice assistants regularly (at least monthly or more frequently)
% \note{given small sample sizes is the following statistically significant? if not, maybe we should omit?}
% Figure \ref{fig:usage_frequency_by_category} shows the number of surveyed participants who use voice assistants regularly (at least monthly or more frequently) by  gender, age, A\&H severity, physical effort of speaking, and self-reported voice assistant accuracy. 
% Among the surveyed participants, men used voice assistants regularly at a proportionally higher rate than women, people with mild stutters used voice assistants more regularly at a proportionally higher rate than people with moderate and severe stutters, and people who reported that voice assistants rarely understood their speech used voice assistants at a proportionally lower rate than those who reported that voice assistants sometimes or often understood their speech.  
% Most participants surveyed reported that they were between 20-29 years old or 30-39 years old and that speaking required 'some effort'. 

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.6 \paperwidth]{figures/stacked_bar_usage_frequency_proportion.png}
%     \caption{Voice assistant usage frequency by A \& H severity and self-reported voice assistant accuracy.   Respondents who said that they didn't know how often they used a voice assistant (n=2) were not included in this analysis.  Respondents with severe stutters had the highest proportion of people who reported never using voice assistants, but also had the highest proportion of daily users.  Usage frequency was generally highest for those who reported that voice assistants often understood their speech accurately and lowest for those who reported that voice assistants rarely understood their speech accurately. 
%     %\todo{Can we add more ticks?} added additional ticks
%     }
%     \label{fig:usage_frequency_by_category}
% \end{figure}
% %\begin{figure}[t!]
% %    \centering
% %    \includegraphics[width=0.4 \paperwidth]{figures/stacked_bar_dictation_usage_frequency_proportion.png}
% %    \caption{Dictation usage frequency by A\&H severity, by participants who reported they are familiar with dictation technology.  Respondents with severe stutters had the highest proportion of users who reported they 'Never' used voice assistants.
% %    }
%     \label{fig:usage_frequency_by_category_dictation}
% %\end{figure}


% In terms of technology use, all participants owned smartphones, with most having an iPhone (93.4\%, n=57) and four having an Android phone. 
% Over half (59.0\%, n=36) had smart speakers in the home: 27 had an Amazon device, 5 had a Google device, and 4 had an Apple device. For other technology, 58 participants reported having a computer, 35 had a tablet, and 27 had a smartwatch or fitness tracker.


% \note{how did we analyze the open-ended responses. If we do any statistical analysis we can describe that here.}

% to do: add participant breakdown by age, gender, race?


% \subsection{Participant Recruitment}
% Participants were recruited through social media, referrals from speech language pathology clinics, and word of mouth. Individuals self-identified as having a stutter. An SLP also screened the individuals by listening to their connected speech and by observing overt stuttering characteristics.\note{Colin mentioned there were 4 tasks the vendor's SLP used to screen and grade a participant)}
% The participants who presented as people who stutter were included and graded using A&H Scale into mild, moderate, and severe stuttering groups to ensure adequate severity distribution. In total \note{66} people filled out the survey and \note{92}  contributed audio recordings. 
% % \note{technically 100 people for audio, but we don't have annotations for 8}.
% % \todo{how do we want to discuss Phase 1 and Phase 2? should they be merged entirely? there are some protocol changes like the connected speech sample}
% Of these individuals, [X] were rated as mild (0-5\% of words have dysfluencies), [X] mild (6-20\% dysfluencies), and [X] severe ($\geq$20\% dysfluencies) using the A&H scale. 

% --------------------------------------------
% \subsection{Overview, severities, characteristics, etc. }

% \todo{These sections are copied from our Quip summary; modify as makes sense...}

% \todo{?How do we want to show numbers? Should we include a table (or set of tables?)}


% --------------------------------------------

\subsubsection{Voice Assistants} \label{subsec:VAs}
All participants were familiar with voice assistants and almost all (96.7\%; n=59) had used one. 
Most of this experience was on phones (83.6\%; n=51) and smart speakers (45.9\%; n=28), while smartwatches and car infotainment systems were also relatively common (both 24.5\%; n=15); 10 or fewer participants had used voice assistants on tablets or traditional computers.
% Here, we report on usage patterns compared to the general population as well as \todo{whatever we report on}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4 \paperwidth]{figures/bar_va_usage_frequency_comparison.png}
    \caption{Voice assistant usage by the general population and by stuttering survey respondents.  Bars show 95\% confidence intervals of calculated proportion calculated using Clopper-Pearson "exact" method.  Raw data was not available to calculate confidence intervals for general population data \cite{npr_smart_audio}}
    \label{fig:utilization_comparison}
\end{figure}

\paragraph{Usage \& Utility}
% %relative to general population}
% %% Comparison to survey of general population (may be too long for how hard this is to interpret %%
Among voice-assistant users, reported usage frequencies were lower than estimates for the general population (Figure \ref{fig:utilization_comparison}).  Particularly, the proportion of daily users among PWS voice assistant users was significantly less than in the general population. 
From a survey- and interview-based study, National Public Media \cite{npr_smart_audio} estimated that, from among 62\% of voice-operated assistant users in America, 57\% use a voice-operated assistant at least daily, 23\% at least weekly, and 20\% at least monthly. From our stuttering survey respondents, among the 86.8\% (n=53) of voice assistant users (respondents who reported any frequency of voice assistant usage), 35.6\% use a voice assistant at least daily (n=19), 22.7\% at least weekly (n=12), and 17.0 (n= \% at least monthly (n=9).  

Respondents interested in voice technology may have been more likely to complete than the survey than those not interested in our technology, which may have biased some of our usage metrics - as reflected in the high proportion of voice-operated assistant users among our respondents compared to the general population.  Comparison of use frequency among voice assistant users only, as reported in Fig. \ref{fig:utilization_comparison}, is more valid than comparing overall usage percentages, as the base for both datasets are respondents who use voice technology only.  Respondents who used voice technology most often reported daily usage, among both the general population and PWS, suggesting that voice assistant users are more likely to use the technology frequently than sparingly irrespective of whether they stutter.


% Among our stuttering survey respondents, 65.6\% (n=40 of 61) reporting using a VA regularly (monthly or more frequently) and of those 47.5\% use daily (n=19, 31.1\% of all), 30.0\% use weekly (n=12, 19.7\% of all) and 20.0\% use monthly (n=9, 14.8\% of all). 
% Results suggest that the proportion of respondents who reported using a VA regularly may be related to stuttering severity (Figure \ref{fig:utilization_comparison_severity}), with users with mild stutters having usage rates similar to the general population. However, these results are not statistically significant due to the small number of participants in each severity group. 

\todo{proposed new points to make?:}
\begin{itemize}
    \item  report similar proportions of usage (i.e. majority are daily users, decreasing proportions as usage frequency decreases) compared to NPM study. Not enough samples to have statistical significance to determine whether usage is generally lower for PWS (added in a sentence describing this).
    \item Usage is correlated with self-reported understanding (for both VA and dictation systems
    \item  reported SR systems' understanding compared to understanding with family, acquaintances, strangers; larger proportion of understanding is seen with VAs (evidence of an area of improvement?) see Figure \ref{fig:understanding_comparison}

\end{itemize}

Figure \ref{fig:usage_frequency_by_category} shows usage breakdowns by  A\&H severity, and self-reported voice assistant accuracy.\footnote{Two respondents reported that voice assistants 'always' understood their speech.  For the presented analyses, this response was included in the 'Often' category.  No respondents reported that voice assistants 'never' understood their speech.} 

VA and DS usage appears to increase when users perceive themselves as being better understood by speech technology. 
We found this correlation to be statistically significant by Kendall Tau between VA usage and self-reported VA understanding (\textit{$r_{\tau}$}=0.45, \textit{p}<0.001) where VA usage is discretized into daily, weekly, monthly, more than monthly usage and never, and VA understanding is discretized into always/often, usually/sometimes, rarely/never. Similarly, DS usage and self-reported VA understanding had lower correlations(\textit{$r_{\tau}$}=0.17, \textit{p}=0.11). 

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4 \paperwidth]{figures/Understanding_proportions.png}
    \caption{Proportions of self-reported understanding by VAs, family, acquaintances, and strangers ($n$=59, $n$=57, $n$=57, $n$=56)\todo{double-check survey responses on why is N different}.}
    \label{fig:understanding_comparison}
\end{figure}


% \paragraph{Utility}
We distinguished usage with usefulness, as perhaps individuals do not use VAs frequently but when they do they find them highly valuable. 
A majority of participants (70.5\%) found VAs to be at least somewhat useful and many 27.3\% found it very or extremely useful: `extremely' (9.8\%; n=6), `very' (27.9\%; n=17), and `somewhat' (32.8\%; n=20). These roughly mirror usage patterns.

%% People who use voice assistants
Amongst regular users (n=40), n=16 described specific use cases that positively influenced their perception, including playing music/radio (n=8), retrieving information (n=5), controlling smart home devices like lights and temperature (n=3), and n=2 each for setting a timer, setting reminders, sending messages, settings alarms, and navigation.
Fourteen of these regular users highlighted the speed of voice assistants (n=6), that voice assistants can be used hands-free when driving (n=6), from across the room (n=1) or without a screen (n=1) and that they can be better than typing (n=6). 
% Participants who were more positive (extremely or very) commonly described the utility of common VA tasks such as listening to music or setting timers, while driving, and hands-free use. 

% described user experience factors that influenced their utility rating, including the speed of voice assistants (n=6), that voice assistants can be used hands-free (n=7) - as in when driving (n=6), from across the room (n=1) or without a screen (n=1) - and that voice assistants can be better than typing (n=6). 
% One regular user said that privacy concerns prevented them from using voice assistants more frequently. 
% Among regular voice assistant users, n=5 respondents reported that poor accuracy of voice assistants influenced their utility rating. 
% One respondent described feeling frustrated by being misunderstood when using a voice assistant.

In contrast, for participants who found VAs to be `not very' (16.4\%, n=10) or `not at all' (13.1\%, n=8) useful, reasons were split between participants who saw no inherent value in VAs (e.g., \textit{``I haven't felt a need for them in my life''} [P2-51]) and those who encountered accessibility challenges due to stuttering. 
For n=10 participants who did not use a VA regularly, they described challenges with poor recognition performance, that it takes longer to speak than type, or noted that they were simply not interested. 
% For example, [P2-64] wrote, \textit{``Voice assistants are not at all useful for me because I often have to repeat myself so many times for it to understand me that it’s quicker and easier for me to just use my hands and search or type what I want the assistant to do''}, while [P1-63] wrote, \textit{``It takes longer for me to speak/stutter [by] using voice assistants than it would for me to type what I need.''}
For example, [P2-64] wrote, \textit{``Voice assistants are not at all useful for me because I often have to repeat myself so many times for it to understand me that it’s quicker and easier for me to just use my hands [...]''}, and [P1-63] wrote, \textit{``It takes longer for me to speak/stutter [by] using voice assistants than it would for me to type what I need.''}
%%People who don't use voice assistants
% n=4 participants described user experience considerations that influenced how useful they found voice assistants.  
% One respondent said hands-free voice assistant usage while driving as a useful facet of voice assistants, one participant said voice assistants allow them to ask questions quickly, one participant said that voice assistants take longer than typing, and one participant said that speaking to voice assistants actually helps them pace their speech.  
% Of those respondents who do not use a voice assistant, n=10 said that their utility rating was influenced by poor accuracy of voice assistants.  
One respondent said that being misunderstood by voice assistants discouraged them from wanting to speak aloud. 
% Three respondents reported that they were not interested in voice recognition technology.

\paragraph{Overall challenges}
We asked about what factors prevented participants from using VAs more often. The most common were `voice assistants cut off my speech before I'm done talking' (59.0\%, n=36) and `voice assistants don't understand my speech well enough' (55.7\%, n=34). 
Other concerns, however, were not purely technical. 
Twenty-two participants (36.1\%) reported not wanting other people to hear them talking to the VA, reflecting a social consideration that past work has also identified~\cite{bleakley2022exploring}. 
As well, many participants (21.3\%, n=13) cited that it takes `too much physical effort for me to speak'. 
Only six participants (9.8\%) responded that `voice assistants don't seem useful'. 

\paragraph{Speech recognition accuracy and errors} \todo{add section similar to what's in dictation?}
\note{this is out of context... e.g. WER on what data? }
\todo{move to ASR section where we talk about similar things} 

The types of dysfluencies, frequency and severity may impact the performance of speech recognition systems (Section \ref{sec: clinical-component}), how comfortable users feel using them, and ultimately usage.

% \todo{Can we state somewhere that we only include correlations with $p<0.5$ instead of including everywhere? or is that insufficient?)
% There may be differences in satisfaction with voice assistants and usage practices between users with stuttered speech and the general population that are not reflected in use frequency metrics. 


% %Note: Redundant with Fig 3? 
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.4 \paperwidth]{figures/bar_va_usage_frequency_by_severity.png}
%     \caption{Voice assistant usage by stuttering survey respondents.  The proportion of u %by the general population (from \cite{npr_smart_audio}) and by stuttering survey respondents.  Bars show 95\% confidence intervals calculated using Clopper-Pearson "exact" method
%     }
%     \label{fig:utilization_comparison_severity}
% \end{figure}





% About half of people surveyed use a voice assistant on a daily or weekly basis. Two-thirds find it at least somewhat useful, especially when driving or when their hands are occupied but only about half says it works often or always. The rest either aren’t interested in this technology or recognition performance is too low to use. Interestingly, some people that are moderate-to-severe stutterers according to our data collection are regular users; stuttering can be very situational and some individuals report interest in Voice Assistants when they are alone and don’t stutter but not in public where stuttering is more likely. 

%\paragraph{Utility and Challenges}
%In general, most people surveyed are interested in speech technology, but are aware of its limitations. The perception of underlying features is in-line with expectations: people are regularly cut off, their words are miss-construed, and they are required to repeat themselves multiple times. 



\paragraph{Invocation}
Most VAs use a wake word to start the system like ``Alexa'' or ``OK Google''. Almost half of participants reported that these wake words `always' (11.5\%, n=7) or `often' (36.1\%, n=22) worked for them. 
Problematically, 17 participants (27.9\%) reported wake words only working `sometimes' and 8 participants reported `rarely' or `never' (13.1\%); the remaining participants had not used a wake word. 
While we did not ask participants to elaborate on their use of wake words, a handful of responses to other open-ended questions referred to challenges with wake words, including: \textit{``Problem with wake words is my biggest frustration. I would want to change it to something I can say easily''} [P2-1] and \textit{``It's [Hold/Squeeze to Speak is] useful on my phone to bypass the lag that occurs when [the VA] does not recognize me using the wake phrase''} [P1-28]. 
A potential solution is to allow users to change the wake word. Alexa has at least five options, Google Assistant has two, and Siri has one.

% TODO: Leah: I commented this out but maybe we should keep it somewhere? -- Very few people (5 of 55) know about Type to Siri and two of those people didn’t find it valuable. 

\paragraph{Endpointer and alternatives}
Being cut off by the VA was a common challenge reported in Bleakley et al.'s~\cite{bleakley2022exploring} interviews with 11 PWS. Our data demonstrates the pervasiveness of this problem: almost half of participants stated that VAs cut them off `always' (3.3\%, n=2) or `often' (37.7\%, n=23), while an additional 31 participants (50.1\%) reported being cut off `sometimes' or `rarely'. For the 57 participants who had at least some experience being cut off, when asked if they knew why they had been cut off, by far the most common explanation was that there was a pause or block in their speech and the system thought they had finished speaking (77.2\%, n=44 of 57). 
% For example, participants wrote: \textit{``[The VA cuts me off] Because I have a break in speaking due to stuttering''} [P2-49] and 
% \textit{``They cut me off because they don't realize I'm blocking''} [P2-29]. 
Being cut off could also have follow-on impacts, as [P2-42] described: \textit{``The [smart speaker] which I use most often does not like any hesitations in speech. It assumes the slightest pause means the person is done speaking. So I get cut off often. It creates a sense of having to rush which makes my speech worse.''}
We address endpointing errors in Section~\ref{sec: endpointer} and significantly reduce the problem for all study participants.
\note{moved from related work} Some people stutter frequently when in a group but not when on their own \cite{tichenor2021variability} or when in front of a smart device because of ``pressure to perform'' as we describe in Section~\ref{sec:survey_results}.


Android and iOS offer an alternative to automatic endpointing on smartphones, where you can push down a button (physical or virtual) while speaking and only release it when done, although this is not available on screen-free devices like smart speakers. Twenty-seven participants (44.3\%) reported using a device that supports this functionality. Of those 27, almost all found being able to press a button and speak to be useful: 51.9\% (n=14 of 27) `extremely useful', 18.5\% (n=5) `very useful', and 29.6\% (n=8) 'useful'. Reasons provided for this utility were most commonly that it eliminates being cut off, but some participants also explicitly referred to feeling less rushed or worried, such as: \textit{``I can fully get my phrase in without worrying about blocking''} [P1-62] and \textit{``I don't feel rushed to finish what I need to say''} [P1-45]. A few participants mentioned that pressing a button to talk also eliminated issues with wake words, such as [P1-73], \textit{``Because it knows when to start listening and when I'm done.''}

%(62.2\%, n=38) state that VAs sometimes, often, or always cut them off due to blocks or other dysfluencies. 

% \paragraph{Revisions} 
\paragraph{Failure mitigation} 
When VAs fail, one strategy used with mixed success by participants is to revise or restate the command. Many participants (36.1\%, n=22) reported `often' or `always' revising what they say due to inaccuracies in speech recognition. 
Of 33 people who reported on how often revision is effective, only 42.4\% (n=14 of 33) said `always' or `often', while an additional 45.5\% (n=15 of 33) said `sometimes'.  

%In order to get around endpointing issues some people use Hold to Speak. Half of the participants that use Siri at least weekly (14 of 27) have used Hold to Speak and generally have a positive impression. Users who do not find it useful say that their speech isn’t recognized even when holding down the button, likely due to word insertions errors associated with blocks or incorrect words sometimes due to partial-word repetitions. 

% [ASR/Intents]
% at least sometimes, (2) incorrect words due to partial word repetitions impacts a large percentage, and (3) in more open-ended voice queries (perhaps creating a reminder) people report word repetitions. Although, the latter is a larger problem for Dictation. 


% [?NLU?]

\paragraph{Improved Recognition} \note{move to challenges?} If speech recognition worked better for these individuals then they would be more likely to use Voice Assistants (at all or more frequently). When asked what would make them use VA’s more, responses were generally as expected: improve support for understanding or accommodating stuttered speech patterns (i.e., endpointing and general ASR). A few people are either not interested in VAs at all, expressed reluctance because of difficulty of speaking, or have other general technology-related concerns such as privacy. 

\paragraph{Non-technical}
% \subsubsection{Non-technical} 
% \note{Leah: I wonder if we can move this as an overarching theme to come in its own section after Dictation} 
There are social and psychological concerns for PWS that may not be as common in the general population.
% Errors from ASR systems may evoke an emotion in PWS that may be less prevalent in the general population. 
Multiple people note that being misunderstood can be stressful or induce negative emotion. For example: 
% one person it gives them the sense that they are inferior because Voice Assistants work for ``everyone else.'' 
    [P2-77] \textit{``I want it to be inclusive to all individuals who stutter, stammer clutter [...] we should be able to feel confident speaking in any devices and not feel inferior because [...] it was made for the population that doesn't have a speech impediment.''}, [P2-36] \textit{``It works for everyone but me. Even though I have virtually no interest in using them, it sucks that the option isn't even available to me.''}, and [P2-8] \textit{``The forcing of the technology on those that cannot navigate due to speech issues.''}
    % [P2-77] \textit{``I want it to be inclusive to all individuals who stutter, stammer clutter anyone with a speech impediment because we should be able to feel confident speaking in any devices and not feel inferior because our own voice assistant devices is not able to understand us because it was made for the population that doesn't have a speech impediment.''}
There is a related social component that extends beyond people’s general insecurities with using Voice Assistants in public. Many individuals who stutter don’t want other people to hear them stutter while talking into their device. From a practical standpoint, due to endpointing issues, there is pressure to say something without a pause or block, which in turn stresses people out, and makes them more likely to stutter.


\note{moved from related work} 
Over time, a PWS may also experience negative psychological outcomes such as social anxiety, low self-esteem, and negative feelings about communication~\cite{boyle2015identifying}. In Section \ref{sec:survey_results} we find that this extends to an emotional impact when VAs fail to recognize one's speech. 
This can be a cycle as increased anxiety may then lead to an increase in producing stutter events.  




% --------------------------------------------
\subsubsection{Dictation Systems}




\paragraph{Overall challenges} 
Of the 55 participants familiar with dictation, when asked what reasons prevent them from using dictation more often, the most common, cited by 31 participants (56.4\% of 55) was `dictation tools don't understand my speech well enough'. This response emphasizes the importance of speech recognition improvements for making dictation accessible to PWS. As with VAs, participants also commonly cited non-technical reasons for not using dictation more, most notably the physical effort it takes to speak (32.7\%, n=18) and not wanting other people to hear them dictate to the device (30.1\%, n=17). Additionally, 11 participants (20.0\%) reported that dictation does not seem useful, and 12 (26.7\%) felt that they use more refined language when they type than when they speak.

The survey asked participants if they don't use dictation regularly, what if anything would make them start. Twenty-seven participants responded, with many references to improving recognition accuracy (e.g., ``If it were more accurate and understand my stuttering speech better'' [P2-72]). Notably, however, seven \todo{IRR??} participants effectively responded that nothing would make them use dictation regularly. 
For example, [P2-44] said, \textit{``I can't think of anything. I much prefer to type''}, while [P2-51] said, \textit{``I'm not sure. As someone who stutters, and just situationally in my life, I can't imagine dictation regularly being a more convenient option than typing.''} 
These responses highlight that even with ASR improvements, some PWS may not wish to use dictation.

\paragraph{Speech recognition accuracy and errors}

With dictation, the user's speech is transcribed verbatim, in contrast to VA systems that predict the most likely command based on a spoken phrase. This difference and focus on specific words is reflected in participants' experiences with dictation errors. 
While 35.6\% (n=16 of 45 who had used dictation) felt dictation systems recognized their speech often and 2.2\% (n=1) said `always', a majority of participants encountered difficulties. Half the participants (51.5\%, n=23) felt dictation only `sometimes' recognized their speech accurately, and the remaining five (11.1\%) felt their speech was `rarely' recognized well. 
As a result of these errors, participants frequently need to revise or restate what they say, with about half of participants `always' (6.7\%, n=3) or `often' (42.2\%, n=19) have to repeat or revise what they say, and an additional 35.6\% (n=16) did so `sometimes'. 
%However, 28 participants also commented on how effective they felt this revision was, and most  this revision is not seen as working often, \note{not sure this is interesting enough to report on}

When asked an open-ended question about what types of errors tend to occur with dictation, a majority of participants \todo{IRR?? 71.1\%, n=32} described the dictation system generally transcribing wrong words (e.g., \textit{``Message contains different words than I intended''} [P2-5]). 
Some participants \todo{IRR?? (13.3\%, n=6)} also mentioned being cut off, although this was a much less common error than with VAs because many dictation systems do not use an automatic endpointer. 
A few participants mentioned punctuation, proper nouns, and slang. 
Finally, some participants mentioned specific stuttering characteristics and challenges, including repetitions being displayed
% (\textit{``Misunderstood due to repetition or actually repeats word''} [P2-46])
, the impact of blocks 
(\textit{``words that I have a block in the middle of will turn into a strange phrase''} [P2-51]) 
, and interjections being shown, as described by [P2-77]: \textit{``because I have blocks and use filler words, the fillers are listed on the text message all my disfluencies are written down and when I read over the text it makes no sense and I have to type it myself instead because I will never be fluent all the time.''} 

\todo{Need a couple of sentences summary/takeaway}

%[ASR]
%The biggest technical limitations are general speech recognition errors such as word insertions and miss recognized words. About 50\% of people report often or always needing to revise their input. With Dictation, what you say is written out verbatim whereas with a Voice Assistant the system will often filter your speech and identify the most likely command. 
%People do report being cut off, in particular when sending text messages, but it is much less common because many forms of dictation don’t have an explicit endpointer. 
%Some individuals note that blocks and partial word repetitions can turn into long strings of nonsense words and as-expected when someone has a word repetition dysfluency the word, indeed, is written multiple times. Other mentions include references to names or proper nouns being commonly miss recognized, filler words being included in a transcript, and several people mentioned punctuation being incorrect likely due to pauses in speech. One individual noted an emotional reaction to seeing their dysfluencies written out mid-dictation. 

%In addition, there should be the ability to re-start a sentence after you have already said half of it — one strategy to overcome a block is to repeat the first half of a sentence.  


%\note{stuff below here is copy/pasted from Quip and could perhaps be just removed at this stage}

%Responses for Dictation largely mirror Voice Assistants but with issues like repetitions and word errors emphasized more than being cut off. 
%Moreover, the time that it takes to revise dictation when incorrect can be a large burden. 

 
%[Usefulness]
%Some people were not familiar with dictation or hadn’t used it but on average usage was similar to voice assistants: 46\% of people use it at least weekly. 
%There is a slight reduction in people who find Dictation useful compared to Voice Assistants but this may not be statistically significant (62\% vs 67\%). 
%Many people again find it useful while driving and 
%for those who don’t find it useful it’s because of inaccuracies in the system, inefficiencies especially when needing to revise text, social acceptability, and the amount of effort needed to speak. The most common use case was sending a text message. 
%If Dictation were more accurate, people would want to use it for note taking, writing an email, and in a web browser.


%[Revisions]
%\todo{rewrite}Apple isn’t doing anything with Dictation explicitly for PWS, but it does have a corrections system that underlines “likely incorrect” words with a squiggle. When you click on the squiggle it gives you alternative word options. This can be much faster than deleting and typing out a new word. It’s unclear how often this is useful for stuttering; nobody mentioned it in their feedback. 


%[Other]
%People in the study are interested in Dictation for the same reasons as the general public: efficiency. In theory you can transcribe what you say quicker than by typing, and you can do so hands-free and without looking at the screen. In practice, for PWS, it is common to revise what you say, which means that you may need to spend more time fixing the text than to type it from scratch. These revisions are often typed, which means you need to use your hands and look at the screen. Some of the reasons study participants aren’t interested in Dictation are similar to the general population. For example, one participant noted that the way you speak is different than the way you typically type out a text message. 




%People say they would be more likely to use dictation if the issues above were improved. Moreover, based on what tasks they currently use and which ones they’re interested in using, if performance is better they may start using Dictation in a wider variety of situations including note taking, writing an email, and in a web browser.  


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.3 \paperwidth]{figures/Frequency of VA and dictation use.png} \includegraphics[width=0.3 \paperwidth]{figures/Interest in future technology.png}
    \caption{\note{Possibility for a simple figure, but also to demonstrate what I mean by a proportional bar graph (in reference previous bar graph figure comment).}}
    \label{fig:freqUseVAandDictation}
\end{figure}


% --------------------------------------------

\subsubsection{Future Technology}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.4 \paperwidth]{figures/Interest in future technology.png}
%     \caption{\note{Possibility for showing interest in speech tech if it recognized speech accurately}}
%     \label{fig:futureInterest}
% \end{figure}

\paragraph{An Ideal Speech Recognizer}
Participants were asked to imagine speech technologies that could accurately understand all of their speech. 
Within this context, most participants were at least `somewhat` interested in VAs (86.9\%, n=53): `extremely’ (n=25)`very' (n=13) `somewhat' (n=15) `not very' (n=7), `not at all' (n=1) and similar for dictation (See Figure~\ref{fig:freqUseVAandDictation} (right)). 
% In open-ended responses explaining their interest level, 
Positive responses reflected earlier feelings about VAs and dictation, notably increasing efficiency, ease and convenience, being able to do actions hands-free (including while driving), and generally having confidence in the system. 
For example, [P1-66], who currently uses VAs at least monthly and has not tried dictation wrote, \textit{``I would be extremely interested in this, especially knowing it's something I don't have to worry about the speech input being able to understand me. It would remove my hesitancy and frustration with my stuttering from the equation.''} 
Negative and neutral sentiments indicated a preference for typing, seeing no need for speech input, and value depending on context (e.g., \textit{``It would depend on the device''} [P1-64], who uses VAs weekly and dictation less than monthly). 

Additionally, some concerns around the effort required to speak and social factors arose, mirroring earlier responses and again emphasizing that speech input may not be relevant to all users even with substantial accuracy improvements. 
For example, commenting on the effort required to speak, [P2-73] wrote, \textit{``It's a nice thought but it's still easier for a person who stutters to type most of the time. Unless our hands are filthy or tied up''}, while [P2-87] wrote, \textit{``It still requires effort to speak even if it understand me perfectly, and I am good at controlling them manually.''} 
Some participants also expressed reluctance to use even such improved speech technology in a social setting, including [P2-1], who wrote, \textit{``It is easier but I would be reluctant to use voice commands in public because of my speech impediment''}, and [P1-58], who wrote, \textit{``I still would not use it at work. I would use it in spaces where I am alone, with my spouse or family.''}

%In general people would be more interested in Siri and related technologies if they did understand stuttered speech perfectly. People noted typical benefits such as efficiency and hands-free interactions. Some people were not interested because it can be effortful to speak or they don’t want other people to hear their stutter. Interest for Dictation is a little lower than a Voice Assistant while both are positive. 

\paragraph{Adaptive Tech}
Finally, we asked participants about two potential technologies that could improve accuracy for an individual user with atypical speech. 
The first was around a personalized speech recognition system that could  recognize the participant's speech well, \textit{``but you need to spend time teaching it, perhaps by reading a set of phrases into the device.''} Of the 58 participants who responded to this scenario, most (n=47) had some interest: `extremely' (27.6\% of 58, n=16), `very' (20.7\%, n=12), or `somewhat' (32.8\%, n=19). 
These 47 participants were roughly evenly split between being willing to spend only 1-5 minutes on training and spending 10-30 minutes on training; however, 12 were willing to spend even longer. One said they were not willing to spend any time. 
For the 11 participants who were either `not very' or `not at all' interested in training a system, the most common concern was the time and effort required. 
One participant, however, noted a potential issue, \textit{``My speech changes from day to day. In the middle of a bad speech day I don’t want to talk more''} [P1-55].

The second technology imagined a VA that works very well but only supports a small set of perhaps 10 to 20 high-value commands. Of the 59 participants who responded to this question, most (n=40) felt it would be useful: `extremely' (20.3\%, n=12), `very' (23.7\%, n=14), and `somewhat' (23.7\%, n=14). 
Some participants expressed the sentiment that they do not use many commands anyway, such as, \textit{``I usually only use my [device] for the same things over and over again so this would be useful''} [P2-73]. 
However, those who did not think this approach would be `very useful' (27.1\%, n=16) or `at all useful' (5.1\%, n=3) commonly had \textit{``no need for voice assisted technology''} [P2-44] or felt that \textit{``10-20 commands is not enough''} [P1-63].

% \todo{Need a couple of sentences summary/takeaway}

%We asked about participants interest in training a personalized model that could improve speech recognition. In general people were receptive to the idea, with almost half being “very” or “extremely” interested. There was a high variance in willingness to spend time training the device, their general interest in the technology, and how effective they thought it would be. Ultimately, one concern (noted by three people) is that someone’s speech characteristics may change over the course of the day or in different contexts, which may make it challenging to build a personalized model that works all the time. 

%About half of individuals were “very” or “extremely“ interested in a minimal Voice Assistant that only allows perhaps 10 to 20 commands but works better for the individual. Many proponents note that they only use a small set of commands regularly anyway so it wouldn’t be very different. There was interest in being able to customize the specific commands that you say versus having a predefined set. Some people that are not interested already use a Voice Assistant regularly with more than 20 commands and thus would view this as a regression. Others simply aren’t interested in speech technologies. 


% \begin{quote}
%     [P2-36] \textit{``It works for everyone but me. Even though I have virtually no interest in using them, it sucks that the option isn't even available to me.''}
% \end{quote}
% \begin{quote}
%     [P2-8] \textit{``The forcing of the technology on those that cannot navigate due to speech issues.''}
% \end{quote}

% --------------------------------------------
% \subsubsection{Implications on Speech Systems}


==> sections/old-method.tex <==
% \section{Methods}
% \note{likely integrate 'Methods' with other sections'}


% Our goal is to understand the experience of speech technology on PWS, how well existing systems work subjectively and quantitatively, where they break, and areas for improvements. 
% % We analyzed interest, usefulness, and performance of speech recognition systems for PWS in two ways. 
% We did this in two ways: through a comprehensive survey to understand the perception of PWS and through a user study where participants recorded hundreds of audio clips that could be used for Voice Assistant and Dictation tasks. 
% We performed baseline ASR, endpointing, and intent recognition experiments and report results in Section~\ref{sec:asr_results}. 
% % as well as production-oriented experiments that could be used to improve performance for PWS. 
% Most participants overlapped between the two data modalities so we also looked at correlations between system performance and survey results. 


% \subsection{Survey Design}\label{survey_design}

% Our survey was split into the following four primary sections and included up to \note{87} questions depending on conditional logic. For an expanded listing of survey questions see the Supplementary Material.\todo{verify we can release.}
% \begin{description}
%     \item[Background] Demographics (age group, gender, race/ethnicity); self-description of speech characteristics; intelligibility of speech to family/acquaintances/strangers; ownership and usage of smart devices.

%     \item[Voice Assistants] Usage, usefulness, and accuracy of VAs; why and when do they use VAs; when do they break and areas for improvements; awareness and effectiveness of features including endpointing, hold-to-speak, invocation models, and other common features. 

%     \item[Dictation Systems] Usage, usefulness, and accuracy of DSs; why and when they use DSs; when do they break and areas for improvements; awareness and effectiveness of relevant features, whether people revise or restate transcriptions upon error. 

%     \item[Future Ideation] Interest in VAs/Dictation if speech was perfectly transcribed; interest in personalizing/training models to improve performance; alternative speech-related features.

% \end{description}
% Many of these questions had multiple choice responses and open-ended text input to explain why they chose each response. For questions related to the endpointer and other technical material, layperson descriptions like "How often does a VA cut off your speech" were used. 

% Surveys were filled out online using a commercial survey website. Most participants took 30 to 45 minutes, which and the surveys were collected over a two-month period in Summer 2022. 

% \note{here we talk about did we need to discard any responses and why, how did we analyze the open-ended responses. If we do any statistical analysis we can describe that here.}


% \subsection{Speech Data Collection}

% Each participant was asked to record \todo{121 VA query + 10 dictation if they recorded any dictation messages} audio clips using a smart phone on their own in a quiet environment (SNR > 30 dB). The phone was located about two feet in front of them either in their hand or approximately in that position. Of these clips, 121 were based on Voice Assistant related prompts and others consisted of fake text messages that they might send to a friend, which are more appropriate for the Dictation use case. People were told not to include personal or identifiable information (PII) and this was verified by an outside group. 
% % Audio clips were single phrases or sentences and ranged from two to \_\_\_\_\todo{the range is 1 to 49 words, median is 6 and average is 5.8} words. 
% Audio clips were single phrases or sentences, with a minimum of two words an median of six words.

% Participants were asked to speak naturally. Instead of providing pre-defined phrases, they were given prompts where they came up with their own phrase to accomplish a given task. For example, they were asked to say a phrase to: ``Find out when a place you might want to visit will open,'' ``Find the lyrics to a song that you like,'' and ``Ask about a question about something not well known.'' A complete set is included in the Supplemental Material \note{Can we include?}. 

% All audio clips were manually annotated with the prompt, the phrase they intended to say (e.g., ``what is the weather'', the articulated phrase with dysfluencies (e.g., ``wuh-wuh-what is [...] the weather,'' and an annotation for each dysfluency including starting frame, ending frame, and type. Four stuttering events were noted: part word repetitions, whole word repetitions, sound prolongations, and audible and inaudible blocks.  Interjections were also noted.  A speech language pathologist estimated stuttering severity (no stutter, mild, moderate, severe) per participant using the Andrew and Harris Scale (A\&H) Scale~\cite{?} by grading 100-300 word audio clip samples. the Andrew and Harris scale

% % \textbf{Do we have an explanation for this?: Eight survey respondents did not have annotated data and were not included in the evaluation of speech recognition models.}.

% PWS vary in terms of how many and what types of dysfluencies they produce. This is fluid; someone may produce more or fewer dysfluencies depending on the setting or environment, current mood/stress level, communication partners, or other variables.  Some people stutter frequently when in a group but not when on their own. Some people stutter more when in front of a smart device because of ``pressure to perform.'' The process of creating these audio recordings -- which were done at an individuals convenience while by themselves -- undoubtedly biased the prevalence and severity of stuttering events. For some users events were likely  higher because they knew they were being recorded and for others was likely lower because they could do it when they felt most comfortable. 

% % \subsubsection{Speech Recognition Results}

% % We used production-like models similar to what are deployed for Siri on iOS. Specifically, the endpointer, ASR model, and intent recognition component of the NLU model. 

% % \todo{what details can we use? look at how we did it for the Interspeech paper. }


% \subsection{Participant Recruitment}
% Participants were recruited through social media, referrals from speech language pathology clinics, and word of mouth. Individuals self-identified as having a stutter. An SLP also screened the individuals by listening to their connected speech and by observing overt stuttering characteristics.\note{Colin mentioned there were 4 tasks the vendor's SLP used to screen and grade a participant)}
% The participants who presented as people who stutter were included and graded using A&H Scale into mild, moderate, and severe stuttering groups to ensure adequate severity distribution. In total \note{61} people filled out the survey and \note{91}  contributed audio recordings. 
% % \note{technically 100 people for audio, but we don't have annotations for 8}.
% % \todo{how do we want to discuss Phase 1 and Phase 2? should they be merged entirely? there are some protocol changes like the connected speech sample}
% Of these individuals, [X] were rated as mild (0-5\% of words have dysfluencies), [X] mild (6-20\% dysfluencies), and [X] severe ($\geq$20\% dysfluencies) using the A&H scale. 
% % \subsubsection{Dataset Overview \& Dysfluency Analysis}

% % * Mild: 0-5\% of words have a dysfluency (2 participants in Phase 2)
% % * Moderate: 6-20\% of words have a dysfluency (12 participants in Phase 2)
% % * Severe: >20\% of words have a dysfluency (27 participants in Phase 2)

% % \todo{Maybe add some distribution plots of annotations? Or wait and add correlations with WER and/or truncation rates?}.  %note: I added some plots of correlations with stuttering severity and WER to 4.3.2, they could be moved here

